CaRoSaC: A Reinforcement Learning-Based Kinematic Control of Cable-Driven Parallel Robots by Addressing Cable Sag through Simulation

This paper introduces the Cable Robot Simulation and Control (CaRoSaC) Framework, which integrates a simulation environment with a model-free reinforcement learning control methodology for suspended Cable-Driven Parallel Robots (CDPRs), accounting for cable sag. Our approach seeks to bridge the knowledge gap of the intricacies of CDPRs due to aspects such as cable sag and precision control necessities by establishing a simulation platform that captures the real-world behaviors of CDPRs, including the impacts of cable sag. The framework offers researchers and developers a tool to further develop estimation and control strategies within the simulation for understanding and predicting the performance nuances, especially in complex operations where cable sag can be significant. Using this simulation framework, we train a model-free control policy in Reinforcement Learning (RL). This approach is chosen for its capability to adaptively learn from the complex dynamics of CDPRs. The policy is trained to discern optimal cable control inputs, ensuring precise end-effector positioning. Unlike traditional feedback-based control methods, our RL control policy focuses on kinematic control and addresses the cable sag issues without being tethered to predefined mathematical models. We also demonstrate that our RL-based controller, coupled with the flexible cable simulation, significantly outperforms the classical kinematics approach, particularly in dynamic conditions and near the boundary regions of the workspace. The combined strength of the described simulation and control approach offers an effective solution in manipulating suspended CDPRs even at workspace boundary conditions where traditional approach fails, as proven from our experiments, ensuring that CDPRs function optimally in various applications while accounting for the often neglected but critical factor of cable sag.

==> sections/default.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\placeholder
\newpage
\section{INTRODUCTION}
This template provides authors with most of the formatting specifications needed for preparing electronic versions of their papers. All standard paper components have been specified for three reasons: (1) ease of use when formatting individual papers, (2) automatic compliance to electronic requirements that facilitate the concurrent or later production of electronic products, and (3) conformity of style throughout a conference proceedings. Margins, column widths, line spacing, and type styles are built-in; examples of the type styles are provided throughout this document and are identified in italic type, within parentheses, following the example. Some components, such as multi-leveled equations, graphics, and tables are not prescribed, although the various table text styles are provided. The formatter will need to create these components, incorporating the applicable criteria that follow.

\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
It may be used for A4 paper size if the paper size setting is suitably modified.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as �3.5-inch disk drive�.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: �Wb/m2� or �webers per square meter�, not �webers/m2�.  Spell out units when they appear in text: �. . . a few henries�, not �. . . a few H�.
\item Use a zero before decimal points: �0.25�, not �.25�. Use �cm3�, not �cc�. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use �(1)�, not �Eq. (1)� or �equation (1)�, except at the beginning of a sentence: �Equation (1) is . . .�

\subsection{Some Common Mistakes}
\begin{itemize}


\item The word �data� is plural, not singular.
\item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter �o�.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an �inset�, not an �insert�. The word alternatively is preferred to the word �alternately� (unless you really mean something that alternates).
\item Do not use the word �essentially� to mean �approximately� or �effectively�.
\item In your paper title, if the words �that uses� can accurately replace the word �using�, capitalize the �u�; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones �affect� and �effect�, �complement� and �compliment�, �discreet� and �discrete�, �principal� and �principle�.
\item Do not confuse �imply� and �infer�.
\item The prefix �non� is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the �et� in the Latin abbreviation �et al.�.
\item The abbreviation �i.e.� means �that is�, and the abbreviation �e.g.� means �for example�.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named �Heading 1�, �Heading 2�, �Heading 3�, and �Heading 4� are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation �Fig. 1�, even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity �Magnetization�, or �Magnetization, M�, not just �M�. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write �Magnetization (A/m)� or �Magnetization {A[m(1)]}�, not just �A/m�. Do not label axes with a ratio of quantities and units. For example, write �Temperature (K)�, not �Temperature/K.�

\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word �acknowledgment� in America is without an �e� after the �g�. Avoid the stilted expression, �One of us (R. B. G.) thanks . . .�  Instead, try �R. B. G. thanks�. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.



\begin{thebibliography}{99}

\bibitem{c1} G. O. Young, �Synthetic structure of industrial plastics (Book style with paper title and editor),� 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15�64.
\bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123�135.
\bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
\bibitem{c4} B. Smith, �An approach to graphs of linear forms (Unpublished work style),� unpublished.
\bibitem{c5} E. H. Miller, �A note on reflector arrays (Periodical style�Accepted for publication),� IEEE Trans. Antennas Propagat., to be publised.
\bibitem{c6} J. Wang, �Fundamentals of erbium-doped fiber amplifiers arrays (Periodical style�Submitted for publication),� IEEE J. Quantum Electron., submitted for publication.
\bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
\bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, �Electron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),� IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740�741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
\bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
\bibitem{c10} J. U. Duncombe, �Infrared navigation�Part I: An assessment of feasibility (Periodical style),� IEEE Trans. Electron Devices, vol. ED-11, pp. 34�39, Jan. 1959.
\bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, �A clustering technique for digital communications channel equalization using radial basis function networks,� IEEE Trans. Neural Networks, vol. 4, pp. 570�578, July 1993.
\bibitem{c12} R. W. Lucky, �Automatic equalization for digital communication,� Bell Syst. Tech. J., vol. 44, no. 4, pp. 547�588, Apr. 1965.
\bibitem{c13} S. P. Bingulac, �On the compatibility of adaptive controllers (Published Conference Proceedings style),� in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8�16.
\bibitem{c14} G. R. Faulhaber, �Design of service systems with priority reservation,� in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3�8.
\bibitem{c15} W. D. Doyle, �Magnetization reversal in films with biaxial anisotropy,� in 1987 Proc. INTERMAG Conf., pp. 2.2-1�2.2-6.
\bibitem{c16} G. W. Juette and L. E. Zeffanella, �Radio noise currents n short sections on bundle conductors (Presented Conference Paper style),� presented at the IEEE Summer power Meeting, Dallas, TX, June 22�27, 1990, Paper 90 SM 690-0 PWRS.
\bibitem{c17} J. G. Kreifeldt, �An analysis of surface-detected EMG as an amplitude-modulated noise,� presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
\bibitem{c18} J. Williams, �Narrow-band analyzer (Thesis or Dissertation style),� Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
\bibitem{c19} N. Kawasaki, �Parametric study of thermal and chemical nonequilibrium nozzle flow,� M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
\bibitem{c20} J. P. Wilkinson, �Nonlinear resonant circuit devices (Patent style),� U.S. Patent 3 624 12, July 16, 1990. 






\end{thebibliography}


==> styles/colors.tex <==
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\definecolor{Accent3qual1}{RGB}{127,201,127}
\definecolor{Accent3qual2}{RGB}{190,174,212}
\definecolor{Accent3qual3}{RGB}{253,192,134}
\definecolor{Accent5qual1}{RGB}{127,201,127}
\definecolor{Accent5qual2}{RGB}{190,174,212}
\definecolor{Accent5qual3}{RGB}{253,192,134}
\definecolor{Accent5qual4}{RGB}{255,255,153}
\definecolor{Accent5qual5}{RGB}{56,108,176}
\definecolor{Accent7qual1}{RGB}{127,201,127}
\definecolor{Accent7qual2}{RGB}{190,174,212}
\definecolor{Accent7qual3}{RGB}{253,192,134}
\definecolor{Accent7qual4}{RGB}{255,255,153}
\definecolor{Accent7qual5}{RGB}{56,108,176}
\definecolor{Accent7qual6}{RGB}{240,2,127}
\definecolor{Accent7qual7}{RGB}{191,91,23}

%EDIT: Added number of classes
\definecolor{Blues3seq1}{RGB}{222,235,247}
\definecolor{Blues3seq2}{RGB}{158,202,225}
\definecolor{Blues3seq3}{RGB}{49,130,189}

\definecolor{Blues4seq1}{RGB}{239,243,255}
\definecolor{Blues4seq2}{RGB}{189,215,231}
\definecolor{Blues4seq3}{RGB}{107,174,214}
\definecolor{Blues4seq4}{RGB}{33,113,181}

\definecolor{Blues5seq1}{RGB}{239,243,255}
\definecolor{Blues5seq2}{RGB}{189,215,231}
\definecolor{Blues5seq3}{RGB}{107,174,214}
\definecolor{Blues5seq4}{RGB}{49,130,189}
\definecolor{Blues5seq5}{RGB}{8,81,156}

\definecolor{Blues6seq1}{RGB}{239,243,255}
\definecolor{Blues6seq2}{RGB}{198,219,239}
\definecolor{Blues6seq3}{RGB}{158,202,225}
\definecolor{Blues6seq4}{RGB}{107,174,214}
\definecolor{Blues6seq5}{RGB}{49,130,189}
\definecolor{Blues6seq6}{RGB}{8,81,156}

\definecolor{Blues7seq1}{RGB}{239,243,255}
\definecolor{Blues7seq2}{RGB}{198,219,239}
\definecolor{Blues7seq3}{RGB}{158,202,225}
\definecolor{Blues7seq4}{RGB}{107,174,214}
\definecolor{Blues7seq5}{RGB}{66,146,198}
\definecolor{Blues7seq6}{RGB}{33,113,181}
\definecolor{Blues7seq7}{RGB}{8,69,148}

\definecolor{Blues8seq1}{RGB}{247,251,255}
\definecolor{Blues8seq2}{RGB}{222,235,247}
\definecolor{Blues8seq3}{RGB}{198,219,239}
\definecolor{Blues8seq4}{RGB}{158,202,225}
\definecolor{Blues8seq5}{RGB}{107,174,214}
\definecolor{Blues8seq6}{RGB}{66,146,198}
\definecolor{Blues8seq7}{RGB}{33,113,181}
\definecolor{Blues8seq8}{RGB}{8,69,148}

\definecolor{Blues9seq1}{RGB}{247,251,255}
\definecolor{Blues9seq2}{RGB}{222,235,247}
\definecolor{Blues9seq3}{RGB}{198,219,239}
\definecolor{Blues9seq4}{RGB}{158,202,225}
\definecolor{Blues9seq5}{RGB}{107,174,214}
\definecolor{Blues9seq6}{RGB}{66,146,198}
\definecolor{Blues9seq7}{RGB}{33,113,181}
\definecolor{Blues9seq8}{RGB}{8,81,156}
\definecolor{Blues9seq9}{RGB}{8,48,107}
%END EDIT

\definecolor{BrBG4div1}{RGB}{166,97,26}
\definecolor{BrBG4div2}{RGB}{223,194,125}
\definecolor{BrBG4div3}{RGB}{128,205,193}
\definecolor{BrBG4div4}{RGB}{1,133,113}
\definecolor{BrBG6div1}{RGB}{140,81,10}
\definecolor{BrBG6div2}{RGB}{216,179,101}
\definecolor{BrBG6div3}{RGB}{246,232,195}
\definecolor{BrBG6div4}{RGB}{199,234,229}
\definecolor{BrBG6div5}{RGB}{90,180,172}
\definecolor{BrBG6div6}{RGB}{1,102,94}
\definecolor{BrBG8div1}{RGB}{140,81,10}
\definecolor{BrBG8div2}{RGB}{191,129,45}
\definecolor{BrBG8div3}{RGB}{223,194,125}
\definecolor{BrBG8div4}{RGB}{246,232,195}
\definecolor{BrBG8div5}{RGB}{199,234,229}
\definecolor{BrBG8div6}{RGB}{128,205,193}
\definecolor{BrBG8div7}{RGB}{53,151,143}
\definecolor{BrBG8div8}{RGB}{1,102,94}
\definecolor{BrBG10div1}{RGB}{84,48,5}
\definecolor{BrBG10div2}{RGB}{140,81,10}
\definecolor{BrBG10div3}{RGB}{191,129,45}
\definecolor{BrBG10div4}{RGB}{223,194,125}
\definecolor{BrBG10div5}{RGB}{246,232,195}
\definecolor{BrBG10div6}{RGB}{199,234,229}
\definecolor{BrBG10div7}{RGB}{128,205,193}
\definecolor{BrBG10div8}{RGB}{53,151,143}
\definecolor{BrBG10div9}{RGB}{1,102,94}
\definecolor{BrBG10div10}{RGB}{0,60,48}
\definecolor{BuGn3seq1}{RGB}{229,245,249}
\definecolor{BuGn3seq2}{RGB}{153,216,201}
\definecolor{BuGn3seq3}{RGB}{44,162,95}
\definecolor{BuGn5seq1}{RGB}{237,248,251}
\definecolor{BuGn5seq2}{RGB}{178,226,226}
\definecolor{BuGn5seq3}{RGB}{102,194,164}
\definecolor{BuGn5seq4}{RGB}{44,162,95}
\definecolor{BuGn5seq5}{RGB}{0,109,44}
\definecolor{BuGn7seq1}{RGB}{237,248,251}
\definecolor{BuGn7seq2}{RGB}{204,236,230}
\definecolor{BuGn7seq3}{RGB}{153,216,201}
\definecolor{BuGn7seq4}{RGB}{102,194,164}
\definecolor{BuGn7seq5}{RGB}{65,174,118}
\definecolor{BuGn7seq6}{RGB}{35,139,69}
\definecolor{BuGn7seq7}{RGB}{0,88,36}
\definecolor{BuGn9seq1}{RGB}{247,252,253}
\definecolor{BuGn9seq2}{RGB}{229,245,249}
\definecolor{BuGn9seq3}{RGB}{204,236,230}
\definecolor{BuGn9seq4}{RGB}{153,216,201}
\definecolor{BuGn9seq5}{RGB}{102,194,164}
\definecolor{BuGn9seq6}{RGB}{65,174,118}
\definecolor{BuGn9seq7}{RGB}{35,139,69}
\definecolor{BuGn9seq8}{RGB}{0,109,44}
\definecolor{BuGn9seq9}{RGB}{0,68,27}
\definecolor{BuPu4seq1}{RGB}{237,248,251}
\definecolor{BuPu4seq2}{RGB}{179,205,227}
\definecolor{BuPu4seq3}{RGB}{140,150,198}
\definecolor{BuPu4seq4}{RGB}{136,65,157}
\definecolor{BuPu6seq1}{RGB}{237,248,251}
\definecolor{BuPu6seq2}{RGB}{191,211,230}
\definecolor{BuPu6seq3}{RGB}{158,188,218}
\definecolor{BuPu6seq4}{RGB}{140,150,198}
\definecolor{BuPu6seq5}{RGB}{136,86,167}
\definecolor{BuPu6seq6}{RGB}{129,15,124}
\definecolor{BuPu8seq1}{RGB}{247,252,253}
\definecolor{BuPu8seq2}{RGB}{224,236,244}
\definecolor{BuPu8seq3}{RGB}{191,211,230}
\definecolor{BuPu8seq4}{RGB}{158,188,218}
\definecolor{BuPu8seq5}{RGB}{140,150,198}
\definecolor{BuPu8seq6}{RGB}{140,107,177}
\definecolor{BuPu8seq7}{RGB}{136,65,157}
\definecolor{BuPu8seq8}{RGB}{110,1,107}
\definecolor{Dark23qual1}{RGB}{27,158,119}
\definecolor{Dark23qual2}{RGB}{217,95,2}
\definecolor{Dark23qual3}{RGB}{117,112,179}
\definecolor{Dark25qual1}{RGB}{27,158,119}
\definecolor{Dark25qual2}{RGB}{217,95,2}
\definecolor{Dark25qual3}{RGB}{117,112,179}
\definecolor{Dark25qual4}{RGB}{231,41,138}
\definecolor{Dark25qual5}{RGB}{102,166,30}
\definecolor{Dark27qual1}{RGB}{27,158,119}
\definecolor{Dark27qual2}{RGB}{217,95,2}
\definecolor{Dark27qual3}{RGB}{117,112,179}
\definecolor{Dark27qual4}{RGB}{231,41,138}
\definecolor{Dark27qual5}{RGB}{102,166,30}
\definecolor{Dark27qual6}{RGB}{230,171,2}
\definecolor{Dark27qual7}{RGB}{166,118,29}
\definecolor{GnBu3seq1}{RGB}{224,243,219}
\definecolor{GnBu3seq2}{RGB}{168,221,181}
\definecolor{GnBu3seq3}{RGB}{67,162,202}
\definecolor{GnBu5seq1}{RGB}{240,249,232}
\definecolor{GnBu5seq2}{RGB}{186,228,188}
\definecolor{GnBu5seq3}{RGB}{123,204,196}
\definecolor{GnBu5seq4}{RGB}{67,162,202}
\definecolor{GnBu5seq5}{RGB}{8,104,172}
\definecolor{GnBu7seq1}{RGB}{240,249,232}
\definecolor{GnBu7seq2}{RGB}{204,235,197}
\definecolor{GnBu7seq3}{RGB}{168,221,181}
\definecolor{GnBu7seq4}{RGB}{123,204,196}
\definecolor{GnBu7seq5}{RGB}{78,179,211}
\definecolor{GnBu7seq6}{RGB}{43,140,190}
\definecolor{GnBu7seq7}{RGB}{8,88,158}
\definecolor{GnBu9seq1}{RGB}{247,252,240}
\definecolor{GnBu9seq2}{RGB}{224,243,219}
\definecolor{GnBu9seq3}{RGB}{204,235,197}
\definecolor{GnBu9seq4}{RGB}{168,221,181}
\definecolor{GnBu9seq5}{RGB}{123,204,196}
\definecolor{GnBu9seq6}{RGB}{78,179,211}
\definecolor{GnBu9seq7}{RGB}{43,140,190}
\definecolor{GnBu9seq8}{RGB}{8,104,172}
\definecolor{GnBu9seq9}{RGB}{8,64,129}

%EDIT: Added number of classes 
\definecolor{Greens3seq1}{RGB}{237,248,233}
\definecolor{Greens3seq2}{RGB}{161,217,155}
\definecolor{Greens3seq3}{RGB}{49,163,84}

\definecolor{Greens4seq1}{RGB}{237,248,233}
\definecolor{Greens4seq2}{RGB}{186,228,179}
\definecolor{Greens4seq3}{RGB}{116,196,118}
\definecolor{Greens4seq4}{RGB}{35,139,69}

\definecolor{Greens5seq1}{RGB}{237,248,233}
\definecolor{Greens5seq2}{RGB}{186,228,179}
\definecolor{Greens5seq3}{RGB}{116,196,118}
\definecolor{Greens5seq4}{RGB}{49,163,84}
\definecolor{Greens5seq5}{RGB}{0,109,44}

\definecolor{Greens6seq1}{RGB}{237,248,233}
\definecolor{Greens6seq2}{RGB}{199,233,192}
\definecolor{Greens6seq3}{RGB}{161,217,155}
\definecolor{Greens6seq4}{RGB}{116,196,118}
\definecolor{Greens6seq5}{RGB}{49,163,84}
\definecolor{Greens6seq6}{RGB}{0,109,44}

\definecolor{Greens7seq1}{RGB}{237,248,233}
\definecolor{Greens7seq2}{RGB}{199,233,192}
\definecolor{Greens7seq3}{RGB}{161,217,155}
\definecolor{Greens7seq4}{RGB}{116,196,118}
\definecolor{Greens7seq5}{RGB}{65,171,93}
\definecolor{Greens7seq6}{RGB}{35,139,69}
\definecolor{Greens7seq7}{RGB}{0,90,50}

\definecolor{Greens8seq1}{RGB}{247,252,245}
\definecolor{Greens8seq2}{RGB}{229,245,224}
\definecolor{Greens8seq3}{RGB}{199,233,192}
\definecolor{Greens8seq4}{RGB}{161,217,155}
\definecolor{Greens8seq5}{RGB}{116,196,118}
\definecolor{Greens8seq6}{RGB}{65,171,93}
\definecolor{Greens8seq7}{RGB}{35,139,69}
\definecolor{Greens8seq8}{RGB}{0,90,50}

\definecolor{Greens9seq1}{RGB}{247,252,245}
\definecolor{Greens9seq2}{RGB}{229,245,224}
\definecolor{Greens9seq3}{RGB}{199,233,192}
\definecolor{Greens9seq4}{RGB}{161,217,155}
\definecolor{Greens9seq5}{RGB}{116,196,118}
\definecolor{Greens9seq6}{RGB}{65,171,93}
\definecolor{Greens9seq7}{RGB}{35,139,69}
\definecolor{Greens9seq8}{RGB}{0,109,44}
\definecolor{Greens9seq9}{RGB}{0,68,27}
%END EDIT

\definecolor{Greys3seq1}{RGB}{240,240,240}
\definecolor{Greys3seq2}{RGB}{189,189,189}
\definecolor{Greys3seq3}{RGB}{99,99,99}
\definecolor{Greys5seq1}{RGB}{247,247,247}
\definecolor{Greys5seq2}{RGB}{204,204,204}
\definecolor{Greys5seq3}{RGB}{150,150,150}
\definecolor{Greys5seq4}{RGB}{99,99,99}
\definecolor{Greys5seq5}{RGB}{37,37,37}
\definecolor{Greys7seq1}{RGB}{247,247,247}
\definecolor{Greys7seq2}{RGB}{217,217,217}
\definecolor{Greys7seq3}{RGB}{189,189,189}
\definecolor{Greys7seq4}{RGB}{150,150,150}
\definecolor{Greys7seq5}{RGB}{115,115,115}
\definecolor{Greys7seq6}{RGB}{82,82,82}
\definecolor{Greys7seq7}{RGB}{37,37,37}
\definecolor{Greys9seq1}{RGB}{255,255,255}
\definecolor{Greys9seq2}{RGB}{240,240,240}
\definecolor{Greys9seq3}{RGB}{217,217,217}
\definecolor{Greys9seq4}{RGB}{189,189,189}
\definecolor{Greys9seq5}{RGB}{150,150,150}
\definecolor{Greys9seq6}{RGB}{115,115,115}
\definecolor{Greys9seq7}{RGB}{82,82,82}
\definecolor{Greys9seq8}{RGB}{37,37,37}
\definecolor{Greys9seq9}{RGB}{0,0,0}
\definecolor{Oranges4seq1}{RGB}{254,237,222}
\definecolor{Oranges4seq2}{RGB}{253,190,133}
\definecolor{Oranges4seq3}{RGB}{253,141,60}
\definecolor{Oranges4seq4}{RGB}{217,71,1}
\definecolor{Oranges6seq1}{RGB}{254,237,222}
\definecolor{Oranges6seq2}{RGB}{253,208,162}
\definecolor{Oranges6seq3}{RGB}{253,174,107}
\definecolor{Oranges6seq4}{RGB}{253,141,60}
\definecolor{Oranges6seq5}{RGB}{230,85,13}
\definecolor{Oranges6seq6}{RGB}{166,54,3}
\definecolor{Oranges8seq1}{RGB}{255,245,235}
\definecolor{Oranges8seq2}{RGB}{254,230,206}
\definecolor{Oranges8seq3}{RGB}{253,208,162}
\definecolor{Oranges8seq4}{RGB}{253,174,107}
\definecolor{Oranges8seq5}{RGB}{253,141,60}
\definecolor{Oranges8seq6}{RGB}{241,105,19}
\definecolor{Oranges8seq7}{RGB}{217,72,1}
\definecolor{Oranges8seq8}{RGB}{140,45,4}
\definecolor{OrRd3seq1}{RGB}{254,232,200}
\definecolor{OrRd3seq2}{RGB}{253,187,132}
\definecolor{OrRd3seq3}{RGB}{227,74,51}
\definecolor{OrRd5seq1}{RGB}{254,240,217}
\definecolor{OrRd5seq2}{RGB}{253,204,138}
\definecolor{OrRd5seq3}{RGB}{252,141,89}
\definecolor{OrRd5seq4}{RGB}{227,74,51}
\definecolor{OrRd5seq5}{RGB}{179,0,0}
\definecolor{OrRd7seq1}{RGB}{254,240,217}
\definecolor{OrRd7seq2}{RGB}{253,212,158}
\definecolor{OrRd7seq3}{RGB}{253,187,132}
\definecolor{OrRd7seq4}{RGB}{252,141,89}
\definecolor{OrRd7seq5}{RGB}{239,101,72}
\definecolor{OrRd7seq6}{RGB}{215,48,31}
\definecolor{OrRd7seq7}{RGB}{153,0,0}
\definecolor{OrRd9seq1}{RGB}{255,247,236}
\definecolor{OrRd9seq2}{RGB}{254,232,200}
\definecolor{OrRd9seq3}{RGB}{253,212,158}
\definecolor{OrRd9seq4}{RGB}{253,187,132}
\definecolor{OrRd9seq5}{RGB}{252,141,89}
\definecolor{OrRd9seq6}{RGB}{239,101,72}
\definecolor{OrRd9seq7}{RGB}{215,48,31}
\definecolor{OrRd9seq8}{RGB}{179,0,0}
\definecolor{OrRd9seq9}{RGB}{127,0,0}

%EDIT: Added number of classes
\definecolor{Paired3qual1}{RGB}{166,206,227}
\definecolor{Paired3qual2}{RGB}{31,120,180}
\definecolor{Paired3qual3}{RGB}{178,223,138}

\definecolor{Paired4qual1}{RGB}{166,206,227}
\definecolor{Paired4qual2}{RGB}{31,120,180}
\definecolor{Paired4qual3}{RGB}{178,223,138}
\definecolor{Paired4qual4}{RGB}{51,160,44}

\definecolor{Paired5qual1}{RGB}{166,206,227}
\definecolor{Paired5qual2}{RGB}{31,120,180}
\definecolor{Paired5qual3}{RGB}{178,223,138}
\definecolor{Paired5qual4}{RGB}{51,160,44}
\definecolor{Paired5qual5}{RGB}{251,154,153}

\definecolor{Paired6qual1}{RGB}{166,206,227}
\definecolor{Paired6qual2}{RGB}{31,120,180}
\definecolor{Paired6qual3}{RGB}{178,223,138}
\definecolor{Paired6qual4}{RGB}{51,160,44}
\definecolor{Paired6qual5}{RGB}{251,154,153}
\definecolor{Paired6qual6}{RGB}{227,26,28}

\definecolor{Paired7qual1}{RGB}{166,206,227}
\definecolor{Paired7qual2}{RGB}{31,120,180}
\definecolor{Paired7qual3}{RGB}{178,223,138}
\definecolor{Paired7qual4}{RGB}{51,160,44}
\definecolor{Paired7qual5}{RGB}{251,154,153}
\definecolor{Paired7qual6}{RGB}{227,26,28}
\definecolor{Paired7qual7}{RGB}{253,191,111}

\definecolor{Paired8qual1}{RGB}{166,206,227}
\definecolor{Paired8qual2}{RGB}{31,120,180}
\definecolor{Paired8qual3}{RGB}{178,223,138}
\definecolor{Paired8qual4}{RGB}{51,160,44}
\definecolor{Paired8qual5}{RGB}{251,154,153}
\definecolor{Paired8qual6}{RGB}{227,26,28}
\definecolor{Paired8qual7}{RGB}{253,191,111}
\definecolor{Paired8qual8}{RGB}{255,127,0}

\definecolor{Paired9qual1}{RGB}{166,206,227}
\definecolor{Paired9qual2}{RGB}{31,120,180}
\definecolor{Paired9qual3}{RGB}{178,223,138}
\definecolor{Paired9qual4}{RGB}{51,160,44}
\definecolor{Paired9qual5}{RGB}{251,154,153}
\definecolor{Paired9qual6}{RGB}{227,26,28}
\definecolor{Paired9qual7}{RGB}{253,191,111}
\definecolor{Paired9qual8}{RGB}{255,127,0}
\definecolor{Paired9qual9}{RGB}{202,178,214}

\definecolor{Paired10qual1}{RGB}{166,206,227}
\definecolor{Paired10qual2}{RGB}{31,120,180}
\definecolor{Paired10qual3}{RGB}{178,223,138}
\definecolor{Paired10qual4}{RGB}{51,160,44}
\definecolor{Paired10qual5}{RGB}{251,154,153}
\definecolor{Paired10qual6}{RGB}{227,26,28}
\definecolor{Paired10qual7}{RGB}{253,191,111}
\definecolor{Paired10qual8}{RGB}{255,127,0}
\definecolor{Paired10qual9}{RGB}{202,178,214}
\definecolor{Paired10qual10}{RGB}{106,61,154}

\definecolor{Paired12qual1}{RGB}{166,206,227}
\definecolor{Paired12qual2}{RGB}{31,120,180}
\definecolor{Paired12qual3}{RGB}{178,223,138}
\definecolor{Paired12qual4}{RGB}{51,160,44}
\definecolor{Paired12qual5}{RGB}{251,154,153}
\definecolor{Paired12qual6}{RGB}{227,26,28}
\definecolor{Paired12qual7}{RGB}{253,191,111}
\definecolor{Paired12qual8}{RGB}{255,127,0}
\definecolor{Paired12qual9}{RGB}{202,178,214}
\definecolor{Paired12qual10}{RGB}{106,61,154}
\definecolor{Paired12qual11}{RGB}{255,255,153}
\definecolor{Paired12qual12}{RGB}{177,89,40}
%END EDIT

\definecolor{Pastel14qual1}{RGB}{251,180,174}
\definecolor{Pastel14qual2}{RGB}{179,205,227}
\definecolor{Pastel14qual3}{RGB}{204,235,197}
\definecolor{Pastel14qual4}{RGB}{222,203,228}
\definecolor{Pastel16qual1}{RGB}{251,180,174}
\definecolor{Pastel16qual2}{RGB}{179,205,227}
\definecolor{Pastel16qual3}{RGB}{204,235,197}
\definecolor{Pastel16qual4}{RGB}{222,203,228}
\definecolor{Pastel16qual5}{RGB}{254,217,166}
\definecolor{Pastel16qual6}{RGB}{255,255,204}
\definecolor{Pastel18qual1}{RGB}{251,180,174}
\definecolor{Pastel18qual2}{RGB}{179,205,227}
\definecolor{Pastel18qual3}{RGB}{204,235,197}
\definecolor{Pastel18qual4}{RGB}{222,203,228}
\definecolor{Pastel18qual5}{RGB}{254,217,166}
\definecolor{Pastel18qual6}{RGB}{255,255,204}
\definecolor{Pastel18qual7}{RGB}{229,216,189}
\definecolor{Pastel18qual8}{RGB}{253,218,236}
\definecolor{Pastel23qual1}{RGB}{179,226,205}
\definecolor{Pastel23qual2}{RGB}{253,205,172}
\definecolor{Pastel23qual3}{RGB}{203,213,232}
\definecolor{Pastel25qual1}{RGB}{179,226,205}
\definecolor{Pastel25qual2}{RGB}{253,205,172}
\definecolor{Pastel25qual3}{RGB}{203,213,232}
\definecolor{Pastel25qual4}{RGB}{244,202,228}
\definecolor{Pastel25qual5}{RGB}{230,245,201}
\definecolor{Pastel27qual1}{RGB}{179,226,205}
\definecolor{Pastel27qual2}{RGB}{253,205,172}
\definecolor{Pastel27qual3}{RGB}{203,213,232}
\definecolor{Pastel27qual4}{RGB}{244,202,228}
\definecolor{Pastel27qual5}{RGB}{230,245,201}
\definecolor{Pastel27qual6}{RGB}{255,242,174}
\definecolor{Pastel27qual7}{RGB}{241,226,204}
\definecolor{PiYG3div1}{RGB}{233,163,201}
\definecolor{PiYG3div2}{RGB}{247,247,247}
\definecolor{PiYG3div3}{RGB}{161,215,106}
\definecolor{PiYG5div1}{RGB}{208,28,139}
\definecolor{PiYG5div2}{RGB}{241,182,218}
\definecolor{PiYG5div3}{RGB}{247,247,247}
\definecolor{PiYG5div4}{RGB}{184,225,134}
\definecolor{PiYG5div5}{RGB}{77,172,38}
\definecolor{PiYG7div1}{RGB}{197,27,125}
\definecolor{PiYG7div2}{RGB}{233,163,201}
\definecolor{PiYG7div3}{RGB}{253,224,239}
\definecolor{PiYG7div4}{RGB}{247,247,247}
\definecolor{PiYG7div5}{RGB}{230,245,208}
\definecolor{PiYG7div6}{RGB}{161,215,106}
\definecolor{PiYG7div7}{RGB}{77,146,33}
\definecolor{PiYG9div1}{RGB}{197,27,125}
\definecolor{PiYG9div2}{RGB}{222,119,174}
\definecolor{PiYG9div3}{RGB}{241,182,218}
\definecolor{PiYG9div4}{RGB}{253,224,239}
\definecolor{PiYG9div5}{RGB}{247,247,247}
\definecolor{PiYG9div6}{RGB}{230,245,208}
\definecolor{PiYG9div7}{RGB}{184,225,134}
\definecolor{PiYG9div8}{RGB}{127,188,65}
\definecolor{PiYG9div9}{RGB}{77,146,33}
\definecolor{PiYG11div1}{RGB}{142,1,82}
\definecolor{PiYG11div2}{RGB}{197,27,125}
\definecolor{PiYG11div3}{RGB}{222,119,174}
\definecolor{PiYG11div4}{RGB}{241,182,218}
\definecolor{PiYG11div5}{RGB}{253,224,239}
\definecolor{PiYG11div6}{RGB}{247,247,247}
\definecolor{PiYG11div7}{RGB}{230,245,208}
\definecolor{PiYG11div8}{RGB}{184,225,134}
\definecolor{PiYG11div9}{RGB}{127,188,65}
\definecolor{PiYG11div10}{RGB}{77,146,33}
\definecolor{PiYG11div11}{RGB}{39,100,25}
\definecolor{PRGn4div1}{RGB}{123,50,148}
\definecolor{PRGn4div2}{RGB}{194,165,207}
\definecolor{PRGn4div3}{RGB}{166,219,160}
\definecolor{PRGn4div4}{RGB}{0,136,55}
\definecolor{PRGn6div1}{RGB}{118,42,131}
\definecolor{PRGn6div2}{RGB}{175,141,195}
\definecolor{PRGn6div3}{RGB}{231,212,232}
\definecolor{PRGn6div4}{RGB}{217,240,211}
\definecolor{PRGn6div5}{RGB}{127,191,123}
\definecolor{PRGn6div6}{RGB}{27,120,55}
\definecolor{PRGn8div1}{RGB}{118,42,131}
\definecolor{PRGn8div2}{RGB}{153,112,171}
\definecolor{PRGn8div3}{RGB}{194,165,207}
\definecolor{PRGn8div4}{RGB}{231,212,232}
\definecolor{PRGn8div5}{RGB}{217,240,211}
\definecolor{PRGn8div6}{RGB}{166,219,160}
\definecolor{PRGn8div7}{RGB}{90,174,97}
\definecolor{PRGn8div8}{RGB}{27,120,55}
\definecolor{PRGn10div1}{RGB}{64,0,75}
\definecolor{PRGn10div2}{RGB}{118,42,131}
\definecolor{PRGn10div3}{RGB}{153,112,171}
\definecolor{PRGn10div4}{RGB}{194,165,207}
\definecolor{PRGn10div5}{RGB}{231,212,232}
\definecolor{PRGn10div6}{RGB}{217,240,211}
\definecolor{PRGn10div7}{RGB}{166,219,160}
\definecolor{PRGn10div8}{RGB}{90,174,97}
\definecolor{PRGn10div9}{RGB}{27,120,55}
\definecolor{PRGn10div10}{RGB}{0,68,27}
\definecolor{PuBu3seq1}{RGB}{236,231,242}
\definecolor{PuBu3seq2}{RGB}{166,189,219}
\definecolor{PuBu3seq3}{RGB}{43,140,190}
\definecolor{PuBu5seq1}{RGB}{241,238,246}
\definecolor{PuBu5seq2}{RGB}{189,201,225}
\definecolor{PuBu5seq3}{RGB}{116,169,207}
\definecolor{PuBu5seq4}{RGB}{43,140,190}
\definecolor{PuBu5seq5}{RGB}{4,90,141}
\definecolor{PuBu7seq1}{RGB}{241,238,246}
\definecolor{PuBu7seq2}{RGB}{208,209,230}
\definecolor{PuBu7seq3}{RGB}{166,189,219}
\definecolor{PuBu7seq4}{RGB}{116,169,207}
\definecolor{PuBu7seq5}{RGB}{54,144,192}
\definecolor{PuBu7seq6}{RGB}{5,112,176}
\definecolor{PuBu7seq7}{RGB}{3,78,123}
\definecolor{PuBu9seq1}{RGB}{255,247,251}
\definecolor{PuBu9seq2}{RGB}{236,231,242}
\definecolor{PuBu9seq3}{RGB}{208,209,230}
\definecolor{PuBu9seq4}{RGB}{166,189,219}
\definecolor{PuBu9seq5}{RGB}{116,169,207}
\definecolor{PuBu9seq6}{RGB}{54,144,192}
\definecolor{PuBu9seq7}{RGB}{5,112,176}
\definecolor{PuBu9seq8}{RGB}{4,90,141}
\definecolor{PuBu9seq9}{RGB}{2,56,88}
\definecolor{PuBuGn4seq1}{RGB}{246,239,247}
\definecolor{PuBuGn4seq2}{RGB}{189,201,225}
\definecolor{PuBuGn4seq3}{RGB}{103,169,207}
\definecolor{PuBuGn4seq4}{RGB}{2,129,138}
\definecolor{PuBuGn6seq1}{RGB}{246,239,247}
\definecolor{PuBuGn6seq2}{RGB}{208,209,230}
\definecolor{PuBuGn6seq3}{RGB}{166,189,219}
\definecolor{PuBuGn6seq4}{RGB}{103,169,207}
\definecolor{PuBuGn6seq5}{RGB}{28,144,153}
\definecolor{PuBuGn6seq6}{RGB}{1,108,89}
\definecolor{PuBuGn8seq1}{RGB}{255,247,251}
\definecolor{PuBuGn8seq2}{RGB}{236,226,240}
\definecolor{PuBuGn8seq3}{RGB}{208,209,230}
\definecolor{PuBuGn8seq4}{RGB}{166,189,219}
\definecolor{PuBuGn8seq5}{RGB}{103,169,207}
\definecolor{PuBuGn8seq6}{RGB}{54,144,192}
\definecolor{PuBuGn8seq7}{RGB}{2,129,138}
\definecolor{PuBuGn8seq8}{RGB}{1,100,80}
\definecolor{PuOr3div1}{RGB}{241,163,64}
\definecolor{PuOr3div2}{RGB}{247,247,247}
\definecolor{PuOr3div3}{RGB}{153,142,195}
\definecolor{PuOr5div1}{RGB}{230,97,1}
\definecolor{PuOr5div2}{RGB}{253,184,99}
\definecolor{PuOr5div3}{RGB}{247,247,247}
\definecolor{PuOr5div4}{RGB}{178,171,210}
\definecolor{PuOr5div5}{RGB}{94,60,153}
\definecolor{PuOr7div1}{RGB}{179,88,6}
\definecolor{PuOr7div2}{RGB}{241,163,64}
\definecolor{PuOr7div3}{RGB}{254,224,182}
\definecolor{PuOr7div4}{RGB}{247,247,247}
\definecolor{PuOr7div5}{RGB}{216,218,235}
\definecolor{PuOr7div6}{RGB}{153,142,195}
\definecolor{PuOr7div7}{RGB}{84,39,136}
\definecolor{PuOr9div1}{RGB}{179,88,6}
\definecolor{PuOr9div2}{RGB}{224,130,20}
\definecolor{PuOr9div3}{RGB}{253,184,99}
\definecolor{PuOr9div4}{RGB}{254,224,182}
\definecolor{PuOr9div5}{RGB}{247,247,247}
\definecolor{PuOr9div6}{RGB}{216,218,235}
\definecolor{PuOr9div7}{RGB}{178,171,210}
\definecolor{PuOr9div8}{RGB}{128,115,172}
\definecolor{PuOr9div9}{RGB}{84,39,136}
\definecolor{PuOr11div1}{RGB}{127,59,8}
\definecolor{PuOr11div2}{RGB}{179,88,6}
\definecolor{PuOr11div3}{RGB}{224,130,20}
\definecolor{PuOr11div4}{RGB}{253,184,99}
\definecolor{PuOr11div5}{RGB}{254,224,182}
\definecolor{PuOr11div6}{RGB}{247,247,247}
\definecolor{PuOr11div7}{RGB}{216,218,235}
\definecolor{PuOr11div8}{RGB}{178,171,210}
\definecolor{PuOr11div9}{RGB}{128,115,172}
\definecolor{PuOr11div10}{RGB}{84,39,136}
\definecolor{PuOr11div11}{RGB}{45,0,75}
\definecolor{PuRd4seq1}{RGB}{241,238,246}
\definecolor{PuRd4seq2}{RGB}{215,181,216}
\definecolor{PuRd4seq3}{RGB}{223,101,176}
\definecolor{PuRd4seq4}{RGB}{206,18,86}
\definecolor{PuRd6seq1}{RGB}{241,238,246}
\definecolor{PuRd6seq2}{RGB}{212,185,218}
\definecolor{PuRd6seq3}{RGB}{201,148,199}
\definecolor{PuRd6seq4}{RGB}{223,101,176}
\definecolor{PuRd6seq5}{RGB}{221,28,119}
\definecolor{PuRd6seq6}{RGB}{152,0,67}
\definecolor{PuRd8seq1}{RGB}{247,244,249}
\definecolor{PuRd8seq2}{RGB}{231,225,239}
\definecolor{PuRd8seq3}{RGB}{212,185,218}
\definecolor{PuRd8seq4}{RGB}{201,148,199}
\definecolor{PuRd8seq5}{RGB}{223,101,176}
\definecolor{PuRd8seq6}{RGB}{231,41,138}
\definecolor{PuRd8seq7}{RGB}{206,18,86}
\definecolor{PuRd8seq8}{RGB}{145,0,63}
\definecolor{Purples3seq1}{RGB}{239,237,245}
\definecolor{Purples3seq2}{RGB}{188,189,220}
\definecolor{Purples3seq3}{RGB}{117,107,177}
\definecolor{Purples5seq1}{RGB}{242,240,247}
\definecolor{Purples5seq2}{RGB}{203,201,226}
\definecolor{Purples5seq3}{RGB}{158,154,200}
\definecolor{Purples5seq4}{RGB}{117,107,177}
\definecolor{Purples5seq5}{RGB}{84,39,143}
\definecolor{Purples7seq1}{RGB}{242,240,247}
\definecolor{Purples7seq2}{RGB}{218,218,235}
\definecolor{Purples7seq3}{RGB}{188,189,220}
\definecolor{Purples7seq4}{RGB}{158,154,200}
\definecolor{Purples7seq5}{RGB}{128,125,186}
\definecolor{Purples7seq6}{RGB}{106,81,163}
\definecolor{Purples7seq7}{RGB}{74,20,134}
\definecolor{Purples9seq1}{RGB}{252,251,253}
\definecolor{Purples9seq2}{RGB}{239,237,245}
\definecolor{Purples9seq3}{RGB}{218,218,235}
\definecolor{Purples9seq4}{RGB}{188,189,220}
\definecolor{Purples9seq5}{RGB}{158,154,200}
\definecolor{Purples9seq6}{RGB}{128,125,186}
\definecolor{Purples9seq7}{RGB}{106,81,163}
\definecolor{Purples9seq8}{RGB}{84,39,143}
\definecolor{Purples9seq9}{RGB}{63,0,125}
\definecolor{RdBu4div1}{RGB}{202,0,32}
\definecolor{RdBu4div2}{RGB}{244,165,130}
\definecolor{RdBu4div3}{RGB}{146,197,222}
\definecolor{RdBu4div4}{RGB}{5,113,176}
\definecolor{RdBu6div1}{RGB}{178,24,43}
\definecolor{RdBu6div2}{RGB}{239,138,98}
\definecolor{RdBu6div3}{RGB}{253,219,199}
\definecolor{RdBu6div4}{RGB}{209,229,240}
\definecolor{RdBu6div5}{RGB}{103,169,207}
\definecolor{RdBu6div6}{RGB}{33,102,172}
\definecolor{RdBu8div1}{RGB}{178,24,43}
\definecolor{RdBu8div2}{RGB}{214,96,77}
\definecolor{RdBu8div3}{RGB}{244,165,130}
\definecolor{RdBu8div4}{RGB}{253,219,199}
\definecolor{RdBu8div5}{RGB}{209,229,240}
\definecolor{RdBu8div6}{RGB}{146,197,222}
\definecolor{RdBu8div7}{RGB}{67,147,195}
\definecolor{RdBu8div8}{RGB}{33,102,172}
\definecolor{RdBu10div1}{RGB}{103,0,31}
\definecolor{RdBu10div2}{RGB}{178,24,43}
\definecolor{RdBu10div3}{RGB}{214,96,77}
\definecolor{RdBu10div4}{RGB}{244,165,130}
\definecolor{RdBu10div5}{RGB}{253,219,199}
\definecolor{RdBu10div6}{RGB}{209,229,240}
\definecolor{RdBu10div7}{RGB}{146,197,222}
\definecolor{RdBu10div8}{RGB}{67,147,195}
\definecolor{RdBu10div9}{RGB}{33,102,172}
\definecolor{RdBu10div10}{RGB}{5,48,97}
\definecolor{RdGy3div1}{RGB}{239,138,98}
\definecolor{RdGy3div2}{RGB}{255,255,255}
\definecolor{RdGy3div3}{RGB}{153,153,153}
\definecolor{RdGy5div1}{RGB}{202,0,32}
\definecolor{RdGy5div2}{RGB}{244,165,130}
\definecolor{RdGy5div3}{RGB}{255,255,255}
\definecolor{RdGy5div4}{RGB}{186,186,186}
\definecolor{RdGy5div5}{RGB}{64,64,64}
\definecolor{RdGy7div1}{RGB}{178,24,43}
\definecolor{RdGy7div2}{RGB}{239,138,98}
\definecolor{RdGy7div3}{RGB}{253,219,199}
\definecolor{RdGy7div4}{RGB}{255,255,255}
\definecolor{RdGy7div5}{RGB}{224,224,224}
\definecolor{RdGy7div6}{RGB}{153,153,153}
\definecolor{RdGy7div7}{RGB}{77,77,77}
\definecolor{RdGy9div1}{RGB}{178,24,43}
\definecolor{RdGy9div2}{RGB}{214,96,77}
\definecolor{RdGy9div3}{RGB}{244,165,130}
\definecolor{RdGy9div4}{RGB}{253,219,199}
\definecolor{RdGy9div5}{RGB}{255,255,255}
\definecolor{RdGy9div6}{RGB}{224,224,224}
\definecolor{RdGy9div7}{RGB}{186,186,186}
\definecolor{RdGy9div8}{RGB}{135,135,135}
\definecolor{RdGy9div9}{RGB}{77,77,77}
\definecolor{RdGy11div1}{RGB}{103,0,31}
\definecolor{RdGy11div2}{RGB}{178,24,43}
\definecolor{RdGy11div3}{RGB}{214,96,77}
\definecolor{RdGy11div4}{RGB}{244,165,130}
\definecolor{RdGy11div5}{RGB}{253,219,199}
\definecolor{RdGy11div6}{RGB}{255,255,255}
\definecolor{RdGy11div7}{RGB}{224,224,224}
\definecolor{RdGy11div8}{RGB}{186,186,186}
\definecolor{RdGy11div9}{RGB}{135,135,135}
\definecolor{RdGy11div10}{RGB}{77,77,77}
\definecolor{RdGy11div11}{RGB}{26,26,26}
\definecolor{RdPu4seq1}{RGB}{254,235,226}
\definecolor{RdPu4seq2}{RGB}{251,180,185}
\definecolor{RdPu4seq3}{RGB}{247,104,161}
\definecolor{RdPu4seq4}{RGB}{174,1,126}
\definecolor{RdPu6seq1}{RGB}{254,235,226}
\definecolor{RdPu6seq2}{RGB}{252,197,192}
\definecolor{RdPu6seq3}{RGB}{250,159,181}
\definecolor{RdPu6seq4}{RGB}{247,104,161}
\definecolor{RdPu6seq5}{RGB}{197,27,138}
\definecolor{RdPu6seq6}{RGB}{122,1,119}
\definecolor{RdPu8seq1}{RGB}{255,247,243}
\definecolor{RdPu8seq2}{RGB}{253,224,221}
\definecolor{RdPu8seq3}{RGB}{252,197,192}
\definecolor{RdPu8seq4}{RGB}{250,159,181}
\definecolor{RdPu8seq5}{RGB}{247,104,161}
\definecolor{RdPu8seq6}{RGB}{221,52,151}
\definecolor{RdPu8seq7}{RGB}{174,1,126}
\definecolor{RdPu8seq8}{RGB}{122,1,119}

%EDIT: Added number of classes
\definecolor{Reds3seq1}{RGB}{254,224,210}
\definecolor{Reds3seq2}{RGB}{252,146,114}
\definecolor{Reds3seq3}{RGB}{222,45,38}

\definecolor{Reds4seq1}{RGB}{254,229,217}
\definecolor{Reds4seq2}{RGB}{252,174,145}
\definecolor{Reds4seq3}{RGB}{251,106,74}
\definecolor{Reds4seq4}{RGB}{203,24,29}

\definecolor{Reds5seq1}{RGB}{254,229,217}
\definecolor{Reds5seq2}{RGB}{252,174,145}
\definecolor{Reds5seq3}{RGB}{251,106,74}
\definecolor{Reds5seq4}{RGB}{222,45,38}
\definecolor{Reds5seq5}{RGB}{165,15,21}

\definecolor{Reds6seq1}{RGB}{254,229,217}
\definecolor{Reds6seq2}{RGB}{252,187,161}
\definecolor{Reds6seq3}{RGB}{252,146,114}
\definecolor{Reds6seq4}{RGB}{251,106,74}
\definecolor{Reds6seq5}{RGB}{222,45,38}
\definecolor{Reds6seq6}{RGB}{165,15,21}

\definecolor{Reds7seq1}{RGB}{254,229,217}
\definecolor{Reds7seq2}{RGB}{252,187,161}
\definecolor{Reds7seq3}{RGB}{252,146,114}
\definecolor{Reds7seq4}{RGB}{251,106,74}
\definecolor{Reds7seq5}{RGB}{239,59,44}
\definecolor{Reds7seq6}{RGB}{203,24,29}
\definecolor{Reds7seq7}{RGB}{153,0,13}

\definecolor{Reds8seq1}{RGB}{255,245,240}
\definecolor{Reds8seq2}{RGB}{254,224,210}
\definecolor{Reds8seq3}{RGB}{252,187,161}
\definecolor{Reds8seq4}{RGB}{252,146,114}
\definecolor{Reds8seq5}{RGB}{251,106,74}
\definecolor{Reds8seq6}{RGB}{239,59,44}
\definecolor{Reds8seq7}{RGB}{203,24,29}
\definecolor{Reds8seq8}{RGB}{153,0,13}

\definecolor{Reds9seq1}{RGB}{255,245,240}
\definecolor{Reds9seq2}{RGB}{254,224,210}
\definecolor{Reds9seq3}{RGB}{252,187,161}
\definecolor{Reds9seq4}{RGB}{252,146,114}
\definecolor{Reds9seq5}{RGB}{251,106,74}
\definecolor{Reds9seq6}{RGB}{239,59,44}
\definecolor{Reds9seq7}{RGB}{203,24,29}
\definecolor{Reds9seq8}{RGB}{165,15,21}
\definecolor{Reds9seq9}{RGB}{103,0,13}

\definecolor{RdYlBu3div1}{RGB}{252,141,89}
\definecolor{RdYlBu3div2}{RGB}{255,255,191}
\definecolor{RdYlBu3div3}{RGB}{145,191,219}

\definecolor{RdYlBu4div1}{RGB}{215,25,28}
\definecolor{RdYlBu4div2}{RGB}{253,174,97}
\definecolor{RdYlBu4div3}{RGB}{171,217,233}
\definecolor{RdYlBu4div4}{RGB}{44,123,182}

\definecolor{RdYlBu5div1}{RGB}{215,25,28}
\definecolor{RdYlBu5div2}{RGB}{253,174,97}
\definecolor{RdYlBu5div3}{RGB}{255,255,191}
\definecolor{RdYlBu5div4}{RGB}{171,217,233}
\definecolor{RdYlBu5div5}{RGB}{44,123,182}

\definecolor{RdYlBu6div1}{RGB}{215,48,39}
\definecolor{RdYlBu6div2}{RGB}{252,141,89}
\definecolor{RdYlBu6div3}{RGB}{254,224,144}
\definecolor{RdYlBu6div4}{RGB}{224,243,248}
\definecolor{RdYlBu6div5}{RGB}{145,191,219}
\definecolor{RdYlBu6div6}{RGB}{69,117,180}

\definecolor{RdYlBu7div1}{RGB}{215,48,39}
\definecolor{RdYlBu7div2}{RGB}{252,141,89}
\definecolor{RdYlBu7div3}{RGB}{254,224,144}
\definecolor{RdYlBu7div4}{RGB}{255,255,191}
\definecolor{RdYlBu7div5}{RGB}{224,243,248}
\definecolor{RdYlBu7div6}{RGB}{145,191,219}
\definecolor{RdYlBu7div7}{RGB}{69,117,180}

\definecolor{RdYlBu8div1}{RGB}{215,48,39}
\definecolor{RdYlBu8div2}{RGB}{244,109,67}
\definecolor{RdYlBu8div3}{RGB}{253,174,97}
\definecolor{RdYlBu8div4}{RGB}{254,224,144}
\definecolor{RdYlBu8div5}{RGB}{224,243,248}
\definecolor{RdYlBu8div6}{RGB}{171,217,233}
\definecolor{RdYlBu8div7}{RGB}{116,173,209}
\definecolor{RdYlBu8div8}{RGB}{69,117,180}

\definecolor{RdYlBu9div1}{RGB}{215,48,39}
\definecolor{RdYlBu9div2}{RGB}{244,109,67}
\definecolor{RdYlBu9div3}{RGB}{253,174,97}
\definecolor{RdYlBu9div4}{RGB}{254,224,144}
\definecolor{RdYlBu9div5}{RGB}{255,255,191}
\definecolor{RdYlBu9div6}{RGB}{224,243,248}
\definecolor{RdYlBu9div7}{RGB}{171,217,233}
\definecolor{RdYlBu9div8}{RGB}{116,173,209}
\definecolor{RdYlBu9div9}{RGB}{69,117,180}

\definecolor{RdYlBu10div1}{RGB}{165,0,38}
\definecolor{RdYlBu10div2}{RGB}{215,48,39}
\definecolor{RdYlBu10div3}{RGB}{244,109,67}
\definecolor{RdYlBu10div4}{RGB}{253,174,97}
\definecolor{RdYlBu10div5}{RGB}{254,224,144}
\definecolor{RdYlBu10div6}{RGB}{224,243,248}
\definecolor{RdYlBu10div7}{RGB}{171,217,233}
\definecolor{RdYlBu10div8}{RGB}{116,173,209}
\definecolor{RdYlBu10div9}{RGB}{69,117,180}
\definecolor{RdYlBu10div10}{RGB}{49,54,149}


\definecolor{RdYlGn3div1}{RGB}{252,141,89}
\definecolor{RdYlGn3div2}{RGB}{255,255,191}
\definecolor{RdYlGn3div3}{RGB}{145,207,96}

\definecolor{RdYlGn4div1}{RGB}{215,25,28}
\definecolor{RdYlGn4div2}{RGB}{253,174,97}
\definecolor{RdYlGn4div3}{RGB}{166,217,106}
\definecolor{RdYlGn4div4}{RGB}{26,150,65}

\definecolor{RdYlGn5div1}{RGB}{215,25,28}
\definecolor{RdYlGn5div2}{RGB}{253,174,97}
\definecolor{RdYlGn5div3}{RGB}{255,255,191}
\definecolor{RdYlGn5div4}{RGB}{166,217,106}
\definecolor{RdYlGn5div5}{RGB}{26,150,65}

\definecolor{RdYlGn6div1}{RGB}{215,48,39}
\definecolor{RdYlGn6div2}{RGB}{252,141,89}
\definecolor{RdYlGn6div3}{RGB}{254,224,139}
\definecolor{RdYlGn6div4}{RGB}{217,239,139}
\definecolor{RdYlGn6div5}{RGB}{145,207,96}
\definecolor{RdYlGn6div6}{RGB}{26,152,80}

\definecolor{RdYlGn7div1}{RGB}{215,48,39}
\definecolor{RdYlGn7div2}{RGB}{252,141,89}
\definecolor{RdYlGn7div3}{RGB}{254,224,139}
\definecolor{RdYlGn7div4}{RGB}{255,255,191}
\definecolor{RdYlGn7div5}{RGB}{217,239,139}
\definecolor{RdYlGn7div6}{RGB}{145,207,96}
\definecolor{RdYlGn7div7}{RGB}{26,152,80}

\definecolor{RdYlGn8div1}{RGB}{215,48,39}
\definecolor{RdYlGn8div2}{RGB}{244,109,67}
\definecolor{RdYlGn8div3}{RGB}{253,174,97}
\definecolor{RdYlGn8div4}{RGB}{254,224,139}
\definecolor{RdYlGn8div5}{RGB}{217,239,139}
\definecolor{RdYlGn8div6}{RGB}{166,217,106}
\definecolor{RdYlGn8div7}{RGB}{102,189,99}
\definecolor{RdYlGn8div8}{RGB}{26,152,80}

\definecolor{RdYlGn9div1}{RGB}{215,48,39}
\definecolor{RdYlGn9div2}{RGB}{244,109,67}
\definecolor{RdYlGn9div3}{RGB}{253,174,97}
\definecolor{RdYlGn9div4}{RGB}{254,224,139}
\definecolor{RdYlGn9div5}{RGB}{255,255,191}
\definecolor{RdYlGn9div6}{RGB}{217,239,139}
\definecolor{RdYlGn9div7}{RGB}{166,217,106}
\definecolor{RdYlGn9div8}{RGB}{102,189,99}
\definecolor{RdYlGn9div9}{RGB}{26,152,80}

\definecolor{RdYlGn10div1}{RGB}{165,0,38}
\definecolor{RdYlGn10div2}{RGB}{215,48,39}
\definecolor{RdYlGn10div3}{RGB}{244,109,67}
\definecolor{RdYlGn10div4}{RGB}{253,174,97}
\definecolor{RdYlGn10div5}{RGB}{254,224,139}
\definecolor{RdYlGn10div6}{RGB}{217,239,139}
\definecolor{RdYlGn10div7}{RGB}{166,217,106}
\definecolor{RdYlGn10div8}{RGB}{102,189,99}
\definecolor{RdYlGn10div9}{RGB}{26,152,80}
\definecolor{RdYlGn10div10}{RGB}{0,104,55}

\definecolor{RdYlGn11div1}{RGB}{165,0,38}
\definecolor{RdYlGn11div2}{RGB}{215,48,39}
\definecolor{RdYlGn11div3}{RGB}{244,109,67}
\definecolor{RdYlGn11div4}{RGB}{253,174,97}
\definecolor{RdYlGn11div5}{RGB}{254,224,139}
\definecolor{RdYlGn11div6}{RGB}{255,255,191}
\definecolor{RdYlGn11div7}{RGB}{217,239,139}
\definecolor{RdYlGn11div8}{RGB}{166,217,106}
\definecolor{RdYlGn11div9}{RGB}{102,189,99}
\definecolor{RdYlGn11div10}{RGB}{26,152,80}
\definecolor{RdYlGn11div11}{RGB}{0,104,55}
%END EDIT

\definecolor{Set14qual1}{RGB}{228,26,28}
\definecolor{Set14qual2}{RGB}{55,126,184}
\definecolor{Set14qual3}{RGB}{77,175,74}
\definecolor{Set14qual4}{RGB}{152,78,163}
\definecolor{Set16qual1}{RGB}{228,26,28}
\definecolor{Set16qual2}{RGB}{55,126,184}
\definecolor{Set16qual3}{RGB}{77,175,74}
\definecolor{Set16qual4}{RGB}{152,78,163}
\definecolor{Set16qual5}{RGB}{255,127,0}
\definecolor{Set16qual6}{RGB}{255,255,51}
\definecolor{Set18qual1}{RGB}{228,26,28}
\definecolor{Set18qual2}{RGB}{55,126,184}
\definecolor{Set18qual3}{RGB}{77,175,74}
\definecolor{Set18qual4}{RGB}{152,78,163}
\definecolor{Set18qual5}{RGB}{255,127,0}
\definecolor{Set18qual6}{RGB}{255,255,51}
\definecolor{Set18qual7}{RGB}{166,86,40}
\definecolor{Set18qual8}{RGB}{247,129,191}
\definecolor{Set23qual1}{RGB}{102,194,165}
\definecolor{Set23qual2}{RGB}{252,141,98}
\definecolor{Set23qual3}{RGB}{141,160,203}
\definecolor{Set25qual1}{RGB}{102,194,165}
\definecolor{Set25qual2}{RGB}{252,141,98}
\definecolor{Set25qual3}{RGB}{141,160,203}
\definecolor{Set25qual4}{RGB}{231,138,195}
\definecolor{Set25qual5}{RGB}{166,216,84}
\definecolor{Set27qual1}{RGB}{102,194,165}
\definecolor{Set27qual2}{RGB}{252,141,98}
\definecolor{Set27qual3}{RGB}{141,160,203}
\definecolor{Set27qual4}{RGB}{231,138,195}
\definecolor{Set27qual5}{RGB}{166,216,84}
\definecolor{Set27qual6}{RGB}{255,217,47}
\definecolor{Set27qual7}{RGB}{229,196,148}
\definecolor{Set33qual1}{RGB}{141,211,199}
\definecolor{Set33qual2}{RGB}{255,255,179}
\definecolor{Set33qual3}{RGB}{190,186,218}
\definecolor{Set35qual1}{RGB}{141,211,199}
\definecolor{Set35qual2}{RGB}{255,255,179}
\definecolor{Set35qual3}{RGB}{190,186,218}
\definecolor{Set35qual4}{RGB}{251,128,114}
\definecolor{Set35qual5}{RGB}{128,177,211}
\definecolor{Set37qual1}{RGB}{141,211,199}
\definecolor{Set37qual2}{RGB}{255,255,179}
\definecolor{Set37qual3}{RGB}{190,186,218}
\definecolor{Set37qual4}{RGB}{251,128,114}
\definecolor{Set37qual5}{RGB}{128,177,211}
\definecolor{Set37qual6}{RGB}{253,180,98}
\definecolor{Set37qual7}{RGB}{179,222,105}
\definecolor{Set39qual1}{RGB}{141,211,199}
\definecolor{Set39qual2}{RGB}{255,255,179}
\definecolor{Set39qual3}{RGB}{190,186,218}
\definecolor{Set39qual4}{RGB}{251,128,114}
\definecolor{Set39qual5}{RGB}{128,177,211}
\definecolor{Set39qual6}{RGB}{253,180,98}
\definecolor{Set39qual7}{RGB}{179,222,105}
\definecolor{Set39qual8}{RGB}{252,205,229}
\definecolor{Set39qual9}{RGB}{217,217,217}
\definecolor{Set311qual1}{RGB}{141,211,199}
\definecolor{Set311qual2}{RGB}{255,255,179}
\definecolor{Set311qual3}{RGB}{190,186,218}
\definecolor{Set311qual4}{RGB}{251,128,114}
\definecolor{Set311qual5}{RGB}{128,177,211}
\definecolor{Set311qual6}{RGB}{253,180,98}
\definecolor{Set311qual7}{RGB}{179,222,105}
\definecolor{Set311qual8}{RGB}{252,205,229}
\definecolor{Set311qual9}{RGB}{217,217,217}
\definecolor{Set311qual10}{RGB}{188,128,189}
\definecolor{Set311qual11}{RGB}{204,235,197}
\definecolor{Spectral3div1}{RGB}{252,141,89}
\definecolor{Spectral3div2}{RGB}{255,255,191}
\definecolor{Spectral3div3}{RGB}{153,213,148}
\definecolor{Spectral5div1}{RGB}{215,25,28}
\definecolor{Spectral5div2}{RGB}{253,174,97}
\definecolor{Spectral5div3}{RGB}{255,255,191}
\definecolor{Spectral5div4}{RGB}{171,221,164}
\definecolor{Spectral5div5}{RGB}{43,131,186}
\definecolor{Spectral7div1}{RGB}{213,62,79}
\definecolor{Spectral7div2}{RGB}{252,141,89}
\definecolor{Spectral7div3}{RGB}{254,224,139}
\definecolor{Spectral7div4}{RGB}{255,255,191}
\definecolor{Spectral7div5}{RGB}{230,245,152}
\definecolor{Spectral7div6}{RGB}{153,213,148}
\definecolor{Spectral7div7}{RGB}{50,136,189}
\definecolor{Spectral9div1}{RGB}{213,62,79}
\definecolor{Spectral9div2}{RGB}{244,109,67}
\definecolor{Spectral9div3}{RGB}{253,174,97}
\definecolor{Spectral9div4}{RGB}{254,224,139}
\definecolor{Spectral9div5}{RGB}{255,255,191}
\definecolor{Spectral9div6}{RGB}{230,245,152}
\definecolor{Spectral9div7}{RGB}{171,221,164}
\definecolor{Spectral9div8}{RGB}{102,194,165}
\definecolor{Spectral9div9}{RGB}{50,136,189}
\definecolor{Spectral11div1}{RGB}{158,1,66}
\definecolor{Spectral11div2}{RGB}{213,62,79}
\definecolor{Spectral11div3}{RGB}{244,109,67}
\definecolor{Spectral11div4}{RGB}{253,174,97}
\definecolor{Spectral11div5}{RGB}{254,224,139}
\definecolor{Spectral11div6}{RGB}{255,255,191}
\definecolor{Spectral11div7}{RGB}{230,245,152}
\definecolor{Spectral11div8}{RGB}{171,221,164}
\definecolor{Spectral11div9}{RGB}{102,194,165}
\definecolor{Spectral11div10}{RGB}{50,136,189}
\definecolor{Spectral11div11}{RGB}{94,79,162}
\definecolor{YlGn4seq1}{RGB}{255,255,204}
\definecolor{YlGn4seq2}{RGB}{194,230,153}
\definecolor{YlGn4seq3}{RGB}{120,198,121}
\definecolor{YlGn4seq4}{RGB}{35,132,67}
\definecolor{YlGn6seq1}{RGB}{255,255,204}
\definecolor{YlGn6seq2}{RGB}{217,240,163}
\definecolor{YlGn6seq3}{RGB}{173,221,142}
\definecolor{YlGn6seq4}{RGB}{120,198,121}
\definecolor{YlGn6seq5}{RGB}{49,163,84}
\definecolor{YlGn6seq6}{RGB}{0,104,55}
\definecolor{YlGn8seq1}{RGB}{255,255,229}
\definecolor{YlGn8seq2}{RGB}{247,252,185}
\definecolor{YlGn8seq3}{RGB}{217,240,163}
\definecolor{YlGn8seq4}{RGB}{173,221,142}
\definecolor{YlGn8seq5}{RGB}{120,198,121}
\definecolor{YlGn8seq6}{RGB}{65,171,93}
\definecolor{YlGn8seq7}{RGB}{35,132,67}
\definecolor{YlGn8seq8}{RGB}{0,90,50}
\definecolor{YlGnBu3seq1}{RGB}{237,248,177}
\definecolor{YlGnBu3seq2}{RGB}{127,205,187}
\definecolor{YlGnBu3seq3}{RGB}{44,127,184}
\definecolor{YlGnBu5seq1}{RGB}{255,255,204}
\definecolor{YlGnBu5seq2}{RGB}{161,218,180}
\definecolor{YlGnBu5seq3}{RGB}{65,182,196}
\definecolor{YlGnBu5seq4}{RGB}{44,127,184}
\definecolor{YlGnBu5seq5}{RGB}{37,52,148}
\definecolor{YlGnBu7seq1}{RGB}{255,255,204}
\definecolor{YlGnBu7seq2}{RGB}{199,233,180}
\definecolor{YlGnBu7seq3}{RGB}{127,205,187}
\definecolor{YlGnBu7seq4}{RGB}{65,182,196}
\definecolor{YlGnBu7seq5}{RGB}{29,145,192}
\definecolor{YlGnBu7seq6}{RGB}{34,94,168}
\definecolor{YlGnBu7seq7}{RGB}{12,44,132}
\definecolor{YlGnBu9seq1}{RGB}{255,255,217}
\definecolor{YlGnBu9seq2}{RGB}{237,248,177}
\definecolor{YlGnBu9seq3}{RGB}{199,233,180}
\definecolor{YlGnBu9seq4}{RGB}{127,205,187}
\definecolor{YlGnBu9seq5}{RGB}{65,182,196}
\definecolor{YlGnBu9seq6}{RGB}{29,145,192}
\definecolor{YlGnBu9seq7}{RGB}{34,94,168}
\definecolor{YlGnBu9seq8}{RGB}{37,52,148}
\definecolor{YlGnBu9seq9}{RGB}{8,29,88}
\definecolor{YlOrBr4seq1}{RGB}{255,255,212}
\definecolor{YlOrBr4seq2}{RGB}{254,217,142}
\definecolor{YlOrBr4seq3}{RGB}{254,153,41}
\definecolor{YlOrBr4seq4}{RGB}{204,76,2}
\definecolor{YlOrBr6seq1}{RGB}{255,255,212}
\definecolor{YlOrBr6seq2}{RGB}{254,227,145}
\definecolor{YlOrBr6seq3}{RGB}{254,196,79}
\definecolor{YlOrBr6seq4}{RGB}{254,153,41}
\definecolor{YlOrBr6seq5}{RGB}{217,95,14}
\definecolor{YlOrBr6seq6}{RGB}{153,52,4}
\definecolor{YlOrBr8seq1}{RGB}{255,255,229}
\definecolor{YlOrBr8seq2}{RGB}{255,247,188}
\definecolor{YlOrBr8seq3}{RGB}{254,227,145}
\definecolor{YlOrBr8seq4}{RGB}{254,196,79}
\definecolor{YlOrBr8seq5}{RGB}{254,153,41}
\definecolor{YlOrBr8seq6}{RGB}{236,112,20}
\definecolor{YlOrBr8seq7}{RGB}{204,76,2}
\definecolor{YlOrBr8seq8}{RGB}{140,45,4}
\definecolor{YlOrRd3seq1}{RGB}{255,237,160}
\definecolor{YlOrRd3seq2}{RGB}{254,178,76}
\definecolor{YlOrRd3seq3}{RGB}{240,59,32}
\definecolor{YlOrRd5seq1}{RGB}{255,255,178}
\definecolor{YlOrRd5seq2}{RGB}{254,204,92}
\definecolor{YlOrRd5seq3}{RGB}{253,141,60}
\definecolor{YlOrRd5seq4}{RGB}{240,59,32}
\definecolor{YlOrRd5seq5}{RGB}{189,0,38}
\definecolor{YlOrRd7seq1}{RGB}{255,255,178}
\definecolor{YlOrRd7seq2}{RGB}{254,217,118}
\definecolor{YlOrRd7seq3}{RGB}{254,178,76}
\definecolor{YlOrRd7seq4}{RGB}{253,141,60}
\definecolor{YlOrRd7seq5}{RGB}{252,78,42}
\definecolor{YlOrRd7seq6}{RGB}{227,26,28}
\definecolor{YlOrRd7seq7}{RGB}{177,0,38}
\definecolor{YlOrRd9seq1}{RGB}{255,255,204}
\definecolor{YlOrRd9seq2}{RGB}{255,237,160}
\definecolor{YlOrRd9seq3}{RGB}{254,217,118}
\definecolor{YlOrRd9seq4}{RGB}{254,178,76}
\definecolor{YlOrRd9seq5}{RGB}{253,141,60}
\definecolor{YlOrRd9seq6}{RGB}{252,78,42}
\definecolor{YlOrRd9seq7}{RGB}{227,26,28}
\definecolor{YlOrRd9seq8}{RGB}{189,0,38}
\definecolor{YlOrRd9seq9}{RGB}{128,0,38}
\pgfplotsset{/pgfplots/colormap={Accent3qual}{
	rgb255=(127,201,127) 
	rgb255=(190,174,212) 
	rgb255=(253,192,134) 
}}
\pgfplotsset{/pgfplots/colormap={Accent5qual}{
	rgb255=(127,201,127) 
	rgb255=(190,174,212) 
	rgb255=(253,192,134) 
	rgb255=(255,255,153) 
	rgb255=(56,108,176) 
}}
\pgfplotsset{/pgfplots/colormap={Accent7qual}{
	rgb255=(127,201,127) 
	rgb255=(190,174,212) 
	rgb255=(253,192,134) 
	rgb255=(255,255,153) 
	rgb255=(56,108,176) 
	rgb255=(240,2,127) 
	rgb255=(191,91,23) 
}}

%EDIT: Added number of classes
\pgfplotsset{/pgfplots/colormap={BluesSeq}{
	rgb255=(239,243,255)
	rgb255=(189,215,231)
	rgb255=(107,174,214)
	rgb255=(49,130,189)
	rgb255=(8,81,156)
}}

\pgfplotsset{/pgfplots/colormap={Blues3seq}{
	rgb255=(222,235,247) 
	rgb255=(158,202,225) 
	rgb255=(49,130,189) 
}}
\pgfplotsset{/pgfplots/colormap={Blues5seq}{
	rgb255=(239,243,255) 
	rgb255=(189,215,231) 
	rgb255=(107,174,214) 
	rgb255=(49,130,189) 
	rgb255=(8,81,156) 
}}
\pgfplotsset{/pgfplots/colormap={Blues7seq}{
	rgb255=(239,243,255) 
	rgb255=(198,219,239) 
	rgb255=(158,202,225) 
	rgb255=(107,174,214) 
	rgb255=(66,146,198) 
	rgb255=(33,113,181) 
	rgb255=(8,69,148) 
}}
\pgfplotsset{/pgfplots/colormap={Blues9seq}{
	rgb255=(247,251,255) 
	rgb255=(222,235,247) 
	rgb255=(198,219,239) 
	rgb255=(158,202,225) 
	rgb255=(107,174,214) 
	rgb255=(66,146,198) 
	rgb255=(33,113,181) 
	rgb255=(8,81,156) 
	rgb255=(8,48,107) 
}}
%END EDIT

\pgfplotsset{/pgfplots/colormap={BrBG4div}{
	rgb255=(166,97,26) 
	rgb255=(223,194,125) 
	rgb255=(128,205,193) 
	rgb255=(1,133,113) 
}}
\pgfplotsset{/pgfplots/colormap={BrBG6div}{
	rgb255=(140,81,10) 
	rgb255=(216,179,101) 
	rgb255=(246,232,195) 
	rgb255=(199,234,229) 
	rgb255=(90,180,172) 
	rgb255=(1,102,94) 
}}
\pgfplotsset{/pgfplots/colormap={BrBG8div}{
	rgb255=(140,81,10) 
	rgb255=(191,129,45) 
	rgb255=(223,194,125) 
	rgb255=(246,232,195) 
	rgb255=(199,234,229) 
	rgb255=(128,205,193) 
	rgb255=(53,151,143) 
	rgb255=(1,102,94) 
}}
\pgfplotsset{/pgfplots/colormap={BrBG10div}{
	rgb255=(84,48,5) 
	rgb255=(140,81,10) 
	rgb255=(191,129,45) 
	rgb255=(223,194,125) 
	rgb255=(246,232,195) 
	rgb255=(199,234,229) 
	rgb255=(128,205,193) 
	rgb255=(53,151,143) 
	rgb255=(1,102,94) 
	rgb255=(0,60,48) 
}}
\pgfplotsset{/pgfplots/colormap={BuGn3seq}{
	rgb255=(229,245,249) 
	rgb255=(153,216,201) 
	rgb255=(44,162,95) 
}}
\pgfplotsset{/pgfplots/colormap={BuGn5seq}{
	rgb255=(237,248,251) 
	rgb255=(178,226,226) 
	rgb255=(102,194,164) 
	rgb255=(44,162,95) 
	rgb255=(0,109,44) 
}}
\pgfplotsset{/pgfplots/colormap={BuGn7seq}{
	rgb255=(237,248,251) 
	rgb255=(204,236,230) 
	rgb255=(153,216,201) 
	rgb255=(102,194,164) 
	rgb255=(65,174,118) 
	rgb255=(35,139,69) 
	rgb255=(0,88,36) 
}}
\pgfplotsset{/pgfplots/colormap={BuGn9seq}{
	rgb255=(247,252,253) 
	rgb255=(229,245,249) 
	rgb255=(204,236,230) 
	rgb255=(153,216,201) 
	rgb255=(102,194,164) 
	rgb255=(65,174,118) 
	rgb255=(35,139,69) 
	rgb255=(0,109,44) 
	rgb255=(0,68,27) 
}}
\pgfplotsset{/pgfplots/colormap={BuPu4seq}{
	rgb255=(237,248,251) 
	rgb255=(179,205,227) 
	rgb255=(140,150,198) 
	rgb255=(136,65,157) 
}}
\pgfplotsset{/pgfplots/colormap={BuPu6seq}{
	rgb255=(237,248,251) 
	rgb255=(191,211,230) 
	rgb255=(158,188,218) 
	rgb255=(140,150,198) 
	rgb255=(136,86,167) 
	rgb255=(129,15,124) 
}}
\pgfplotsset{/pgfplots/colormap={BuPu8seq}{
	rgb255=(247,252,253) 
	rgb255=(224,236,244) 
	rgb255=(191,211,230) 
	rgb255=(158,188,218) 
	rgb255=(140,150,198) 
	rgb255=(140,107,177) 
	rgb255=(136,65,157) 
	rgb255=(110,1,107) 
}}
\pgfplotsset{/pgfplots/colormap={Dark23qual}{
	rgb255=(27,158,119) 
	rgb255=(217,95,2) 
	rgb255=(117,112,179) 
}}
\pgfplotsset{/pgfplots/colormap={Dark25qual}{
	rgb255=(27,158,119) 
	rgb255=(217,95,2) 
	rgb255=(117,112,179) 
	rgb255=(231,41,138) 
	rgb255=(102,166,30) 
}}
\pgfplotsset{/pgfplots/colormap={Dark27qual}{
	rgb255=(27,158,119) 
	rgb255=(217,95,2) 
	rgb255=(117,112,179) 
	rgb255=(231,41,138) 
	rgb255=(102,166,30) 
	rgb255=(230,171,2) 
	rgb255=(166,118,29) 
}}
\pgfplotsset{/pgfplots/colormap={GnBu3seq}{
	rgb255=(224,243,219) 
	rgb255=(168,221,181) 
	rgb255=(67,162,202) 
}}
\pgfplotsset{/pgfplots/colormap={GnBu5seq}{
	rgb255=(240,249,232) 
	rgb255=(186,228,188) 
	rgb255=(123,204,196) 
	rgb255=(67,162,202) 
	rgb255=(8,104,172) 
}}
\pgfplotsset{/pgfplots/colormap={GnBu7seq}{
	rgb255=(240,249,232) 
	rgb255=(204,235,197) 
	rgb255=(168,221,181) 
	rgb255=(123,204,196) 
	rgb255=(78,179,211) 
	rgb255=(43,140,190) 
	rgb255=(8,88,158) 
}}
\pgfplotsset{/pgfplots/colormap={GnBu9seq}{
	rgb255=(247,252,240) 
	rgb255=(224,243,219) 
	rgb255=(204,235,197) 
	rgb255=(168,221,181) 
	rgb255=(123,204,196) 
	rgb255=(78,179,211) 
	rgb255=(43,140,190) 
	rgb255=(8,104,172) 
	rgb255=(8,64,129) 
}}

%EDIT: Added number of classes
\pgfplotsset{/pgfplots/colormap={GreensSeq}{
	rgb255=(237,248,233)
	rgb255=(186,228,179)
	rgb255=(116,196,118)
	rgb255=(49,163,84)
	rgb255=(0,109,44)
}}

\pgfplotsset{/pgfplots/colormap={Greens3seq}{
	rgb255=(237,248,233)
	rgb255=(161,217,155)
	rgb255=(49,163,84)
}}
\pgfplotsset{/pgfplots/colormap={Greens4seq}{
	rgb255=(237,248,233) 
	rgb255=(186,228,179) 
	rgb255=(116,196,118) 
	rgb255=(35,139,69) 
}}
\pgfplotsset{/pgfplots/colormap={Greens6seq}{
	rgb255=(237,248,233) 
	rgb255=(199,233,192) 
	rgb255=(161,217,155) 
	rgb255=(116,196,118) 
	rgb255=(49,163,84) 
	rgb255=(0,109,44) 
}}
\pgfplotsset{/pgfplots/colormap={Greens8seq}{
	rgb255=(247,252,245) 
	rgb255=(229,245,224) 
	rgb255=(199,233,192) 
	rgb255=(161,217,155) 
	rgb255=(116,196,118) 
	rgb255=(65,171,93) 
	rgb255=(35,139,69) 
	rgb255=(0,90,50) 
}}
\pgfplotsset{/pgfplots/colormap={Greens9seq}{
	rgb255=(247,252,245)
	rgb255=(229,245,224)
	rgb255=(199,233,192)
	rgb255=(161,217,155)
	rgb255=(116,196,118)
	rgb255=(65,171,93)
	rgb255=(35,139,69)
	rgb255=(0,109,44)
	rgb255=(0,68,27)
}}
%END EDIT

\pgfplotsset{/pgfplots/colormap={Greys3seq}{
	rgb255=(240,240,240) 
	rgb255=(189,189,189) 
	rgb255=(99,99,99) 
}}
\pgfplotsset{/pgfplots/colormap={Greys5seq}{
	rgb255=(247,247,247) 
	rgb255=(204,204,204) 
	rgb255=(150,150,150) 
	rgb255=(99,99,99) 
	rgb255=(37,37,37) 
}}
\pgfplotsset{/pgfplots/colormap={Greys7seq}{
	rgb255=(247,247,247) 
	rgb255=(217,217,217) 
	rgb255=(189,189,189) 
	rgb255=(150,150,150) 
	rgb255=(115,115,115) 
	rgb255=(82,82,82) 
	rgb255=(37,37,37) 
}}
\pgfplotsset{/pgfplots/colormap={Greys9seq}{
	rgb255=(255,255,255) 
	rgb255=(240,240,240) 
	rgb255=(217,217,217) 
	rgb255=(189,189,189) 
	rgb255=(150,150,150) 
	rgb255=(115,115,115) 
	rgb255=(82,82,82) 
	rgb255=(37,37,37) 
	rgb255=(0,0,0) 
}}
\pgfplotsset{/pgfplots/colormap={Oranges4seq}{
	rgb255=(254,237,222) 
	rgb255=(253,190,133) 
	rgb255=(253,141,60) 
	rgb255=(217,71,1) 
}}
\pgfplotsset{/pgfplots/colormap={Oranges6seq}{
	rgb255=(254,237,222) 
	rgb255=(253,208,162) 
	rgb255=(253,174,107) 
	rgb255=(253,141,60) 
	rgb255=(230,85,13) 
	rgb255=(166,54,3) 
}}
\pgfplotsset{/pgfplots/colormap={Oranges8seq}{
	rgb255=(255,245,235) 
	rgb255=(254,230,206) 
	rgb255=(253,208,162) 
	rgb255=(253,174,107) 
	rgb255=(253,141,60) 
	rgb255=(241,105,19) 
	rgb255=(217,72,1) 
	rgb255=(140,45,4) 
}}
\pgfplotsset{/pgfplots/colormap={OrRd3seq}{
	rgb255=(254,232,200) 
	rgb255=(253,187,132) 
	rgb255=(227,74,51) 
}}
\pgfplotsset{/pgfplots/colormap={OrRd5seq}{
	rgb255=(254,240,217) 
	rgb255=(253,204,138) 
	rgb255=(252,141,89) 
	rgb255=(227,74,51) 
	rgb255=(179,0,0) 
}}
\pgfplotsset{/pgfplots/colormap={OrRd7seq}{
	rgb255=(254,240,217) 
	rgb255=(253,212,158) 
	rgb255=(253,187,132) 
	rgb255=(252,141,89) 
	rgb255=(239,101,72) 
	rgb255=(215,48,31) 
	rgb255=(153,0,0) 
}}
\pgfplotsset{/pgfplots/colormap={OrRd9seq}{
	rgb255=(255,247,236) 
	rgb255=(254,232,200) 
	rgb255=(253,212,158) 
	rgb255=(253,187,132) 
	rgb255=(252,141,89) 
	rgb255=(239,101,72) 
	rgb255=(215,48,31) 
	rgb255=(179,0,0) 
	rgb255=(127,0,0) 
}}
\pgfplotsset{/pgfplots/colormap={Paired4qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
}}
\pgfplotsset{/pgfplots/colormap={Paired6qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
	rgb255=(251,154,153) 
	rgb255=(227,26,28) 
}}
\pgfplotsset{/pgfplots/colormap={Paired8qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
	rgb255=(251,154,153) 
	rgb255=(227,26,28) 
	rgb255=(253,191,111) 
	rgb255=(255,127,0) 
}}
\pgfplotsset{/pgfplots/colormap={Paired10qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
	rgb255=(251,154,153) 
	rgb255=(227,26,28) 
	rgb255=(253,191,111) 
	rgb255=(255,127,0) 
	rgb255=(202,178,214) 
	rgb255=(106,61,154) 
}}
\pgfplotsset{/pgfplots/colormap={Paired12qual}{
	rgb255=(166,206,227) 
	rgb255=(31,120,180) 
	rgb255=(178,223,138) 
	rgb255=(51,160,44) 
	rgb255=(251,154,153) 
	rgb255=(227,26,28) 
	rgb255=(253,191,111) 
	rgb255=(255,127,0) 
	rgb255=(202,178,214) 
	rgb255=(106,61,154) 
	rgb255=(255,255,153) 
	rgb255=(177,89,40) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel14qual}{
	rgb255=(251,180,174) 
	rgb255=(179,205,227) 
	rgb255=(204,235,197) 
	rgb255=(222,203,228) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel16qual}{
	rgb255=(251,180,174) 
	rgb255=(179,205,227) 
	rgb255=(204,235,197) 
	rgb255=(222,203,228) 
	rgb255=(254,217,166) 
	rgb255=(255,255,204) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel18qual}{
	rgb255=(251,180,174) 
	rgb255=(179,205,227) 
	rgb255=(204,235,197) 
	rgb255=(222,203,228) 
	rgb255=(254,217,166) 
	rgb255=(255,255,204) 
	rgb255=(229,216,189) 
	rgb255=(253,218,236) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel23qual}{
	rgb255=(179,226,205) 
	rgb255=(253,205,172) 
	rgb255=(203,213,232) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel25qual}{
	rgb255=(179,226,205) 
	rgb255=(253,205,172) 
	rgb255=(203,213,232) 
	rgb255=(244,202,228) 
	rgb255=(230,245,201) 
}}
\pgfplotsset{/pgfplots/colormap={Pastel27qual}{
	rgb255=(179,226,205) 
	rgb255=(253,205,172) 
	rgb255=(203,213,232) 
	rgb255=(244,202,228) 
	rgb255=(230,245,201) 
	rgb255=(255,242,174) 
	rgb255=(241,226,204) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG3div}{
	rgb255=(233,163,201) 
	rgb255=(247,247,247) 
	rgb255=(161,215,106) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG5div}{
	rgb255=(208,28,139) 
	rgb255=(241,182,218) 
	rgb255=(247,247,247) 
	rgb255=(184,225,134) 
	rgb255=(77,172,38) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG7div}{
	rgb255=(197,27,125) 
	rgb255=(233,163,201) 
	rgb255=(253,224,239) 
	rgb255=(247,247,247) 
	rgb255=(230,245,208) 
	rgb255=(161,215,106) 
	rgb255=(77,146,33) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG9div}{
	rgb255=(197,27,125) 
	rgb255=(222,119,174) 
	rgb255=(241,182,218) 
	rgb255=(253,224,239) 
	rgb255=(247,247,247) 
	rgb255=(230,245,208) 
	rgb255=(184,225,134) 
	rgb255=(127,188,65) 
	rgb255=(77,146,33) 
}}
\pgfplotsset{/pgfplots/colormap={PiYG11div}{
	rgb255=(142,1,82) 
	rgb255=(197,27,125) 
	rgb255=(222,119,174) 
	rgb255=(241,182,218) 
	rgb255=(253,224,239) 
	rgb255=(247,247,247) 
	rgb255=(230,245,208) 
	rgb255=(184,225,134) 
	rgb255=(127,188,65) 
	rgb255=(77,146,33) 
	rgb255=(39,100,25) 
}}
\pgfplotsset{/pgfplots/colormap={PRGn4div}{
	rgb255=(123,50,148) 
	rgb255=(194,165,207) 
	rgb255=(166,219,160) 
	rgb255=(0,136,55) 
}}
\pgfplotsset{/pgfplots/colormap={PRGn6div}{
	rgb255=(118,42,131) 
	rgb255=(175,141,195) 
	rgb255=(231,212,232) 
	rgb255=(217,240,211) 
	rgb255=(127,191,123) 
	rgb255=(27,120,55) 
}}
\pgfplotsset{/pgfplots/colormap={PRGn8div}{
	rgb255=(118,42,131) 
	rgb255=(153,112,171) 
	rgb255=(194,165,207) 
	rgb255=(231,212,232) 
	rgb255=(217,240,211) 
	rgb255=(166,219,160) 
	rgb255=(90,174,97) 
	rgb255=(27,120,55) 
}}
\pgfplotsset{/pgfplots/colormap={PRGn10div}{
	rgb255=(64,0,75) 
	rgb255=(118,42,131) 
	rgb255=(153,112,171) 
	rgb255=(194,165,207) 
	rgb255=(231,212,232) 
	rgb255=(217,240,211) 
	rgb255=(166,219,160) 
	rgb255=(90,174,97) 
	rgb255=(27,120,55) 
	rgb255=(0,68,27) 
}}
\pgfplotsset{/pgfplots/colormap={PuBu3seq}{
	rgb255=(236,231,242) 
	rgb255=(166,189,219) 
	rgb255=(43,140,190) 
}}
\pgfplotsset{/pgfplots/colormap={PuBu5seq}{
	rgb255=(241,238,246) 
	rgb255=(189,201,225) 
	rgb255=(116,169,207) 
	rgb255=(43,140,190) 
	rgb255=(4,90,141) 
}}
\pgfplotsset{/pgfplots/colormap={PuBu7seq}{
	rgb255=(241,238,246) 
	rgb255=(208,209,230) 
	rgb255=(166,189,219) 
	rgb255=(116,169,207) 
	rgb255=(54,144,192) 
	rgb255=(5,112,176) 
	rgb255=(3,78,123) 
}}
\pgfplotsset{/pgfplots/colormap={PuBu9seq}{
	rgb255=(255,247,251) 
	rgb255=(236,231,242) 
	rgb255=(208,209,230) 
	rgb255=(166,189,219) 
	rgb255=(116,169,207) 
	rgb255=(54,144,192) 
	rgb255=(5,112,176) 
	rgb255=(4,90,141) 
	rgb255=(2,56,88) 
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn4seq}{
	rgb255=(246,239,247) 
	rgb255=(189,201,225) 
	rgb255=(103,169,207) 
	rgb255=(2,129,138) 
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn6seq}{
	rgb255=(246,239,247) 
	rgb255=(208,209,230) 
	rgb255=(166,189,219) 
	rgb255=(103,169,207) 
	rgb255=(28,144,153) 
	rgb255=(1,108,89) 
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn8seq}{
	rgb255=(255,247,251) 
	rgb255=(236,226,240) 
	rgb255=(208,209,230) 
	rgb255=(166,189,219) 
	rgb255=(103,169,207) 
	rgb255=(54,144,192) 
	rgb255=(2,129,138) 
	rgb255=(1,100,80) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr3div}{
	rgb255=(241,163,64) 
	rgb255=(247,247,247) 
	rgb255=(153,142,195) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr5div}{
	rgb255=(230,97,1) 
	rgb255=(253,184,99) 
	rgb255=(247,247,247) 
	rgb255=(178,171,210) 
	rgb255=(94,60,153) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr7div}{
	rgb255=(179,88,6) 
	rgb255=(241,163,64) 
	rgb255=(254,224,182) 
	rgb255=(247,247,247) 
	rgb255=(216,218,235) 
	rgb255=(153,142,195) 
	rgb255=(84,39,136) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr9div}{
	rgb255=(179,88,6) 
	rgb255=(224,130,20) 
	rgb255=(253,184,99) 
	rgb255=(254,224,182) 
	rgb255=(247,247,247) 
	rgb255=(216,218,235) 
	rgb255=(178,171,210) 
	rgb255=(128,115,172) 
	rgb255=(84,39,136) 
}}
\pgfplotsset{/pgfplots/colormap={PuOr11div}{
	rgb255=(127,59,8) 
	rgb255=(179,88,6) 
	rgb255=(224,130,20) 
	rgb255=(253,184,99) 
	rgb255=(254,224,182) 
	rgb255=(247,247,247) 
	rgb255=(216,218,235) 
	rgb255=(178,171,210) 
	rgb255=(128,115,172) 
	rgb255=(84,39,136) 
	rgb255=(45,0,75) 
}}
\pgfplotsset{/pgfplots/colormap={PuRd4seq}{
	rgb255=(241,238,246) 
	rgb255=(215,181,216) 
	rgb255=(223,101,176) 
	rgb255=(206,18,86) 
}}
\pgfplotsset{/pgfplots/colormap={PuRd6seq}{
	rgb255=(241,238,246) 
	rgb255=(212,185,218) 
	rgb255=(201,148,199) 
	rgb255=(223,101,176) 
	rgb255=(221,28,119) 
	rgb255=(152,0,67) 
}}
\pgfplotsset{/pgfplots/colormap={PuRd8seq}{
	rgb255=(247,244,249) 
	rgb255=(231,225,239) 
	rgb255=(212,185,218) 
	rgb255=(201,148,199) 
	rgb255=(223,101,176) 
	rgb255=(231,41,138) 
	rgb255=(206,18,86) 
	rgb255=(145,0,63) 
}}
\pgfplotsset{/pgfplots/colormap={Purples3seq}{
	rgb255=(239,237,245) 
	rgb255=(188,189,220) 
	rgb255=(117,107,177) 
}}
\pgfplotsset{/pgfplots/colormap={Purples5seq}{
	rgb255=(242,240,247) 
	rgb255=(203,201,226) 
	rgb255=(158,154,200) 
	rgb255=(117,107,177) 
	rgb255=(84,39,143) 
}}
\pgfplotsset{/pgfplots/colormap={Purples7seq}{
	rgb255=(242,240,247) 
	rgb255=(218,218,235) 
	rgb255=(188,189,220) 
	rgb255=(158,154,200) 
	rgb255=(128,125,186) 
	rgb255=(106,81,163) 
	rgb255=(74,20,134) 
}}
\pgfplotsset{/pgfplots/colormap={Purples9seq}{
	rgb255=(252,251,253) 
	rgb255=(239,237,245) 
	rgb255=(218,218,235) 
	rgb255=(188,189,220) 
	rgb255=(158,154,200) 
	rgb255=(128,125,186) 
	rgb255=(106,81,163) 
	rgb255=(84,39,143) 
	rgb255=(63,0,125) 
}}
\pgfplotsset{/pgfplots/colormap={RdBu4div}{
	rgb255=(202,0,32) 
	rgb255=(244,165,130) 
	rgb255=(146,197,222) 
	rgb255=(5,113,176) 
}}
\pgfplotsset{/pgfplots/colormap={RdBu6div}{
	rgb255=(178,24,43) 
	rgb255=(239,138,98) 
	rgb255=(253,219,199) 
	rgb255=(209,229,240) 
	rgb255=(103,169,207) 
	rgb255=(33,102,172) 
}}
\pgfplotsset{/pgfplots/colormap={RdBu8div}{
	rgb255=(178,24,43) 
	rgb255=(214,96,77) 
	rgb255=(244,165,130) 
	rgb255=(253,219,199) 
	rgb255=(209,229,240) 
	rgb255=(146,197,222) 
	rgb255=(67,147,195) 
	rgb255=(33,102,172) 
}}
\pgfplotsset{/pgfplots/colormap={RdBu10div}{
	rgb255=(103,0,31) 
	rgb255=(178,24,43) 
	rgb255=(214,96,77) 
	rgb255=(244,165,130) 
	rgb255=(253,219,199) 
	rgb255=(209,229,240) 
	rgb255=(146,197,222) 
	rgb255=(67,147,195) 
	rgb255=(33,102,172) 
	rgb255=(5,48,97) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy3div}{
	rgb255=(239,138,98) 
	rgb255=(255,255,255) 
	rgb255=(153,153,153) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy5div}{
	rgb255=(202,0,32) 
	rgb255=(244,165,130) 
	rgb255=(255,255,255) 
	rgb255=(186,186,186) 
	rgb255=(64,64,64) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy7div}{
	rgb255=(178,24,43) 
	rgb255=(239,138,98) 
	rgb255=(253,219,199) 
	rgb255=(255,255,255) 
	rgb255=(224,224,224) 
	rgb255=(153,153,153) 
	rgb255=(77,77,77) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy9div}{
	rgb255=(178,24,43) 
	rgb255=(214,96,77) 
	rgb255=(244,165,130) 
	rgb255=(253,219,199) 
	rgb255=(255,255,255) 
	rgb255=(224,224,224) 
	rgb255=(186,186,186) 
	rgb255=(135,135,135) 
	rgb255=(77,77,77) 
}}
\pgfplotsset{/pgfplots/colormap={RdGy11div}{
	rgb255=(103,0,31) 
	rgb255=(178,24,43) 
	rgb255=(214,96,77) 
	rgb255=(244,165,130) 
	rgb255=(253,219,199) 
	rgb255=(255,255,255) 
	rgb255=(224,224,224) 
	rgb255=(186,186,186) 
	rgb255=(135,135,135) 
	rgb255=(77,77,77) 
	rgb255=(26,26,26) 
}}
\pgfplotsset{/pgfplots/colormap={RdPu4seq}{
	rgb255=(254,235,226) 
	rgb255=(251,180,185) 
	rgb255=(247,104,161) 
	rgb255=(174,1,126) 
}}
\pgfplotsset{/pgfplots/colormap={RdPu6seq}{
	rgb255=(254,235,226) 
	rgb255=(252,197,192) 
	rgb255=(250,159,181) 
	rgb255=(247,104,161) 
	rgb255=(197,27,138) 
	rgb255=(122,1,119) 
}}
\pgfplotsset{/pgfplots/colormap={RdPu8seq}{
	rgb255=(255,247,243) 
	rgb255=(253,224,221) 
	rgb255=(252,197,192) 
	rgb255=(250,159,181) 
	rgb255=(247,104,161) 
	rgb255=(221,52,151) 
	rgb255=(174,1,126) 
	rgb255=(122,1,119) 
}}
%EDIT: Added number of classes
\pgfplotsset{/pgfplots/colormap={RedsSeq}{
	rgb255=(254,229,217)
	rgb255=(252,174,145)
	rgb255=(251,106,74)
	rgb255=(222,45,38)
	rgb255=(165,15,21)
}}

\pgfplotsset{/pgfplots/colormap={Reds3seq}{
	rgb255=(254,224,210) 
	rgb255=(252,146,114) 
	rgb255=(222,45,38) 
}}
\pgfplotsset{/pgfplots/colormap={Reds5seq}{
	rgb255=(254,229,217) 
	rgb255=(252,174,145) 
	rgb255=(251,106,74) 
	rgb255=(222,45,38) 
	rgb255=(165,15,21) 
}}
\pgfplotsset{/pgfplots/colormap={Reds7seq}{
	rgb255=(254,229,217) 
	rgb255=(252,187,161) 
	rgb255=(252,146,114) 
	rgb255=(251,106,74) 
	rgb255=(239,59,44) 
	rgb255=(203,24,29) 
	rgb255=(153,0,13) 
}}
\pgfplotsset{/pgfplots/colormap={Reds9seq}{
	rgb255=(255,245,240) 
	rgb255=(254,224,210) 
	rgb255=(252,187,161) 
	rgb255=(252,146,114) 
	rgb255=(251,106,74) 
	rgb255=(239,59,44) 
	rgb255=(203,24,29) 
	rgb255=(165,15,21) 
	rgb255=(103,0,13) 
}}

\pgfplotsset{/pgfplots/colormap={RdYlBuSeq}{
	rgb255=(165,0,38) 
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,144) 
	rgb255=(224,243,248) 
	rgb255=(171,217,233) 
	rgb255=(116,173,209) 
	rgb255=(69,117,180) 
	rgb255=(49,54,149) 
}}

\pgfplotsset{/pgfplots/colormap={RdYlBu4div}{
	rgb255=(215,25,28) 
	rgb255=(253,174,97) 
	rgb255=(171,217,233) 
	rgb255=(44,123,182) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu6div}{
	rgb255=(215,48,39) 
	rgb255=(252,141,89) 
	rgb255=(254,224,144) 
	rgb255=(224,243,248) 
	rgb255=(145,191,219) 
	rgb255=(69,117,180) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu8div}{
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,144) 
	rgb255=(224,243,248) 
	rgb255=(171,217,233) 
	rgb255=(116,173,209) 
	rgb255=(69,117,180) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu10div}{
	rgb255=(165,0,38) 
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,144) 
	rgb255=(224,243,248) 
	rgb255=(171,217,233) 
	rgb255=(116,173,209) 
	rgb255=(69,117,180) 
	rgb255=(49,54,149) 
}}
%END EDIT

\pgfplotsset{/pgfplots/colormap={RdYlGn3div}{
	rgb255=(252,141,89) 
	rgb255=(255,255,191) 
	rgb255=(145,207,96) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn5div}{
	rgb255=(215,25,28) 
	rgb255=(253,174,97) 
	rgb255=(255,255,191) 
	rgb255=(166,217,106) 
	rgb255=(26,150,65) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn7div}{
	rgb255=(215,48,39) 
	rgb255=(252,141,89) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(217,239,139) 
	rgb255=(145,207,96) 
	rgb255=(26,152,80) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn9div}{
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(217,239,139) 
	rgb255=(166,217,106) 
	rgb255=(102,189,99) 
	rgb255=(26,152,80) 
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn11div}{
	rgb255=(165,0,38) 
	rgb255=(215,48,39) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(217,239,139) 
	rgb255=(166,217,106) 
	rgb255=(102,189,99) 
	rgb255=(26,152,80) 
	rgb255=(0,104,55) 
}}
\pgfplotsset{/pgfplots/colormap={Set14qual}{
	rgb255=(228,26,28) 
	rgb255=(55,126,184) 
	rgb255=(77,175,74) 
	rgb255=(152,78,163) 
}}
\pgfplotsset{/pgfplots/colormap={Set16qual}{
	rgb255=(228,26,28) 
	rgb255=(55,126,184) 
	rgb255=(77,175,74) 
	rgb255=(152,78,163) 
	rgb255=(255,127,0) 
	rgb255=(255,255,51) 
}}
\pgfplotsset{/pgfplots/colormap={Set18qual}{
	rgb255=(228,26,28) 
	rgb255=(55,126,184) 
	rgb255=(77,175,74) 
	rgb255=(152,78,163) 
	rgb255=(255,127,0) 
	rgb255=(255,255,51) 
	rgb255=(166,86,40) 
	rgb255=(247,129,191) 
}}
\pgfplotsset{/pgfplots/colormap={Set23qual}{
	rgb255=(102,194,165) 
	rgb255=(252,141,98) 
	rgb255=(141,160,203) 
}}
\pgfplotsset{/pgfplots/colormap={Set25qual}{
	rgb255=(102,194,165) 
	rgb255=(252,141,98) 
	rgb255=(141,160,203) 
	rgb255=(231,138,195) 
	rgb255=(166,216,84) 
}}
\pgfplotsset{/pgfplots/colormap={Set27qual}{
	rgb255=(102,194,165) 
	rgb255=(252,141,98) 
	rgb255=(141,160,203) 
	rgb255=(231,138,195) 
	rgb255=(166,216,84) 
	rgb255=(255,217,47) 
	rgb255=(229,196,148) 
}}
\pgfplotsset{/pgfplots/colormap={Set33qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
}}
\pgfplotsset{/pgfplots/colormap={Set35qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
	rgb255=(251,128,114) 
	rgb255=(128,177,211) 
}}
\pgfplotsset{/pgfplots/colormap={Set37qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
	rgb255=(251,128,114) 
	rgb255=(128,177,211) 
	rgb255=(253,180,98) 
	rgb255=(179,222,105) 
}}
\pgfplotsset{/pgfplots/colormap={Set39qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
	rgb255=(251,128,114) 
	rgb255=(128,177,211) 
	rgb255=(253,180,98) 
	rgb255=(179,222,105) 
	rgb255=(252,205,229) 
	rgb255=(217,217,217) 
}}
\pgfplotsset{/pgfplots/colormap={Set311qual}{
	rgb255=(141,211,199) 
	rgb255=(255,255,179) 
	rgb255=(190,186,218) 
	rgb255=(251,128,114) 
	rgb255=(128,177,211) 
	rgb255=(253,180,98) 
	rgb255=(179,222,105) 
	rgb255=(252,205,229) 
	rgb255=(217,217,217) 
	rgb255=(188,128,189) 
	rgb255=(204,235,197) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral3div}{
	rgb255=(252,141,89) 
	rgb255=(255,255,191) 
	rgb255=(153,213,148) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral5div}{
	rgb255=(215,25,28) 
	rgb255=(253,174,97) 
	rgb255=(255,255,191) 
	rgb255=(171,221,164) 
	rgb255=(43,131,186) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral7div}{
	rgb255=(213,62,79) 
	rgb255=(252,141,89) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(230,245,152) 
	rgb255=(153,213,148) 
	rgb255=(50,136,189) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral9div}{
	rgb255=(213,62,79) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(230,245,152) 
	rgb255=(171,221,164) 
	rgb255=(102,194,165) 
	rgb255=(50,136,189) 
}}
\pgfplotsset{/pgfplots/colormap={Spectral11div}{
	rgb255=(158,1,66) 
	rgb255=(213,62,79) 
	rgb255=(244,109,67) 
	rgb255=(253,174,97) 
	rgb255=(254,224,139) 
	rgb255=(255,255,191) 
	rgb255=(230,245,152) 
	rgb255=(171,221,164) 
	rgb255=(102,194,165) 
	rgb255=(50,136,189) 
	rgb255=(94,79,162) 
}}
\pgfplotsset{/pgfplots/colormap={YlGn4seq}{
	rgb255=(255,255,204) 
	rgb255=(194,230,153) 
	rgb255=(120,198,121) 
	rgb255=(35,132,67) 
}}
\pgfplotsset{/pgfplots/colormap={YlGn6seq}{
	rgb255=(255,255,204) 
	rgb255=(217,240,163) 
	rgb255=(173,221,142) 
	rgb255=(120,198,121) 
	rgb255=(49,163,84) 
	rgb255=(0,104,55) 
}}
\pgfplotsset{/pgfplots/colormap={YlGn8seq}{
	rgb255=(255,255,229) 
	rgb255=(247,252,185) 
	rgb255=(217,240,163) 
	rgb255=(173,221,142) 
	rgb255=(120,198,121) 
	rgb255=(65,171,93) 
	rgb255=(35,132,67) 
	rgb255=(0,90,50) 
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu3seq}{
	rgb255=(237,248,177) 
	rgb255=(127,205,187) 
	rgb255=(44,127,184) 
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu5seq}{
	rgb255=(255,255,204) 
	rgb255=(161,218,180) 
	rgb255=(65,182,196) 
	rgb255=(44,127,184) 
	rgb255=(37,52,148) 
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu7seq}{
	rgb255=(255,255,204) 
	rgb255=(199,233,180) 
	rgb255=(127,205,187) 
	rgb255=(65,182,196) 
	rgb255=(29,145,192) 
	rgb255=(34,94,168) 
	rgb255=(12,44,132) 
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu9seq}{
	rgb255=(255,255,217) 
	rgb255=(237,248,177) 
	rgb255=(199,233,180) 
	rgb255=(127,205,187) 
	rgb255=(65,182,196) 
	rgb255=(29,145,192) 
	rgb255=(34,94,168) 
	rgb255=(37,52,148) 
	rgb255=(8,29,88) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr4seq}{
	rgb255=(255,255,212) 
	rgb255=(254,217,142) 
	rgb255=(254,153,41) 
	rgb255=(204,76,2) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr6seq}{
	rgb255=(255,255,212) 
	rgb255=(254,227,145) 
	rgb255=(254,196,79) 
	rgb255=(254,153,41) 
	rgb255=(217,95,14) 
	rgb255=(153,52,4) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr8seq}{
	rgb255=(255,255,229) 
	rgb255=(255,247,188) 
	rgb255=(254,227,145) 
	rgb255=(254,196,79) 
	rgb255=(254,153,41) 
	rgb255=(236,112,20) 
	rgb255=(204,76,2) 
	rgb255=(140,45,4) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd3seq}{
	rgb255=(255,237,160) 
	rgb255=(254,178,76) 
	rgb255=(240,59,32) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd5seq}{
	rgb255=(255,255,178) 
	rgb255=(254,204,92) 
	rgb255=(253,141,60) 
	rgb255=(240,59,32) 
	rgb255=(189,0,38) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd7seq}{
	rgb255=(255,255,178) 
	rgb255=(254,217,118) 
	rgb255=(254,178,76) 
	rgb255=(253,141,60) 
	rgb255=(252,78,42) 
	rgb255=(227,26,28) 
	rgb255=(177,0,38) 
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd9seq}{
	rgb255=(255,255,204) 
	rgb255=(255,237,160) 
	rgb255=(254,217,118) 
	rgb255=(254,178,76) 
	rgb255=(253,141,60) 
	rgb255=(252,78,42) 
	rgb255=(227,26,28) 
	rgb255=(189,0,38) 
	rgb255=(128,0,38) 
}}


==> styles/def-colors.tex <==
%-------------------------------------------------------------------
%university colors
%-------------------------------------------------------------------
\definecolor{AAUlogodarkblue}{RGB}{51,107,129}
\definecolor{AAUlogolightblue}{RGB}{70,153,194}
\definecolor{AAUdarkblue}{RGB}{10,54,96}
\definecolor{AAUviolett}{RGB}{84,63,145}
\definecolor{AAUgreen}{RGB}{128,167,51}
\definecolor{AAUyellow}{RGB}{239,213,34}
\definecolor{AAUtewi}{RGB}{122,20,112}
\definecolor{AAUwiwi}{RGB}{145,191,62}
\definecolor{AAUiff}{RGB}{184,34,49}
\definecolor{AAUkuwi}{RGB}{120,92,167}


==> styles/def-kinematics.tex <==
%-------------------------------------------------------------------
%kinematics definitions
%-------------------------------------------------------------------

\newcommand\angleaxis[2]{(\theta,\vn)_{#1\!#2}}
\newcommand\rotvec[2]{\vvph_{#1\!#2}}


\newcommand\dvch[0]{\dot{\vch}}
\newcommand\imquatvec[3]{\mathbf{#1}_{v,\!#2\!#3}}
\newcommand\realquat[3]{#1_{w,\!#2\!#3}}
%\newcommand\imquatvec[1]{\check{\mathbf{#1}}}
%\newcommand\imquatvec[1]{\overrightarrow{\mathbf{#1}}}
%\newcommand\imquatvecFrame[3]{\check{\mathbf{#1}}_{#2\!#3}}
\newcommand\skewImquatvecFrame[3]{\hat{\check{\mathbf{#1}}}_{#2\!#3}}

%\renewcommand\unitvec[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
%  \ifthenelse{\equal{#1}{\empty}}
%     {\ve_{#2}}
%     {{}_{#1}\ve_{#2}}
%}

\newcommand\unitvec[2]{{}_{#1}\ve_{#2}}

\newcommand\symdt[1]{\dot{#1}}
\newcommand\symddt[1]{\ddot{#1}}
\newcommand\symdddt[1]{\dddot{#1}}
\newcommand\symddddt[1]{\ddddot{#1}}
\newcommand\symest[1]{\hat{#1}}
\newcommand\symjoint[1]{\check{#1}}
\newcommand\symerr[1]{\widetilde{#1}}
\newcommand\symvec[1]{\vec{#1}}
\newcommand\symmeas[1]{#1{m}} %!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
\newcommand\symdiff[1]{\Delta #1}
\newcommand\symmean[1]{\mu_{#1}}
\newcommand\symmeanvec[1]{\symvec{\vmu}_{#1}}
\newcommand\symstd[1]{\sigma_{#1}}
\newcommand\symstdvec[1]{\symvec{\vsi}_{#1}}
\newcommand\symsubscript[1]{\mbox{\scriptsize $#1$}} %!!!!!!!!!!!!!!!!!!!!!!!!!!
%\newcommand\syminv[1]{{#1}^{$\scriptscriptstyle-\!1$}}
%\newcommand\symtranspose[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}

\newcommand\transhom[2]{\vT_{#1\!#2}}

%Filter
\newcommand\TransMatC{{\boldsymbol\vF}}
\newcommand\TransMatD{{\boldsymbol\Phi}}
\newcommand\TransMatSerD{{\boldsymbol{\mathcal{F}}}} % transition matrix series discrete
\newcommand\NoiseMatC{{\boldsymbol{\mathbf Q} }}
\newcommand\NoiseMatD{{\boldsymbol\Gamma}}
\newcommand\CovMatD{{\boldsymbol{\mathbf P} }}
\newcommand\CovMatC{{\boldsymbol{\mathbf P} }}
\newcommand\MeasNoiseMat{{\boldsymbol{\mathbf R} }}

%State vector
%\newcommand\State{\vX}
\newcommand\state{\vx}
\newcommand\statetranspose{\vx^\transpose} 		%transposed vector
\newcommand\statedt{\symdt{\vx}} 				%first time derivative
\newcommand\stateest{\symest{\vx}} 				%estimate
\newcommand\stateerr{\symerr{\vx}} 				%error
\newcommand\stateerrjoint{\symjoint{\symerr{\vx}}} 				%error-joint
\newcommand\stateestjoint{\symjoint{\symest{\vx}}} 				%error-joint
\newcommand\stateerrdt{\symdt{\symerr{\vx}}} 	%first time derivative of error
\newcommand\statediff{\symdiff{\vx}} 			%difference
\newcommand\statejoint{\symjoint{\vx}} 			%joint

%Control vector
\newcommand\ctrl{\vu}
\newcommand\ctrltranspose{\vu^\transpose} 		%transposed vector
\newcommand\ctrldt{\symdt{\vu}} 				%first time derivative
\newcommand\ctrlest{\symest{\vu}} 				%estimate
\newcommand\ctrlerr{\symerr{\vu}} 				%error
\newcommand\ctrldiff{\symdiff{\vu}} 			%difference

%Measurement vector
\newcommand\meas{\vz}
\newcommand\meastranspose{\vz^\transpose} 		%transposed vector
\newcommand\measdt{\symdt{\vz}} 				%first time derivative
\newcommand\measest{\symest{\vz}} 				%estimate
\newcommand\measerr{\symerr{\vz}} 				%error
\newcommand\measdiff{\symdiff{\vz}} 			%difference
\newcommand\measjoint{\symjoint{\vz}} 			%joint
\newcommand\measestjoint{\symjoint{\measest}} 			%joint est
\newcommand\measerrjoint{\symjoint{\measerr}} 			%joint est

%Residual vector
\newcommand\res{\vr}
\newcommand\restranspose{\vr^\transpose} 		%transposed vector
\newcommand\resdt{\symdt{\vr}} 				    %first time derivative
\newcommand\resest{\symest{\vr}} 				%estimate
\newcommand\reserr{\symerr{\vr}} 				%error
\newcommand\resdiff{\symdiff{\vr}} 			    %difference
\newcommand\resjoint{\symjoint{\vr}} 			%joint

\newcommand\referencentofrom[4]{{}_{#4}#1_{#2#3}}   % variable #1, to #2 from #3 in #4  e.g.: $\reference{\vp}{i}{w}{w}^\transpose$
\newcommand\referencevert[4]{{}_{#4}#1^{#2}_{#3}}   % variable #1, to #2 from #3 in #4  e.g.: ${\referenceold{\vp}{i}{w}{w}}^\transpose$
\newcommand\reference[4]{\referencetofrom{#1}{#2}{#3}{#4}}  % {\reference{\vp}{[to]}{[from]}{[in]}}
%Position vector
\newcommand\posSymbol{\symvec{\vp}}
\newcommand\posnew[3]{\reference{\vp}{#1}{#2}{#3}}
\newcommand\pos[3]{{}_{#1}\posSymbol_{#2\!#3}}
\newcommand\postranspose[3]{{}_{#1}\posSymbol_{#2\!#3}^\transpose} 	%transposed vector
\newcommand\poshom[3]{{}_{#1}\bar{\posSymbol}_{#2\!#3}} 		%homogeneus vector
\newcommand\posdt[3]{{}_{#1}\symdt{\posSymbol}_{#2\!#3}} 		%first time derivative
\newcommand\posddt[3]{{}_{#1}\symddt{\posSymbol}_{#2\!#3}} 		%second time derivative
\newcommand\posdddt[3]{{}_{#1}\symdddt{\posSymbol}_{#2\!#3}} 		%third time derivative
\newcommand\posddddt[3]{{}_{#1}\symddddt{\posSymbol}_{#2\!#3}} 		%fourth time derivative
\newcommand\posest[3]{{}_{#1}\symest{\posSymbol}_{#2\!#3}} 		%estimate
\newcommand\poserr[3]{{}_{#1}\symerr{\posSymbol}_{#2\!#3}} 		%error
\newcommand\posmeas[3]{{}_{#1}\symmeas{\posSymbol}_{#2\!#3}} 		%measurement
\newcommand\posdiff[3]{\symdiff{{}_{#1}\posSymbol}_{#2\!#3}} 		%difference
\newcommand\posmean[3]{\symmeanvec{{}_{#1}{\posSymbol}_{#2\!#3}}} 		%statistical mean
\newcommand\posstd[3]{\symstdvec{{}_{#1}{\posSymbol}_{#2\!#3}}} 		%statistical standard deviation

%Linear velocity vector
\newcommand\linvelSymbol{\symvec{\vv}}
\newcommand\linvel[3]{{}_{#1}\linvelSymbol_{#2\!#3}}
\newcommand\linveltranspose[3]{{}_{#1}\linvelSymbol_{#2\!#3}^\transpose} 		%transposed vector
\newcommand\linvelhom[3]{{}_{#1}\bar{\linvelSymbol}_{#2\!#3}} 				%homogeneus vector
\newcommand\linveldt[3]{{}_{#1}\symdt{\linvelSymbol}_{#2\!#3}} 				%first time derivative
\newcommand\linvelddt[3]{{}_{#1}\symddt{\linvelSymbol}_{#2\!#3}} 				%second time derivative
\newcommand\linveldddt[3]{{}_{#1}\symdddt{\linvelSymbol}_{#2\!#3}} 			%third time derivative
\newcommand\linvelest[3]{{}_{#1}\symest{\linvelSymbol}_{#2\!#3}} 				%estimate
\newcommand\linvelerr[3]{{}_{#1}\symerr{\linvelSymbol}_{#2\!#3}} 				%error
\newcommand\linvelmeas[3]{{}_{#1}\symmeas{\linvelSymbol}_{#2\!#3}} 			%measurement
\newcommand\linveldiff[3]{\symdiff{{}_{#1}\linvelSymbol}_{#2\!#3}} 			%difference
\newcommand\linvelmean[3]{\symmeanvec{{}_{#1}{\linvelSymbol}_{#2\!#3}}} 			%statistical mean
\newcommand\linvelstd[3]{\symstdvec{{}_{#1}{\linvelSymbol}_{#2\!#3}}} 			%statistical standard deviation

%Linear acceleration vector
\newcommand\linaccSymbol{\symvec{\va}}
\newcommand\linacc[3]{{}_{#1}\linaccSymbol_{#2\!#3}}
\newcommand\linacctranspose[3]{{}_{#1}\linaccSymbol_{#2\!#3}^\transpose} 		%transposed vector
\newcommand\linacchom[3]{{}_{#1}\bar{\linaccSymbol}_{#2\!#3}} 				%homogeneus vector
\newcommand\linaccdt[3]{{}_{#1}\symdt{\linaccSymbol}_{#2\!#3}} 				%first time derivative
\newcommand\linaccddt[3]{{}_{#1}\symddt{\linaccSymbol}_{#2\!#3}} 				%second time derivative
\newcommand\linaccest[3]{{}_{#1}\symest{\linaccSymbol}_{#2\!#3}} 				%estimate
\newcommand\linaccerr[3]{{}_{#1}\symerr{\linaccSymbol}_{#2\!#3}} 				%error
\newcommand\linaccmeas[3]{{}_{#1}\symmeas{\linaccSymbol}_{#2\!#3}} 			%measurement
\newcommand\linaccdiff[3]{\symdiff{{}_{#1}\linaccSymbol}_{#2\!#3}} 			%difference
\newcommand\linaccmean[3]{\symmeanvec{{}_{#1}{\linaccSymbol}_{#2\!#3}}} 			%statistical mean
\newcommand\linaccstd[3]{\symstdvec{{}_{#1}{\linaccSymbol}_{#2\!#3}}} 			%statistical standard deviation

%Linear jerk vector
\newcommand\linjerkSymbol{\symvec{\vj}}
\newcommand\linjerk[3]{{}_{#1}\linjerkSymbol_{#2\!#3}}
\newcommand\linjerktranspose[3]{{}_{#1}\linjerkSymbol_{#2\!#3}^\transpose} 	%transposed vector
\newcommand\linjerkhom[3]{{}_{#1}\bar{\linjerkSymbol}_{#2\!#3}} 				%homogeneus vector
\newcommand\linjerkdt[3]{{}_{#1}\symdt{\linjerkSymbol}_{#2\!#3}} 				%first time derivative
\newcommand\linjerkest[3]{{}_{#1}\symest{\linjerkSymbol}_{#2\!#3}} 			%estimate
\newcommand\linjerkerr[3]{{}_{#1}\symerr{\linjerkSymbol}_{#2\!#3}} 			%error
\newcommand\linjerkmeas[3]{{}_{#1}\symmeas{\linjerkSymbol}_{#2\!#3}} 			%measurement
\newcommand\linjerkdiff[3]{\symdiff{{}_{#1}\linjerkSymbol}_{#2\!#3}} 			%difference
\newcommand\linjerkmean[3]{\symmeanvec{{}_{#1}{\linjerkSymbol}_{#2\!#3}}} 		%statistical mean
\newcommand\linjerkstd[3]{\symstdvec{{}_{#1}{\linjerkSymbol}_{#2\!#3}}} 			%statistical standard deviation

%Linear snap vector
\newcommand\linsnapSymbol{\symvec{\vs}}
\newcommand\linsnap[3]{{}_{#1}\linsnapSymbol_{#2\!#3}}
\newcommand\linsnaptranspose[3]{{}_{#1}\linsnapSymbol_{#2\!#3}^\transpose} 	%transposed vector
\newcommand\linsnaphom[3]{{}_{#1}\bar{\linsnapSymbol}_{#2\!#3}} 				%homogeneus vector
\newcommand\linsnapest[3]{{}_{#1}\symest{\linsnapSymbol}_{#2\!#3}} 			%estimate
\newcommand\linsnaperr[3]{{}_{#1}\symerr{\linsnapSymbol}_{#2\!#3}} 			%error
\newcommand\linsnapmeas[3]{{}_{#1}\symmeas{\linsnapSymbol}_{#2\!#3}} 			%measurement
\newcommand\linsnapdiff[3]{\symdiff{{}_{#1}\linsnapSymbol}_{#2\!#3}} 			%difference
\newcommand\linsnapmean[3]{\symmeanvec{{}_{#1}{\linsnapSymbol}_{#2\!#3}}} 		%statistical mean
\newcommand\linsnapstd[3]{\symstdvec{{}_{#1}{\linsnapSymbol}_{#2\!#3}}} 			%statistical standard deviation

%Attitude quaternion
\newcommand\Quat[2]{Q_{#1\!#2}}
\newcommand\quatSymbol{q}
\newcommand\quat[2]{\bar{\mathbf{\quatSymbol}}_{#1\!#2}}
\newcommand\quatnew[2]{\reference{\vq}{#1}{#2}{}}
\newcommand\quatimvec[2]{\symvec{\mathbf{\quatSymbol}}_{v\!,#1\!#2}}
\newcommand\quatimx[2]{\quatSymbol_{x\!,#1\!#2}}
\newcommand\quatimy[2]{\quatSymbol_{y\!,#1\!#2}}
\newcommand\quatimz[2]{\quatSymbol_{z\!,#1\!#2}}
\newcommand\quatreal[2]{\quatSymbol_{w\!,#1\!#2}}
\newcommand\quattwo{\left[ \quatSymbol_w, \symvec{\mathbf{\quatSymbol}}_v \right]^\transpose}
\newcommand\quatfull{\left[ \quatSymbol_w, \quatSymbol_x, \quatSymbol_y, \quatSymbol_z \right]^\transpose}
\newcommand\quattranspose[2]{\quat{#1}{#2}^\transpose} 	%transposed vector
\newcommand\quatconj[2]{\quat{#1}{#2}^{*}} 	%transposed vector
\newcommand\quatest[2]{\symest{\quat{}{}}_{#1\!#2}} 			%estimate
\newcommand\quaterr[2]{\symerr{\quat{}{}}_{#1\!#2}} 			%error
\newcommand\quatmeas[2]{\symmeas{\quat{}{}}_{#1\!#2}} 			%measurement
\newcommand\quatdiff[2]{\symdiff{\quat{#1}{#2}}} 			%difference
\newcommand\quatmean[2]{\symmeanvec{{\quat{}{_{#1\!#2}}}}} 		%statistical mean
\newcommand\quatstd[2]{\symstdvec{{\quat{}{_{#1\!#2}}}}} 			%statistical standard deviation
\newcommand\quatmul{\otimes}
%Orientation RPY
\newcommand{\roll}{\phi}
\newcommand{\pitch}{\theta}
\newcommand{\yaw}{\psi}

\newcommand\smallangle{{\boldsymbol\theta}}

%Rotation matrices
\newcommand\romatSymbol{\vR}
\newcommand\rotmat[2]{\reference{\romatSymbol}{#1}{#2}{}}
\newcommand\rotmatdt[2]{\symdt{\romatSymbol}_{#1\!#2}}
\newcommand\comatSymbol{\vC}
\newcommand\comat[2]{\reference{\comatSymbol}{#1}{#2}{}}
\newcommand\comattranspose[2]{\comatSymbol_{#1\!#2}^\transpose}
\newcommand\comatinv[2]{\comatSymbol_{#1\!#2}^\inverse}
\newcommand\comatdt[2]{\symdt{\comatSymbol}_{#1\!#2}}
\newcommand\comatdttranspose[2]{\symdt{\comatSymbol}_{#1\!#2}^\transpose}
\newcommand\comatquat[2]{\vC{\left( \quat{#1}{#2}{} \right)}}  % {\comatquat{[to]}{[from]}^\transpose}

%Angular velocity vector
\newcommand\angvelSymbol{\symvec{\vom}}
\newcommand\angvel[3]{{}_{#1}\angvelSymbol_{#2\!#3}}
\newcommand\angveltranspose[3]{{}_{#1}\angvelSymbol_{#2\!#3}^\transpose} 	%transposed vector
\newcommand\angvelhom[3]{{}_{#1}\bar{\angvelSymbol}_{#2\!#3}} 				%homogeneus vector
\newcommand\angveldt[3]{{}_{#1}\symdt{\angvelSymbol}_{#2\!#3}} 				%first time derivative
\newcommand\angvelddt[3]{{}_{#1}\symddt{\angvelSymbol}_{#2\!#3}} 			%second time derivative
\newcommand\angveldddt[3]{{}_{#1}\symdddt{\angvelSymbol}_{#2\!#3}} 			%third time derivative
\newcommand\angvelest[3]{{}_{#1}\symest{\angvelSymbol}_{#2\!#3}} 			%estimate
\newcommand\angvelerr[3]{{}_{#1}\symerr{\angvelSymbol}_{#2\!#3}}			%error
\newcommand\angvelmeas[3]{{}_{#1}\symmeas{\angvelSymbol}_{#2\!#3}} 			%measurement
\newcommand\angveldiff[3]{\symdiff{{}_{#1}\angvelSymbol}_{#2\!#3}} 			%difference
\newcommand\angvelmean[3]{\symmeanvec{{}_{#1}{\angvelSymbol}_{#2\!#3}}} 		%statistical mean
\newcommand\angvelstd[3]{\symstdvec{{}_{#1}{\angvelSymbol}_{#2\!#3}}} 			%statistical standard deviation

%Angular acceleration vector
\newcommand\angaccSymbol{\symvec{\val}}
\newcommand\angacc[3]{{}_{#1}\angaccSymbol_{#2\!#3}}
\newcommand\angacctranspose[3]{{}_{#1}\angaccSymbol_{#2\!#3}^\transpose} 	%transposed vector
\newcommand\angacchom[3]{{}_{#1}\bar{\angaccSymbol}_{#2\!#3}} 				%homogeneus vector
\newcommand\angaccdt[3]{{}_{#1}\symdt{\angaccSymbol}_{#2\!#3}} 				%first time derivative
\newcommand\angaccddt[3]{{}_{#1}\symddt{\angaccSymbol}_{#2\!#3}} 			%second time derivative
\newcommand\angaccest[3]{{}_{#1}\symest{\angaccSymbol}_{#2\!#3}} 			%estimate
\newcommand\angaccerr[3]{{}_{#1}\symerr{\angaccSymbol}_{#2\!#3}} 			%error
\newcommand\angaccmeas[3]{{}_{#1}\symmeas{\angaccSymbol}_{#2\!#3}} 			%measurement
\newcommand\angaccdiff[3]{\symdiff{{}_{#1}\angaccSymbol}_{#2\!#3}} 			%difference
\newcommand\angaccmean[3]{\symmeanvec{{}_{#1}{\angaccSymbol}_{#2\!#3}}} 		%statistical mean
\newcommand\angaccstd[3]{\symstdvec{{}_{#1}{\angaccSymbol}_{#2\!#3}}} 			%statistical standard deviation

%Angular jerk vector
\newcommand\angjerkSymbol{\symvec{\vga}}
\newcommand\angjerk[3]{{}_{#1}\angjerkSymbol_{#2\!#3}}
\newcommand\angjerktranspose[3]{{}_{#1}\angjerkSymbol_{#2\!#3}^\transpose} 	%transposed vector
\newcommand\angjerkhom[3]{{}_{#1}\bar{\angjerkSymbol}_{#2\!#3}} 				%homogeneus vector
\newcommand\angjerkdt[3]{{}_{#1}\symdt{\angjerkSymbol}_{#2\!#3}} 				%first time derivative
\newcommand\angjerkest[3]{{}_{#1}\symest{\angjerkSymbol}_{#2\!#3}} 			%estimate
\newcommand\angjerkerr[3]{{}_{#1}\symerr{\angjerkSymbol}_{#2\!#3}} 			%error
\newcommand\angjerkmeas[3]{{}_{#1}\symmeas{\angjerkSymbol}_{#2\!#3}} 			%measurement
\newcommand\angjerkdiff[3]{\symdiff{{}_{#1}\angjerkSymbol}_{#2\!#3}} 			%difference
\newcommand\angjerkmean[3]{\symmeanvec{{}_{#1}{\angjerkSymbol}_{#2\!#3}}} 		%statistical mean
\newcommand\angjerkstd[3]{\symstdvec{{}_{#1}{\angjerkSymbol}_{#2\!#3}}} 			%statistical standard deviation

%Angular snap vector
\newcommand\angsnapSymbol{\symvec{\vio}}
\newcommand\angsnap[3]{{}_{#1}\angsnapSymbol_{#2\!#3}}
\newcommand\angsnaptranspose[3]{{}_{#1}\angsnapSymbol_{#2\!#3}^\transpose} 	%transposed vector
\newcommand\angsnaphom[3]{{}_{#1}\bar{\angsnapSymbol}_{#2\!#3}} 				%homogeneus vector
\newcommand\angsnapest[3]{{}_{#1}\symest{\angsnapSymbol}_{#2\!#3}} 			%estimate
\newcommand\angsnaperr[3]{{}_{#1}\symerr{\angsnapSymbol}_{#2\!#3}}			%error
\newcommand\angsnapmeas[3]{{}_{#1}\symmeas{\angsnapSymbol}_{#2\!#3}} 			%measurement
\newcommand\angsnapdiff[3]{\symdiff{{}_{#1}\angsnapSymbol}_{#2\!#3}} 			%difference
\newcommand\angsnapmean[3]{\symmeanvec{{}_{#1}{\angsnapSymbol}_{#2\!#3}}} 		%statistical mean
\newcommand\angsnapstd[3]{\symstdvec{{}_{#1}{\angsnapSymbol}_{#2\!#3}}} 			%statistical standard deviation

%Bias of ...
\newcommand\biasrealSymbol{b}
\newcommand\biasvecSymbol{\symvec{\vb}}
\newcommand\biasreal[1]{\biasrealSymbol_{#1}}
\newcommand\biasrealdt[1]{\symdt{\biasrealSymbol_{#1}}} 		%first time derivative
\newcommand\biasrealest[1]{\symest{\biasrealSymbol_{#1}}} 		%estimate
\newcommand\biasrealerr[1]{\symerr{\biasrealSymbol_{#1}}} 		%error
\newcommand\biasrealmeas[1]{\symmeas{\biasrealSymbol_{#1}}} 		%measurement
\newcommand\biasrealdiff[1]{\symdiff{\biasrealSymbol_{#1}}} 		%difference
\newcommand\biasrealmean[1]{\symmean{\biasrealSymbol_{#1}}} 		%statistical mean
\newcommand\biasrealstd[1]{\symstd{\biasrealSymbol_{#1}}} 		%statistical standard deviation
\newcommand\biasvec[1]{\biasvecSymbol_{#1}}
\newcommand\biasvectranspose[1]{\biasvecSymbol_{#1}^\transpose} 	%transposed vector
\newcommand\biasvechom[1]{\bar{\biasvecSymbol_{#1}}} 		%homogeneus vector
\newcommand\biasvecdt[1]{\symdt{\biasvecSymbol_{#1}}} 		%first time derivative
\newcommand\biasvecest[1]{\symest{\biasvecSymbol_{#1}}} 		%estimate
\newcommand\biasvecerr[1]{\symerr{\biasvecSymbol_{#1}}} 		%error
\newcommand\biasvecmeas[1]{\symmeas{\biasvecSymbol_{#1}}} 		%measurement
\newcommand\biasvecdiff[1]{\symdiff{\biasvecSymbol_{#1}}} 		%difference
\newcommand\biasvecmean[1]{\symmeanvec{\biasvecSymbol_{#1}}} 		%statistical mean
\newcommand\biasvecstd[1]{\symstdvec{\biasvecSymbol_{#1}}} 		%statistical standard deviation

%Noise of ...
\newcommand\noiserealSymbol{n}
\newcommand\noisevecSymbol{\symvec{\vn}}
\newcommand\noisereal[1]{\noiserealSymbol_{#1}}	
\newcommand\noiserealdt[1]{\symdt{\noiserealSymbol_{#1}}} 		%first time derivative
\newcommand\noiserealest[1]{\symest{\noiserealSymbol_{#1}}} 		%estimate
\newcommand\noiserealerr[1]{\symerr{\noiserealSymbol_{#1}}} 		%error
\newcommand\noiserealmeas[1]{\symmeas{\noiserealSymbol_{#1}}} 		%measurement
\newcommand\noiserealdiff[1]{\symdiff{\noiserealSymbol_{#1}}} 		%difference
\newcommand\noiserealmean[1]{\symmean{\noiserealSymbol_{#1}}} 		%statistical mean
\newcommand\noiserealstd[1]{\symstd{\noiserealSymbol_{#1}}} 		%statistical standard deviation
\newcommand\noisevec[1]{\noisevecSymbol_{#1}}
\newcommand\noisevectranspose[1]{\noisevecSymbol_{#1}^\transpose} 	%transposed vector
\newcommand\noisevechom[1]{\bar{\noisevecSymbol_{#1}}} 		%homogeneus vector
\newcommand\noisevecdt[1]{\symdt{\noisevecSymbol_{#1}}} 		%first time derivative
\newcommand\noisevecest[1]{\symest{\noisevecSymbol_{#1}}} 		%estimate
\newcommand\noisevecerr[1]{\symerr{\noisevecSymbol_{#1}}} 		%error
\newcommand\noisevecmeas[1]{\symmeas{\noisevecSymbol_{#1}}} 		%measurement
\newcommand\noisevecdiff[1]{\symdiff{\noisevecSymbol_{#1}}} 		%difference
\newcommand\noisevecmean[1]{\symmeanvec{\noisevecSymbol_{#1}}} 		%statistical mean
\newcommand\noisevecstd[1]{\symstdvec{\noisevecSymbol_{#1}}} 		%statistical standard deviation

%Mechanics - inertia
\newcommand\inertiaSymbol{\mathbf \mathit{I}}
\newcommand\inertia[1]{{}_{#1}\inertiaSymbol} 	%Referenced inertia tensor
\newcommand\inertiatranspose[1]{{}_{#1}\inertiaSymbol^\transpose} 	%transposed
\newcommand\inertiainv[1]{{}_{#1}\inertiaSymbol^\inverse} 	%inverse
\newcommand\inertiadt[1]{{}_{#1}\symdt{\inertiaSymbol}} 		%first time derivative
\newcommand\inertiaest[1]{{}_{#1}\symest{\inertiaSymbol}} 		%estimate
\newcommand\inertiaerr[1]{{}_{#1}\symerr{\inertiaSymbol}} 		%error
\newcommand\inertiameas[1]{{}_{#1}\symmeas{\inertiaSymbol}} 		%measurement
\newcommand\inertiadiff[1]{\symdiff{{}_{#1}\inertiaSymbol}} 		%difference
\newcommand\inertiamean[1]{\symmeanvec{{}_{#1}{\inertiaSymbol}}} 		%statistical mean
\newcommand\inertiastd[1]{\symstdvec{{}_{#1}{\inertiaSymbol}}} 		%statistical standard deviation
\newcommand\inertiadiagSymbol{\vec{\boldsymbol{i}}}
\newcommand\inertiadiag[1]{{}_{#1}\inertiadiagSymbol} 	%Referenced diagonal of inertia tensor
\newcommand\inertiadiagtranspose[1]{{}_{#1}\inertiadiagSymbol^\transpose} 	%transposed
\newcommand\inertiadiagdt[1]{{}_{#1}\symdt{\inertiadiagSymbol}} 		%first time derivative
\newcommand\inertiadiagest[1]{{}_{#1}\symest{\inertiadiagSymbol}} 		%estimate
\newcommand\inertiadiagerr[1]{{}_{#1}\symerr{\inertiadiagSymbol}} 		%error
\newcommand\inertiadiagmeas[1]{{}_{#1}\symmeas{\inertiadiagSymbol}} 		%measurement
\newcommand\inertiadiagdiff[1]{\symdiff{{}_{#1}\inertiadiagSymbol}} 		%difference
\newcommand\inertiadiagmean[1]{\symmeanvec{{}_{#1}{\inertiadiagSymbol}}} 		%statistical mean
\newcommand\inertiadiagstd[1]{\symstdvec{{}_{#1}{\inertiadiagSymbol}}} 		%statistical standard deviation

%Mechanics - force


==> styles/def-math.tex <==
%-------------------------------------------------------------------
%math operators
%-------------------------------------------------------------------
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\logmap}{log}
\DeclareMathOperator{\expmap}{exp}
\DeclareMathOperator{\logmatrix}{log}
\DeclareMathOperator{\expmatrix}{exp}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\atantwo}{atan2}

\newcommand{\drv}[2]{\frac{\dd}{\dd#1}{\left(#2\right)}}

%-------------------------------------------------------------------
%math
%-------------------------------------------------------------------
\newcommand\identity[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#2}{\empty}}
    {\vI}
    {\ifthenelse{\equal{#1}{\empty}}
        {\vI_{#2}}
        {\vI_{#1\!\times\!#2}}
    }
}
%\renewcommand\identity{\vI}
\newcommand\zero[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#2}{\empty}}
    {\mathbf{0}}
    {\ifthenelse{\equal{#1}{\empty}}
        {\mathbf{0}_{#2}}
        {\mathbf{0}_{#1\!\times\!#2}}
    }
}
%\renewcommand\zero{\mathbf{0}}
\newcommand\norm[1]{\lVert #1 \rVert}
\newcommand\transpose{\mathsf{T}}
\newcommand\inverse{\mathsf{-\!1}}
%\newcommand\inverse{\scriptscriptstyle{\text{-\!1}}}
\newcommand{\dd}{\textnormal{d}}
\newcommand{\dt}{\textnormal{d}t}
\newcommand{\DD}{\textnormal{D}}
\newcommand{\Dt}{\textnormal{D}t}
\newcommand{\deta}{\textnormal{d}\eta}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\Upr}{{\mathop{\mathrm{Upr}}}}
\newcommand{\Sgn}{{\mathop{\mathrm{Sgn}}}}
\newcommand{\h}{\mathop{\mathrm{H}}}
\newcommand{\prox}{{\mathop{\mathrm{prox}}}}
\newcommand{\abs}{\mathop{\mathrm{abs}}}
\newcommand{\T}{^{\mathop{\mathrm{T}}}}
\newcommand{\diag}{{\mathop{\mathrm{diag}}}}
\newcommand{\skewmat}[1]{\left[#1\right]_{\!\times}}
\newcommand{\fullskewmat}[3]{
    \begin{bmatrix} 0 & -#3 & #2 \\ #3 & 0 & -#1 \\ -#2 & #1 & 0 \end{bmatrix}
}
\newcommand{\normaldist}[2]{\mathcal{N}\left(#1,#2 \right)} % \normaldist{\mu}{\sigma^2}

%-------------------------------------------------------------------
%math definitions
%-------------------------------------------------------------------
%Definition of SO(3) matrix
\newcommand\SOthree{\mathrm{SO}(3)}
\newcommand\inSOthree{\in \SOthree}
%Definition of real numbers (vectors, matrices)
\newcommand\Real[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#2}{\empty}}
    {\mathbb{R}}
    {\ifthenelse{\equal{#1}{\empty}}
        {\mathbb{R}^{#2}}
        {\mathbb{R}^{#1\!\times\!#2}}
    }
}
\newcommand\inReal[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#2}{\empty}}
    {\in \Real{}}
    {\ifthenelse{\equal{#1}{\empty}}
        {\in \Real{#2}}
        {\in \Real[#1]{#2}}
    }
}
%Definition of Hamiltonian quaternion
\newcommand\Ham{\mathbb{H}}
\newcommand\inHam{\in \Ham}

%\newcommand\tuple[2]{[#1,#2]}
\newcommand\tuple[2]{\left\langle #1,#2\right\rangle}
\newcommand\teststyles[1]{\mathrm{#1},~\mathit{#1},~\mathcal{#1},~\mathfrak{#1},~\mathbb{#1},~\uppercase{#1},~{}_{\mathrm{#1}},~{\scriptstyle \mathrm{#1}},~{\scriptscriptstyle \mathrm{#1}} }
%-------------------------------------------------------------------
%math variables
%-------------------------------------------------------------------

%-------------------------------------------------------------------
%boldmath
%bold operator
%-------------------------------------------------------------------
\newcommand{\vna}{\mbox{\boldmath $\nabla$}}
%-------------------------------------------------------------------
%bold greek
%-------------------------------------------------------------------
\newcommand{\val}{\mbox{\boldmath $\alpha$}}
\newcommand{\vbe}{\mbox{\boldmath $\beta$}}
\newcommand{\vga}{\mbox{\boldmath $\gamma$}}
\newcommand{\vde}{\mbox{\boldmath $\delta$}}
\newcommand{\vep}{\mbox{\boldmath $\epsilon$}}
\newcommand{\vze}{\mbox{\boldmath $\zeta$}}
\newcommand{\vet}{\mbox{\boldmath $\eta$}}
\newcommand{\vth}{\mbox{\boldmath $\theta$}}
\newcommand{\vio}{\mbox{\boldmath $\iota$}}
\newcommand{\vka}{\mbox{\boldmath $\kappa$}}
\newcommand{\vla}{\mbox{\boldmath $\lambda$}}
\newcommand{\vmu}{\mbox{\boldmath $\mu$}}
\newcommand{\vnu}{\mbox{\boldmath $\nu$}}
\newcommand{\vxi}{\mbox{\boldmath $\xi$}}
\newcommand{\vpi}{\mbox{\boldmath $\pi$}}
\newcommand{\vrh}{\mbox{\boldmath $\rho$}}
\newcommand{\vsi}{\mbox{\boldmath $\sigma$}}
\newcommand{\vta}{\mbox{\boldmath $\tau$}}
\newcommand{\vup}{\mbox{\boldmath $\upsilon$}}
\newcommand{\vph}{\mbox{\boldmath $\varphi$}}
\newcommand{\vch}{\mbox{\boldmath $\chi$}}
\newcommand{\vps}{\mbox{\boldmath $\psi$}}
\newcommand{\vom}{\mbox{\boldmath $\omega$}}

\newcommand{\vvep}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\vvth}{\mbox{\boldmath $\vartheta$}}
\newcommand{\vvrh}{\mbox{\boldmath $\varrho$}}
\newcommand{\vvpi}{\mbox{\boldmath $\varpi$}}
\newcommand{\vvsi}{\mbox{\boldmath $\varsigma$}}
\newcommand{\vvph}{\mbox{\boldmath $\phi$}}

%-------------------------------------------------------------------
%bold capital greek
%-------------------------------------------------------------------
\newcommand{\vGa}{\mathbf \Gamma}
\newcommand{\vDe}{\mathbf \Delta}
\newcommand{\vTh}{\mathbf \Theta}
\newcommand{\vLa}{\mathbf \Lambda}
\newcommand{\vXi}{\mathbf \Xi}
\newcommand{\vPi}{\mathbf \Pi}
\newcommand{\vSi}{\mathbf \Sigma}
\newcommand{\vUp}{\mathbf \Upsilon}
\newcommand{\vPh}{\mathbf \Phi}
\newcommand{\vPs}{\mathbf \Psi}
\newcommand{\vOm}{\mathbf \Omega}

%capital greek slanted, OHNE amsmath-package
%\newcommand{\iGa}{\mathnormal{\Gamma}}
%\newcommand{\iDe}{\mathnormal{\Delta}}
%\newcommand{\iTh}{\mathnormal{\Theta}}
%\newcommand{\iLa}{\mathnormal{\Lambda}}
%\newcommand{\iXi}{\mathnormal{\Xi}}
%\newcommand{\iPi}{\mathnormal{\Pi}}
%\newcommand{\iSi}{\mathnormal{\Sigma}}
%\newcommand{\iUp}{\mathnormal{\Upsilon}}
%\newcommand{\iPh}{\mathnormal{\Phi}}
%\newcommand{\iPs}{\mathnormal{\Psi}}
%\newcommand{\iOm}{\mathnormal{\Omega}}

%-------------------------------------------------------------------
%capital greek slanted, MIT amsmath-package
%-------------------------------------------------------------------
\newcommand{\iGa}{\varGamma}
\newcommand{\iDe}{\varDelta}
\newcommand{\iTh}{\varTheta}
\newcommand{\iLa}{\varLambda}
\newcommand{\iXi}{\varXi}
\newcommand{\iPi}{\varPi}
\newcommand{\iSi}{\varSigma}
\newcommand{\iUp}{\varUpsilon}
\newcommand{\iPh}{\varPhi}
\newcommand{\iPs}{\varPsi}
\newcommand{\iOm}{\varOmega}

%-------------------------------------------------------------------
%bold latin
%-------------------------------------------------------------------
\newcommand{\va}{\mathbf a}
\newcommand{\vb}{\mathbf b}
\newcommand{\vc}{\mathbf c}
\newcommand{\vd}{\mathbf d}
\newcommand{\ve}{\mathbf e}
\newcommand{\vf}{\mathbf f}
\newcommand{\vg}{\mathbf g}
\newcommand{\vh}{\mathbf h}
\newcommand{\vi}{\mathbf i}
\newcommand{\vj}{\mathbf j}
\newcommand{\vk}{\mathbf k}
\newcommand{\vl}{\mathbf l}
\newcommand{\vm}{\mathbf m}
\newcommand{\vn}{\mathbf n}
\newcommand{\vo}{\mathbf o}
\newcommand{\vp}{\mathbf p}
\newcommand{\vq}{\mathbf q}
\newcommand{\vr}{\mathbf r}
\newcommand{\vs}{\mathbf s}
\newcommand{\vt}{\mathbf t}
\newcommand{\vu}{\mathbf u}
\newcommand{\vv}{\mathbf v}
\newcommand{\vw}{\mathbf w}
\newcommand{\vx}{\mathbf x}
\newcommand{\vy}{\mathbf y}
\newcommand{\vz}{\mathbf z}
\newcommand{\eins}{\mathbf 1}

%-------------------------------------------------------------------
%bold capital latin
%-------------------------------------------------------------------
\newcommand{\vA}{\mathbf A}
\newcommand{\vB}{\mathbf B}
\newcommand{\vC}{\mathbf C}
\newcommand{\vD}{\mathbf D}
\newcommand{\vE}{\mathbf E}
\newcommand{\vF}{\mathbf F}
\newcommand{\vG}{\mathbf G}
\newcommand{\vH}{\mathbf H}
\newcommand{\vI}{\mathbf I}
\newcommand{\vJ}{\mathbf J}
\newcommand{\vK}{\mathbf K}
\newcommand{\vL}{\mathbf L}
\newcommand{\vM}{\mathbf M}
\newcommand{\vN}{\mathbf N}
\newcommand{\vO}{\mathbf O}
\newcommand{\vP}{\mathbf P}
\newcommand{\vQ}{\mathbf Q}
\newcommand{\vR}{\mathbf R}
\newcommand{\vS}{\mathbf S}
\newcommand{\vT}{\mathbf T}
\newcommand{\vU}{\mathbf U}
\newcommand{\vV}{\mathbf V}
\newcommand{\vW}{\mathbf W}
\newcommand{\vX}{\mathbf X}
\newcommand{\vY}{\mathbf Y}
\newcommand{\vZ}{\mathbf Z}

%-------------------------------------------------------------------
%calligraphic
%-------------------------------------------------------------------
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%-------------------------------------------------------------------
%fraktur
%-------------------------------------------------------------------
\newcommand{\frA}{\mathfrak{A}}
\newcommand{\frB}{\mathfrak{B}}
\newcommand{\frC}{\mathfrak{C}}
\newcommand{\frD}{\mathfrak{D}}
\newcommand{\frE}{\mathfrak{E}}
\newcommand{\frF}{\mathfrak{F}}
\newcommand{\frG}{\mathfrak{G}}
\newcommand{\frH}{\mathfrak{H}}
\newcommand{\frI}{\mathfrak{I}}
\newcommand{\frJ}{\mathfrak{J}}
\newcommand{\frK}{\mathfrak{K}}
\newcommand{\frL}{\mathfrak{L}}
\newcommand{\frM}{\mathfrak{M}}
\newcommand{\frN}{\mathfrak{N}}
\newcommand{\frO}{\mathfrak{O}}
\newcommand{\frP}{\mathfrak{P}}
\newcommand{\frQ}{\mathfrak{Q}}
\newcommand{\frR}{\mathfrak{R}}
\newcommand{\frS}{\mathfrak{S}}
\newcommand{\frT}{\mathfrak{T}}
\newcommand{\frU}{\mathfrak{U}}
\newcommand{\frV}{\mathfrak{V}}
\newcommand{\frW}{\mathfrak{W}}
\newcommand{\frX}{\mathfrak{X}}
\newcommand{\frY}{\mathfrak{Y}}
\newcommand{\frZ}{\mathfrak{Z}}

\newcommand{\fra}{\mathfrak{a}}
\newcommand{\frb}{\mathfrak{b}}
\newcommand{\frc}{\mathfrak{c}}
\newcommand{\frd}{\mathfrak{d}}
\newcommand{\fre}{\mathfrak{e}}
\newcommand{\frf}{\mathfrak{f}}
\newcommand{\frg}{\mathfrak{g}}
\newcommand{\frh}{\mathfrak{h}}
\newcommand{\fri}{\mathfrak{i}}
\newcommand{\frj}{\mathfrak{j}}
\newcommand{\frk}{\mathfrak{k}}
\newcommand{\frl}{\mathfrak{l}}
\newcommand{\frm}{\mathfrak{m}}
\newcommand{\frn}{\mathfrak{n}}
\newcommand{\fro}{\mathfrak{o}}
\newcommand{\frp}{\mathfrak{p}}
\newcommand{\frq}{\mathfrak{q}}
\newcommand{\frr}{\mathfrak{r}}
\newcommand{\frs}{\mathfrak{s}}
\newcommand{\frt}{\mathfrak{t}}
\newcommand{\fru}{\mathfrak{u}}
\newcommand{\frv}{\mathfrak{v}}
\newcommand{\frw}{\mathfrak{w}}
\newcommand{\frx}{\mathfrak{x}}
\newcommand{\fry}{\mathfrak{y}}
\newcommand{\frz}{\mathfrak{z}}
%
%-------------------------------------------------------------------
%mathrm for reference frames
%-------------------------------------------------------------------
\newcommand{\rmA}{\mathrm{A}}
\newcommand{\rmB}{\mathrm{B}}
\newcommand{\rmC}{\mathrm{C}}
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\rmE}{\mathrm{E}}
\newcommand{\rmF}{\mathrm{F}}
\newcommand{\rmG}{\mathrm{G}}
\newcommand{\rmH}{\mathrm{H}}
\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmJ}{\mathrm{J}}
\newcommand{\rmK}{\mathrm{K}}
\newcommand{\rmL}{\mathrm{L}}
\newcommand{\rmM}{\mathrm{M}}
\newcommand{\rmN}{\mathrm{N}}
\newcommand{\rmO}{\mathrm{O}}
\newcommand{\rmP}{\mathrm{P}}
\newcommand{\rmQ}{\mathrm{Q}}
\newcommand{\rmR}{\mathrm{R}}
\newcommand{\rmS}{\mathrm{S}}
\newcommand{\rmT}{\mathrm{T}}
\newcommand{\rmU}{\mathrm{U}}
\newcommand{\rmV}{\mathrm{V}}
\newcommand{\rmW}{\mathrm{W}}
\newcommand{\rmX}{\mathrm{X}}
\newcommand{\rmY}{\mathrm{Y}}
\newcommand{\rmZ}{\mathrm{Z}}
                     
\newcommand{\rma}{\mathrm{a}}
\newcommand{\rmb}{\mathrm{b}}
\newcommand{\rmc}{\mathrm{c}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmf}{\mathrm{f}}
\newcommand{\rmg}{\mathrm{g}}
\newcommand{\rmh}{\mathrm{h}}
\newcommand{\rmi}{\mathrm{i}}
\newcommand{\rmj}{\mathrm{j}}
\newcommand{\rmk}{\mathrm{k}}
\newcommand{\rml}{\mathrm{l}}
\newcommand{\rmm}{\mathrm{m}}
\newcommand{\rmn}{\mathrm{n}}
\newcommand{\rmo}{\mathrm{o}}
\newcommand{\rmp}{\mathrm{p}}
\newcommand{\rmq}{\mathrm{q}}
\newcommand{\rmr}{\mathrm{r}}
\newcommand{\rms}{\mathrm{s}}
\newcommand{\rmt}{\mathrm{t}}
\newcommand{\rmu}{\mathrm{u}}
\newcommand{\rmv}{\mathrm{v}}
\newcommand{\rmw}{\mathrm{w}}
\newcommand{\rmx}{\mathrm{x}}
\newcommand{\rmy}{\mathrm{y}}
\newcommand{\rmz}{\mathrm{z}}



==> styles/def.tex <==
%CB2018
%RJ2018

%-------------------------------------------------------------------
% packages
%-------------------------------------------------------------------

\usepackage{nonfloat}
\usepackage{multicol}
\usepackage[font=scriptsize]{caption}
\usepackage{calc}
\usepackage{ifthen}
\usepackage[landscape]{geometry}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{multirow}
 \usepackage[T1]{fontenc}
% \usepackage{bbold}
    \usepackage{dsfont}
%\usepackage{esvect}
\usepackage{graphics}
   \usepackage[pdftex]{graphicx}

\usepackage{tabularx,booktabs} 
\usepackage{epstopdf}
 \usepackage{ifpdf}
\usepackage{sectsty}
\usepackage{tikz}
\usepackage{mathtools} % \mathclap for underbrace
\paragraphfont{\small}

\usepackage[explicit]{titlesec}
\usepackage{xcolor}
\usepackage{listings}

%\usepackage{hyperref}
\usepackage[linktoc=all]{hyperref}

%\usepackage{subdepth}%%Keeping subscripts down


%-------------------------------------------------------------------
% page settings
%-------------------------------------------------------------------

% This sets page margins to .5 inch if using letter paper, and to 1/2cm
% if using A4 paper. (This probably isn't strictly necessary.)
% If using another size paper, use default 1cm margins.
\ifthenelse{\lengthtest { \paperwidth = 11in}}
	{ \geometry{top=.5in,left=.5in,right=.5in,bottom=.5in} }
	{\ifthenelse{ \lengthtest{ \paperwidth = 297mm}}
		{\geometry{top=2cm,left=1cm,right=1cm,bottom=2cm} }
		{\geometry{top=1cm,left=1cm,right=1cm,bottom=1cm} }
	}

% Turn off header and footer
\pagestyle{plain}

% Redefine section commands to use less space
\makeatletter
\renewcommand{\chapter}{\@startsection{chapter}{0}{0mm}%
                               {-1sp plus -0sp minus -1sp}%
                                {1\baselineskip}%x
                                {\normalfont\huge\bfseries}}
\renewcommand \thechapter {\@Roman\c@chapter.\hspace{-1.5ex}}

\renewcommand{\section}{\@startsection{section}{1}{0mm}%
                               {-1ex plus -.5ex minus -.2ex}%
                                {0.5ex plus .2ex}%x
                                {\normalfont\large\bfseries}}
  
\renewcommand{\subsection}{\@startsection{subsection}{2}{0mm}%
                                {-1explus -.5ex minus -.2ex}%
                                {0.5ex plus .2ex}%
                                {\normalfont\normalsize\bfseries}}
\renewcommand{\subsubsection}{\@startsection{subsubsection}{3}{0mm}%
                                {-1ex plus -.5ex minus -.2ex}%
                                {1ex plus .2ex}%
                                {\normalfont\small\bfseries}}
\makeatother

% Define BibTeX command
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% Don't print section numbers
\setcounter{secnumdepth}{0}

\setlength{\parindent}{0pt}
\setlength{\parskip}{0pt plus 0.5ex}


%-------------------------------------------------------------------
% listing styles
%-------------------------------------------------------------------
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstdefinestyle{customcpp}{
%  belowcaptionskip=1\baselineskip,
%  frame=L,
   xleftmargin=2ex,
   xrightmargin=2ex,
%  language=C++,
%  showstringspaces=false,
%  basicstyle=\footnotesize\ttfamily,
%  keywordstyle=\bfseries\color{green!40!black},
%  commentstyle=\itshape\color{purple!40!black},
%  identifierstyle=\color{blue},
%  stringstyle=\color{orange},
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\tiny,        % the size of the fonts that are used for=true the code
  breakatwhitespace=true,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  breakautoindent=true             % activates or deactivates automatic indention of broken line
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  escapebegin=\color{mygreen},
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=C++,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,	                   % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with 
}

\lstdefinestyle{customasm}{
  belowcaptionskip=1\baselineskip,
  frame=L,
  xleftmargin=\parindent,
  language=[x86masm]Assembler,
  basicstyle=\footnotesize\ttfamily,
  commentstyle=\itshape\color{purple!40!black},
}


%-------------------------------------------------------------------
% markings
%-------------------------------------------------------------------
\newcommand{\addition}[1]{\textcolor{green}{\textbf{#1}}}
\newcommand{\change}[1]{\textcolor{orange}{\textbf{#1}}}
\newcommand{\comment}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\warning}[1]{\textcolor{red}{\textbf{#1}}}


%-------------------------------------------------------------------
%graphics
%-------------------------------------------------------------------
\DeclareGraphicsExtensions{.pdf,.eps}


%-------------------------------------------------------------------
%figures
%-------------------------------------------------------------------
\input{styles/colors} %.m file!
%using: Blues, Greens, Reds, RdYlBu, RdYlGn and Paired

\newcommand{\sizes}{3.4} % selbstdefinierte Punktgrösse in Bilder
\newcommand{\sizem}{5.1}% selbstdefinierte Punktgrösse in Bilder

\newcommand\myfigure[1]{%
\medskip\noindent\begin{minipage}{\columnwidth}
\centering%
#1%
%figure,caption, and label go here
\end{minipage}\medskip}


%-------------------------------------------------------------------
%university colors
%-------------------------------------------------------------------
\input{styles/def-colors}

%-------------------------------------------------------------------
%math
%-------------------------------------------------------------------
\input{styles/def-math}
%-------------------------------------------------------------------
%kinematics definitions
%-------------------------------------------------------------------
\input{styles/def-kinematics}








==> styles/def_no_subscript_alignment.tex <==
%CB2018

%-------------------------------------------------------------------
% packages
%-------------------------------------------------------------------

\usepackage{nonfloat}
\usepackage{multicol}
\usepackage[font=scriptsize]{caption}
\usepackage{calc}
\usepackage{ifthen}
\usepackage[landscape]{geometry}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{multirow}
 \usepackage[T1]{fontenc}
% \usepackage{bbold}
    \usepackage{dsfont}
%\usepackage{esvect}
\usepackage{graphics}
   \usepackage[pdftex]{graphicx}

\usepackage{tabularx,booktabs} 
\usepackage{epstopdf}
 \usepackage{ifpdf}
\usepackage{sectsty}
\usepackage{tikz}
\usepackage{mathtools} % \mathclap for underbrace
\paragraphfont{\small}

\usepackage[explicit]{titlesec}
\usepackage{xcolor}

%\usepackage{hyperref}
\usepackage[linktoc=all]{hyperref}

%\usepackage{subdepth}%%Keeping subscripts down


%-------------------------------------------------------------------
% page settings
%-------------------------------------------------------------------

% This sets page margins to .5 inch if using letter paper, and to 1/2cm
% if using A4 paper. (This probably isn't strictly necessary.)
% If using another size paper, use default 1cm margins.
\ifthenelse{\lengthtest { \paperwidth = 11in}}
	{ \geometry{top=.5in,left=.5in,right=.5in,bottom=.5in} }
	{\ifthenelse{ \lengthtest{ \paperwidth = 297mm}}
		{\geometry{top=2cm,left=1cm,right=1cm,bottom=2cm} }
		{\geometry{top=1cm,left=1cm,right=1cm,bottom=1cm} }
	}

% Turn off header and footer
\pagestyle{plain}

% Redefine section commands to use less space
\makeatletter
  \renewcommand{\section}{\@startsection{section}{1}{0mm}%
                               {-1ex plus -.5ex minus -.2ex}%
                                {0.5ex plus .2ex}%x
                                {\normalfont\large\bfseries}}
  
\renewcommand{\subsection}{\@startsection{subsection}{2}{0mm}%
                                {-1explus -.5ex minus -.2ex}%
                                {0.5ex plus .2ex}%
                                {\normalfont\normalsize\bfseries}}
\renewcommand{\subsubsection}{\@startsection{subsubsection}{3}{0mm}%
                                {-1ex plus -.5ex minus -.2ex}%
                                {1ex plus .2ex}%
                                {\normalfont\small\bfseries}}
\makeatother

% Define BibTeX command
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% Don't print section numbers
\setcounter{secnumdepth}{0}

\setlength{\parindent}{0pt}
\setlength{\parskip}{0pt plus 0.5ex}


% \input{styles/settings}

%-------------------------------------------------------------------
% markings
%-------------------------------------------------------------------

\newcommand{\addition}[1]{\textcolor{green}{\textbf{#1}}}
\newcommand{\remark}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\change}[1]{\textcolor{orange}{\textbf{#1}}}
\newcommand{\warning}[1]{\textcolor{red}{\textbf{#1}}}


%-------------------------------------------------------------------
%graphics
%-------------------------------------------------------------------
\DeclareGraphicsExtensions{.pdf,.eps}

%-------------------------------------------------------------------
%figures
%-------------------------------------------------------------------
\input{styles/colors} %.m file!

\newcommand{\sizes}{3.4} % selbstdefinierte Punktgrösse in Bilder
\newcommand{\sizem}{5.1}% selbstdefinierte Punktgrösse in Bilder

\newcommand\myfigure[1]{%
\medskip\noindent\begin{minipage}{\columnwidth}
\centering%
#1%
%figure,caption, and label go here
\end{minipage}\medskip}

%-------------------------------------------------------------------
%additional colors
%-------------------------------------------------------------------
\definecolor{AAUlogodarkblue}{RGB}{51,107,129}
\definecolor{AAUlogolightblue}{RGB}{70,153,194}
\definecolor{AAUdarkblue}{RGB}{10,54,96}
\definecolor{AAUviolett}{RGB}{84,63,145}
\definecolor{AAUgreen}{RGB}{128,167,51}
\definecolor{AAUyellow}{RGB}{239,213,34}
\definecolor{AAUtewi}{RGB}{122,20,112}
\definecolor{AAUwiwi}{RGB}{145,191,62}
\definecolor{AAUiff}{RGB}{184,34,49}
\definecolor{AAUkuwi}{RGB}{120,92,167}

%-------------------------------------------------------------------
%math operators
%-------------------------------------------------------------------
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\logmap}{log}
\DeclareMathOperator{\expmap}{exp}
\DeclareMathOperator{\logmatrix}{log}
\DeclareMathOperator{\expmatrix}{exp}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\atantwo}{atan2}

%-------------------------------------------------------------------
%math
%-------------------------------------------------------------------
\newcommand\identity[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#2}{\empty}}
    {\vI}
    {\ifthenelse{\equal{#1}{\empty}}
        {\vI_{#2}^{}}
        {\vI_{#1\!\times\!#2}}
    }
}
%\renewcommand\identity{\vI}
\newcommand\zero[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#2}{\empty}}
    {\mathbf{0}}
    {\ifthenelse{\equal{#1}{\empty}}
        {\mathbf{0}_{#2}}
        {\mathbf{0}_{#1\!\times\!#2}}
    }
}
%\renewcommand\zero{\mathbf{0}}
\newcommand\norm[1]{\lVert #1 \rVert}
\newcommand\transpose{\mathsf{T}}
\newcommand{\dd}{\textnormal{d}}
\newcommand{\dt}{\textnormal{d}t}
\newcommand{\DD}{\textnormal{D}}
\newcommand{\Dt}{\textnormal{D}t}
\newcommand{\deta}{\textnormal{d}\eta}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\Upr}{{\mathop{\mathrm{Upr}}}}
\newcommand{\Sgn}{{\mathop{\mathrm{Sgn}}}}
\newcommand{\h}{\mathop{\mathrm{H}}}
\newcommand{\prox}{{\mathop{\mathrm{prox}}}}
\newcommand{\abs}{\mathop{\mathrm{abs}}}
\newcommand{\T}{^{\mathop{\mathrm{T}}}}
\newcommand{\diag}{{\mathop{\mathrm{diag}}}}
\newcommand{\skewmat}[1]{\left[#1\right]_{\times}}
\newcommand{\fullskewmat}[3]{
    \begin{bmatrix} 0 & -#3 & #2 \\ #3 & 0 & -#1 \\ -#2 & #1 & 0 \end{bmatrix}
}


%-------------------------------------------------------------------
%math definitions
%-------------------------------------------------------------------

%Definition of SO(3) matrix
\newcommand\SOthree{\mathrm{SO}(3)}
\newcommand\inSOthree{\in \SOthree}
%Definition of real numbers (vectors, matrices)
\newcommand\Real[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#2}{\empty}}
    {\mathbb{R}}
    {\ifthenelse{\equal{#1}{\empty}}
        {\mathbb{R}^{#2}}
        {\mathbb{R}^{#1\!\times\!#2}}
    }
}
\newcommand\inReal[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#2}{\empty}}
    {\in \Real{}}
    {\ifthenelse{\equal{#1}{\empty}}
        {\in \Real{#2}}
        {\in \Real[#1]{#2}}
    }
}


%-------------------------------------------------------------------
%math variables
%-------------------------------------------------------------------

%Position vector
\newcommand\pos[4][\empty]{{}^{}_#2\vp_{#3\!#4}^{#1}}
%Time derivative of position vector
\newcommand\posdot[3]{{}_#1\dot{\vp}_{#2\!#3}}
\newcommand\poshat[3]{{}_#1\hat{\vp}_{#2\!#3}}
\newcommand\poshatdot[3]{{}_#1\dot{\hat{\vp}}_{#2\!#3}}
\newcommand\postranspose[3]{{}_#1\vp_{#2\!#3}^\transpose}
\newcommand\poshom[4][\empty]{{}^{}_#2\bar{\vp}_{#3\!#4}^{#1}}
\newcommand\rotmat[2]{\vR_{#1\!#2}}
\newcommand\drotmat[2]{\dot{\vR}_{#1\!#2}}
\newcommand\comat[2]{\vC_{#1\!#2}}
\newcommand\dcomat[2]{\dot{\vC}_{#1\!#2}}
\newcommand\quat[2]{\vq_{#1\!#2}}
\newcommand\Quat[2]{Q_{#1\!#2}}
\newcommand\angleaxis[2]{(\theta,\vn)_{#1\!#2}}
\newcommand\rotvec[2]{\vvph_{#1\!#2}}
\newcommand\linvel[2]{{}_#1\vv_{#2}}
\newcommand\rotvel[3]{{}_#1\vom_{#2\!#3}}
\newcommand\rotvelhat[3]{{}_#1\hat{\vom}_{#2\!#3}}
\newcommand\dvch[0]{\dot{\vch}}
\newcommand\imquatvec[1]{\check{\mathbf{#1}}}
%\newcommand\imquatvec[1]{\overrightarrow{\mathbf{#1}}}
\newcommand\imquatvecFrame[3]{\check{\mathbf{#1}}_{#2\!#3}}
\newcommand\skewImquatvecFrame[3]{\hat{\check{\mathbf{#1}}}_{#2\!#3}}
\newcommand\unitvec[2]{{}_#1\ve_{#2}}
\renewcommand\unitvec[2][\empty \empty]{%%% \empty: Standardwert des optionalen Parameters
  \ifthenelse{\equal{#1}{\empty}}
     {\ve_{#2}}
     {{}_#1\ve_{#2}}
}

%-------------------------------------------------------------------
%boldmath
%bold operator
%-------------------------------------------------------------------
\newcommand{\vna}{\mbox{\boldmath $\nabla$}}
%-------------------------------------------------------------------
%bold greek
%-------------------------------------------------------------------
\newcommand{\val}{\mbox{\boldmath $\alpha$}}
\newcommand{\vbe}{\mbox{\boldmath $\beta$}}
\newcommand{\vga}{\mbox{\boldmath $\gamma$}}
\newcommand{\vde}{\mbox{\boldmath $\delta$}}
\newcommand{\vep}{\mbox{\boldmath $\epsilon$}}
\newcommand{\vze}{\mbox{\boldmath $\zeta$}}
\newcommand{\vet}{\mbox{\boldmath $\eta$}}
\newcommand{\vth}{\mbox{\boldmath $\theta$}}
\newcommand{\vio}{\mbox{\boldmath $\iota$}}
\newcommand{\vka}{\mbox{\boldmath $\kappa$}}
\newcommand{\vla}{\mbox{\boldmath $\lambda$}}
\newcommand{\vmu}{\mbox{\boldmath $\mu$}}
\newcommand{\vnu}{\mbox{\boldmath $\nu$}}
\newcommand{\vxi}{\mbox{\boldmath $\xi$}}
\newcommand{\vpi}{\mbox{\boldmath $\pi$}}
\newcommand{\vrh}{\mbox{\boldmath $\rho$}}
\newcommand{\vsi}{\mbox{\boldmath $\sigma$}}
\newcommand{\vta}{\mbox{\boldmath $\tau$}}
\newcommand{\vup}{\mbox{\boldmath $\upsilon$}}
\newcommand{\vph}{\mbox{\boldmath $\varphi$}}
\newcommand{\vch}{\mbox{\boldmath $\chi$}}
\newcommand{\vps}{\mbox{\boldmath $\psi$}}
\newcommand{\vom}{\mbox{\boldmath $\omega$}}

\newcommand{\vvep}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\vvth}{\mbox{\boldmath $\vartheta$}}
\newcommand{\vvrh}{\mbox{\boldmath $\varrho$}}
\newcommand{\vvpi}{\mbox{\boldmath $\varpi$}}
\newcommand{\vvsi}{\mbox{\boldmath $\varsigma$}}
\newcommand{\vvph}{\mbox{\boldmath $\phi$}}

%-------------------------------------------------------------------
%bold capital greek
%-------------------------------------------------------------------
\newcommand{\vGa}{\mathbf \Gamma}
\newcommand{\vDe}{\mathbf \Delta}
\newcommand{\vTh}{\mathbf \Theta}
\newcommand{\vLa}{\mathbf \Lambda}
\newcommand{\vXi}{\mathbf \Xi}
\newcommand{\vPi}{\mathbf \Pi}
\newcommand{\vSi}{\mathbf \Sigma}
\newcommand{\vUp}{\mathbf \Upsilon}
\newcommand{\vPh}{\mathbf \Phi}
\newcommand{\vPs}{\mathbf \Psi}
\newcommand{\vOm}{\mathbf \Omega}

%capital greek slanted, OHNE amsmath-package
%\newcommand{\iGa}{\mathnormal{\Gamma}}
%\newcommand{\iDe}{\mathnormal{\Delta}}
%\newcommand{\iTh}{\mathnormal{\Theta}}
%\newcommand{\iLa}{\mathnormal{\Lambda}}
%\newcommand{\iXi}{\mathnormal{\Xi}}
%\newcommand{\iPi}{\mathnormal{\Pi}}
%\newcommand{\iSi}{\mathnormal{\Sigma}}
%\newcommand{\iUp}{\mathnormal{\Upsilon}}
%\newcommand{\iPh}{\mathnormal{\Phi}}
%\newcommand{\iPs}{\mathnormal{\Psi}}
%\newcommand{\iOm}{\mathnormal{\Omega}}

%-------------------------------------------------------------------
%capital greek slanted, MIT amsmath-package
%-------------------------------------------------------------------
\newcommand{\iGa}{\varGamma}
\newcommand{\iDe}{\varDelta}
\newcommand{\iTh}{\varTheta}
\newcommand{\iLa}{\varLambda}
\newcommand{\iXi}{\varXi}
\newcommand{\iPi}{\varPi}
\newcommand{\iSi}{\varSigma}
\newcommand{\iUp}{\varUpsilon}
\newcommand{\iPh}{\varPhi}
\newcommand{\iPs}{\varPsi}
\newcommand{\iOm}{\varOmega}

%-------------------------------------------------------------------
%bold latin
%-------------------------------------------------------------------
\newcommand{\va}{\mathbf a}
\newcommand{\vb}{\mathbf b}
\newcommand{\vc}{\mathbf c}
\newcommand{\vd}{\mathbf d}
\newcommand{\ve}{\mathbf e}
\newcommand{\vf}{\mathbf f}
\newcommand{\vg}{\mathbf g}
\newcommand{\vh}{\mathbf h}
\newcommand{\vi}{\mathbf i}
\newcommand{\vj}{\mathbf j}
\newcommand{\vk}{\mathbf k}
\newcommand{\vl}{\mathbf l}
\newcommand{\vm}{\mathbf m}
\newcommand{\vn}{\mathbf n}
\newcommand{\vo}{\mathbf o}
\newcommand{\vp}{\mathbf p}
\newcommand{\vq}{\mathbf q}
\newcommand{\vr}{\mathbf r}
\newcommand{\vs}{\mathbf s}
\newcommand{\vt}{\mathbf t}
\newcommand{\vu}{\mathbf u}
\newcommand{\vv}{\mathbf v}
\newcommand{\vw}{\mathbf w}
\newcommand{\vx}{\mathbf x}
\newcommand{\vy}{\mathbf y}
\newcommand{\vz}{\mathbf z}
\newcommand{\eins}{\mathbf 1}

%-------------------------------------------------------------------
%bold capital latin
%-------------------------------------------------------------------
\newcommand{\vA}{\mathbf A}
\newcommand{\vB}{\mathbf B}
\newcommand{\vC}{\mathbf C}
\newcommand{\vD}{\mathbf D}
\newcommand{\vE}{\mathbf E}
\newcommand{\vF}{\mathbf F}
\newcommand{\vG}{\mathbf G}
\newcommand{\vH}{\mathbf H}
\newcommand{\vI}{\mathbf I}
\newcommand{\vJ}{\mathbf J}
\newcommand{\vK}{\mathbf K}
\newcommand{\vL}{\mathbf L}
\newcommand{\vM}{\mathbf M}
\newcommand{\vN}{\mathbf N}
\newcommand{\vO}{\mathbf O}
\newcommand{\vP}{\mathbf P}
\newcommand{\vQ}{\mathbf Q}
\newcommand{\vR}{\mathbf R}
\newcommand{\vS}{\mathbf S}
\newcommand{\vT}{\mathbf T}
\newcommand{\vU}{\mathbf U}
\newcommand{\vV}{\mathbf V}
\newcommand{\vW}{\mathbf W}
\newcommand{\vX}{\mathbf X}
\newcommand{\vY}{\mathbf Y}
\newcommand{\vZ}{\mathbf Z}

%-------------------------------------------------------------------
%calligraphic
%-------------------------------------------------------------------
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%-------------------------------------------------------------------
%fraktur
%-------------------------------------------------------------------
\newcommand{\frA}{\mathfrak{A}}
\newcommand{\frB}{\mathfrak{B}}
\newcommand{\frC}{\mathfrak{C}}
\newcommand{\frD}{\mathfrak{D}}
\newcommand{\frE}{\mathfrak{E}}
\newcommand{\frF}{\mathfrak{F}}
\newcommand{\frG}{\mathfrak{G}}
\newcommand{\frH}{\mathfrak{H}}
\newcommand{\frI}{\mathfrak{I}}
\newcommand{\frJ}{\mathfrak{J}}
\newcommand{\frK}{\mathfrak{K}}
\newcommand{\frL}{\mathfrak{L}}
\newcommand{\frM}{\mathfrak{M}}
\newcommand{\frN}{\mathfrak{N}}
\newcommand{\frO}{\mathfrak{O}}
\newcommand{\frP}{\mathfrak{P}}
\newcommand{\frQ}{\mathfrak{Q}}
\newcommand{\frR}{\mathfrak{R}}
\newcommand{\frS}{\mathfrak{S}}
\newcommand{\frT}{\mathfrak{T}}
\newcommand{\frU}{\mathfrak{U}}
\newcommand{\frV}{\mathfrak{V}}
\newcommand{\frW}{\mathfrak{W}}
\newcommand{\frX}{\mathfrak{X}}
\newcommand{\frY}{\mathfrak{Y}}
\newcommand{\frZ}{\mathfrak{Z}}

\newcommand{\fra}{\mathfrak{a}}
\newcommand{\frb}{\mathfrak{b}}
\newcommand{\frc}{\mathfrak{c}}
\newcommand{\frd}{\mathfrak{d}}
\newcommand{\fre}{\mathfrak{e}}
\newcommand{\frf}{\mathfrak{f}}
\newcommand{\frg}{\mathfrak{g}}
\newcommand{\frh}{\mathfrak{h}}
\newcommand{\fri}{\mathfrak{i}}
\newcommand{\frj}{\mathfrak{j}}
\newcommand{\frk}{\mathfrak{k}}
\newcommand{\frl}{\mathfrak{l}}
\newcommand{\frm}{\mathfrak{m}}
\newcommand{\frn}{\mathfrak{n}}
\newcommand{\fro}{\mathfrak{o}}
\newcommand{\frp}{\mathfrak{p}}
\newcommand{\frq}{\mathfrak{q}}
\newcommand{\frr}{\mathfrak{r}}
\newcommand{\frs}{\mathfrak{s}}
\newcommand{\frt}{\mathfrak{t}}
\newcommand{\fru}{\mathfrak{u}}
\newcommand{\frv}{\mathfrak{v}}
\newcommand{\frw}{\mathfrak{w}}
\newcommand{\frx}{\mathfrak{x}}
\newcommand{\fry}{\mathfrak{y}}
\newcommand{\frz}{\mathfrak{z}}


==> styles/settings.tex <==
%% Packages
%\usepackage{mathtools}
\graphicspath{{figures/}}
\usepackage{color}
\usepackage[table]{xcolor}

\input{def}

%% Matrix options
\setcounter{MaxMatrixCols}{20}

%% colors (http://colorbrewer2.org) Colorblind save
\definecolor{color_good}{RGB}{145 191 219}
\newcommand{\tblbgg}{\cellcolor{color_good}}
\definecolor{color_bad}{RGB}{252 141 89}
\newcommand{\tblbgb}{\cellcolor{color_bad}}
\definecolor{new_neutral}{RGB}{255 255 191}
\newcommand{\tblbgn}{\cellcolor{new_neutral}}

%% Commenting
\newcommand{\addition}[1]{\textcolor{green}{\textbf{#1}}}
\newcommand{\remark}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\note}[1]{\textcolor{orange}{\textbf{#1}}}
\newcommand{\warning}[1]{\textcolor{red}{\textbf{#1}}}

%% Referencing
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\equref}[1]{Eq.~\ref{eq:#1}}
\newcommand{\algref}[1]{Alg.~\ref{alg:#1}}
\newcommand{\tabref}[1]{Tab.~\ref{tab:#1}}

%% Math Operators
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\logmap}{log}
\DeclareMathOperator{\expmap}{exp}
\DeclareMathOperator{\logmatrix}{log}
\DeclareMathOperator{\expmatrix}{exp}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\atantwo}{atan2}

%% Math Symbols
\newcommand\identity{\mathds{1}}
\newcommand\zero{\mathbf{0}}
\newcommand\norm[1]{\lVert #1 \rVert}
\newcommand\transpose{\mathsf{T}}

\newcommand\imquatvec[1]{\check{\mathbf{#1}}}
\newcommand\imquatvecFrame[3]{\check{\mathbf{#1}}_{#2\!#3}}
\newcommand\skewImquatvecFrame[3]{\hat{\check{\mathbf{#1}}}_{#2\!#3}}

\newcommand\pos[3]{{}_#1\vr_{#2\!#3}}
\newcommand\posdot[3]{{}_#1\dot{\vr}_{#2\!#3}}
\newcommand\poshat[3]{{}_#1\hat{\vr}_{#2\!#3}}
\newcommand\poshatdot[3]{{}_#1\dot{\hat{\vr}}_{#2\!#3}}
\newcommand\postranspose[3]{{}_#1\vr_{#2\!#3}^\transpose}
\newcommand\rotmat[2]{\vR_{#1\!#2}}
\newcommand\drotmat[2]{\dot{\vR}_{#1\!#2}}
\newcommand\comat[2]{\vC_{#1\!#2}}
\newcommand\dcomat[2]{\dot{\vC}_{#1\!#2}}
\newcommand\quat[2]{\vq_{#1\!#2}}
\newcommand\Quat[2]{Q_{#1\!#2}}
\newcommand\angleaxis[2]{(\theta,\vn)_{#1\!#2}}
\newcommand\rotvec[2]{\vvph_{#1\!#2}}
\newcommand\linvel[2]{{}_#1\vv_{#2}}
\newcommand\rotvel[3]{{}_#1\vom_{#2\!#3}}
\newcommand\rotvelhat[3]{{}_#1\hat{\vom}_{#2\!#3}}
\newcommand\dvch[0]{\dot{\vch}}

\newcommand{\MSvec}[3]{#1_{#2}^{#3}}
\newcommand{\MSvecdot}[3]{\dot{#1}_{#2}^{#3}}
\newcommand{\MSvectranspose}[3]{#1_{#2}^{#3\;\transpose}}

\newcommand{\MSskew}[1]{\left[#1\right]_{\times}}

\newcommand{\MSdist}{\MSvec{{\vF_{\!d}}}{\cW}{}}
\newcommand{\MSdistdot}{\MSvecdot{{\vF_{\!d}}}{\cW}{}}
\newcommand{\MSdisttranspose}{\MSvectranspose{{\vF_{\!d}}}{\cG}{}}
\newcommand{\MSedist}{\Delta\MSvec{{\vF_{\!d}}}{\cW}{}}
\newcommand{\MSedisttranspose}{\Delta\MSvectranspose{{\vF_{\!d}}}{\cG}{}}
\newcommand{\MSmoment}{\MSvec{{\vM_{\!d}}}{\cG}{}}
\newcommand{\MSmomenttranspose}{\MSvectranspose{{\vM_{\!d}}}{\cG}{}}
\newcommand{\MSmomentdot}{\MSvecdot{{\vM_{\!d}}}{\cG}{}}

\newcommand{\MSez}{\mathbf{e}_{z}}
\newcommand{\MSezT}{\mathbf{e}_{z}^{T}}

\newcommand{\MSx}{\mathbf{x}}
\newcommand{\MSdx}{\dot{\mathbf{x}}}
\newcommand{\MSex}{\widetilde{\mathbf{x}}}

\newcommand{\MSp}{\mathbf{p}}
\newcommand{\MSpwi}{\MSvec{\vp}{\cW}{\cI}}
\newcommand{\MSdpwi}{\MSvecdot{\vp}{\cW}{\cI}}
\newcommand{\MSpwiT}{\MSvectranspose{\vp}{\cW}{\cI}}
\newcommand{\MSepwi}{\Delta\mathbf{p}_{W}^{I}}
\newcommand{\MSepwiT}{\Delta\mathbf{p}_{W}^{I\:T}}

\newcommand{\MSv}{\mathbf{v}}
\newcommand{\MSvwi}{\MSvec{\vv}{\cW}{\cI}}
\newcommand{\MSdvwi}{\MSvecdot{\vv}{\cW}{\cI}}
\newcommand{\MSvwiT}{\MSvectranspose{\vv}{\cW}{\cI}}
\newcommand{\MSevwi}{\Delta\mathbf{v}_{w}^{i}}
\newcommand{\MSevwiT}{\Delta\mathbf{v}_{w}^{i\:T}}

\newcommand{\MSa}{\mathbf{a}}
\newcommand{\MSai}{\mathbf{a}_{i}}
\newcommand{\MSdai}{\dot{\mathbf{a}}_{i}}
\newcommand{\MSaiT}{\mathbf{a}_{i}^{\:\:T}}
\newcommand{\MSaim}{\widetilde{\mathbf{a}}_{i}}
\newcommand{\MSaimT}{\MSvectranspose{\widetilde{\va}}{\cI}{}}
\newcommand{\MSeai}{\Delta\mathbf{a}_{i}}
\newcommand{\MSeaiT}{\Delta\mathbf{a}_{i}^{\:\:T}}

\newcommand{\MSq}{\mathbf{q}}
\newcommand{\MSqwi}{\MSvec{\bar{\vq}}{\cW}{\cI}}
\newcommand{\MSqwiRE}{\MSvec{\bar{\vq}}{\cW,\mathrm{RE}}{\cI}}
\newcommand{\MSqwiIM}{\MSvec{\bar{\vq}}{\cW,\mathrm{IM}}{\cI}}
\newcommand{\MSqwiIMT}{\MSvectranspose{\bar{\vq}}{\cW,\mathrm{IM}}{\cI}}
\newcommand{\MSqwiIMcs}{\MSskew{\MSqwiIM}}
\newcommand{\MSdqwi}{\MSvecdot{\bar{\vq}}{\cW}{\cI}}
\newcommand{\MSqwiT}{\MSvectranspose{\bar{\vq}}{\cW}{\cI}}
\newcommand{\MSqwiLm}{\left[\MSqwi\right]_{L}}
\newcommand{\MSeqwi}{\delta\mathbf{q}_{w}^{i}}
\newcommand{\MSeqwiT}{\delta\mathbf{q}_{w}^{i\:T}}

\newcommand{\MSethetawi}{\delta\mathbf{\theta}_{w}^{i}}
\newcommand{\MSethetawiT}{\delta\mathbf{\theta}_{w}^{i\:T}}
\newcommand{\MSedthetawi}{\delta\dot{\mathbf{\theta}}_{w}^{i}}

\newcommand{\MSomega}{\boldsymbol{\omega}}
\newcommand{\MSomegai}{\MSvec{\vom}{\cI}{}}
\newcommand{\MSomegaics}{\left[\boldsymbol{\omega}_{i}\right]_{\times}}
\newcommand{\MSdomegai}{\MSvecdot{\vom}{\cI}{}}
\newcommand{\MSddomegai}{\ddot{\boldsymbol{\omega}}_{i}}
\newcommand{\MSdomegaics}{\left[\dot{\boldsymbol{\omega}}_{i}\right]_{\times}}
\newcommand{\MSddomegaics}{\left[\ddot{\boldsymbol{\omega}}_{i}\right]_{\times}}
\newcommand{\MSomegaiT}{\MSvectranspose{\vom}{\cI}{}}
\newcommand{\MSomegaim}{\widetilde{\boldsymbol{\omega}}_{i}}
\newcommand{\MSomegaimT}{\MSvectranspose{\widetilde{\vom}}{\cI}{}}
\newcommand{\MSeomegai}{\Delta\boldsymbol{\omega}_{i}}
\newcommand{\MSeomegaiT}{\Delta\boldsymbol{\omega}_{i}^{\:\:T}}
\newcommand{\MSomegaiest}{\hat{\boldsymbol{\omega}}_{i}}
\newcommand{\MSomegaiestcs}{\left[\hat{\boldsymbol{\omega}}_{i}\right]_{\times}}
\newcommand{\MSomegaiecs}{\left[\Delta\boldsymbol{\omega}_{i}\right]_{\times}}

\newcommand{\MSb}{\mathbf{b}}

\newcommand{\MSbomega}{\MSvec{\vb}{\vom_{\cI}}{}}
\newcommand{\MSdbomega}{\MSvecdot{\vb}{\vom_{\cI}}{}}
\newcommand{\MSbomegaT}{\MSvectranspose{\vb}{\vom_{\cI}}{}}
\newcommand{\MSebomega}{\Delta\mathbf{b}_{\omega_I}}
\newcommand{\MSebomegaT}{\Delta\mathbf{b}_{\omega_I}^{\:\:T}}

\newcommand{\MSba}{\MSvec{\vb}{\va_{\cI}}{}}
\newcommand{\MSdba}{\MSvecdot{\vb}{\va_{\cI}}{}}
\newcommand{\MSbaT}{\MSvectranspose{\vb}{\va_{\cI}}{}}
\newcommand{\MSeba}{\Delta\mathbf{b}_{a_I}}
\newcommand{\MSebaT}{\Delta\mathbf{b}_{a_I}^{\:\:T}}

\newcommand{\MSi}{\MSvec{\boldsymbol{i}}{\cG}{}}
\newcommand{\MSiinv}{\MSvec{\boldsymbol{i}}{\cG}{-1}}
\newcommand{\MSdi}{\MSvecdot{\boldsymbol{i}}{\cG}{}}
\newcommand{\MSiT}{\MSvectranspose{\boldsymbol{i}}{\cG}{}}
\newcommand{\MSei}{\Delta\boldsymbol{i}}
\newcommand{\MSeiT}{\Delta\boldsymbol{i}^{\,T}}

\newcommand{\MSpig}{\MSvec{\vp}{\cI}{\cG}}
\newcommand{\MSdpig}{\MSvecdot{\vp}{\cI}{\cG}}
\newcommand{\MSddpig}{\ddot{\mathbf{p}}_{i}^{g}}
\newcommand{\MSpigT}{\MSvectranspose{\vp}{\cI}{\cG}}
\newcommand{\MSpigcs}{\left[\mathbf{p}_{i}^{g}\right]_{\times}}
\newcommand{\MSpigestcs}{\left[\hat{\mathbf{p}}_{i}^{g}\right]_{\times}}
\newcommand{\MSepig}{\Delta\mathbf{p}_{i}^{g}}
\newcommand{\MSepigT}{\Delta\mathbf{p}_{i}^{g\:T}}

\newcommand{\MSpis}{\MSvec{\vp}{\cI}{\cS}}
\newcommand{\MSdpis}{\MSvecdot{\vp}{\cI}{\cS}}
\newcommand{\MSpisT}{\MSvectranspose{\vp}{\cI}{\cS}}
\newcommand{\MSepis}{\Delta\mathbf{p}_{i}^{s}}
\newcommand{\MSepisT}{\Delta\mathbf{p}_{i}^{s\:T}}

\newcommand{\MSqis}{\MSvec{\bar{\vq}}{\cI}{\cS}}
\newcommand{\MSdqis}{\MSvecdot{\bar{\vq}}{\cI}{\cS}}
\newcommand{\MSqisT}{\MSvectranspose{\bar{\vq}}{\cI}{\cS}}
\newcommand{\MSeqis}{\delta\mathbf{q}_{i}^{s}}
\newcommand{\MSeqisT}{\delta\mathbf{q}_{i}^{s\:T}}
\newcommand{\MSqisLm}{\left[\MSqis\right]_{L}}

\newcommand{\MSethetais}{\delta\mathbf{\theta}_{i}^{s}}
\newcommand{\MSethetaisT}{\delta\mathbf{\theta}_{i}^{s\:T}}

\newcommand{\MSpwsm}{\widetilde{\mathbf{p}}_{w}^{s}}
\newcommand{\MSpwsmT}{\MSvectranspose{\widetilde{\vp}}{\cW}{\cS}}
\newcommand{\MSqwsm}{\widetilde{\mathbf{q}}_{w}^{s}}
\newcommand{\MSqwsmT}{\MSvectranspose{\widetilde{\bar{\vq}}}{\cW}{\cS}}

\newcommand{\MSu}{\mathbf{u}}

\newcommand{\MSF}{\mathrm{F}_{\!c}}
%\newcommand{\MSF}{\mathbf{F}}
\newcommand{\MSFT}{\mathbf{F}^{\:T}}
\newcommand{\MSdF}{\dot{F}}
%\newcommand{\MSdF}{\dot{\mathbf{F}}}
\newcommand{\MSdFT}{\dot{\mathbf{F}}^{\:T}}

\newcommand{\MSM}{\mathbf{M}_{\!c}}
\newcommand{\MSMT}{\vM^{\transpose}_{\!c}}
\newcommand{\MSdM}{\dot{\mathbf{M}}}
\newcommand{\MSdMT}{\dot{\mathbf{M}}^{\:T}}

\newcommand{\MSz}{\mathbf{z}}
\newcommand{\MSzero}{\mathbf{0}}

\newcommand{\MScqwi}{\MSvec{\vC}{\left(\MSqwi\right)}{}}
\newcommand{\MSdcqwi}{\mathbf{\dot{C}}_{\left(\mathbf{q}_{w}^{i}\right)}}
\newcommand{\MSdcqwiT}{\mathbf{\dot{C}}_{\left(\mathbf{q}_{w}^{i\:T}\right)}}
\newcommand{\MScqwiT}{\mathbf{C}_{\left(\mathbf{q}_{w}^{i}\right)}^{\:T}}

\newcommand{\MSRwi}{\mathbf{R}_{\mathcal{W}}^{\mathcal{I}}}
\newcommand{\MSRiw}{\mathbf{R}_{\mathcal{I}}^{\mathcal{W}}}

\newcommand{\MSg}{\vg_\cW}

\newcommand{\MSRomegai}{\Omega\left(\MSomegai\right)}

\newcommand{\MSinertia}{\MSvec{\vI}{\cG}{}}%\mathbb{I}}
\newcommand{\MSinertiainv}{\MSvec{\vI}{\cG}{-1}}
\newcommand{\MSinertiaest}{\hat{\mathbf{I}}_{G}}%\mathbb{I}}

\newcommand{\MSn}{\mathbf{n}}
\newcommand{\MSnbomega}{\mathbf{n}_{\vb_{\omega}}}
\newcommand{\MSnba}{\mathbf{n}_{\vb_{a}}}
\newcommand{\MSnF}{\mathrm{n}_{F}}
\newcommand{\MSnM}{\mathbf{n}_{\mathbf{M}}}
\newcommand{\MSnai}{\mathbf{n}_{\va_{\cI}}}
\newcommand{\MSnomega}{\mathbf{n}_{\vom_\cI}}
\newcommand{\MSnp}{\mathbf{n}_{\vp}}
\newcommand{\MSnq}{\mathbf{n}_{\bar{\vq}}}
\newcommand{\MSndist}{\mathbf{n}_{\vF_{\!d}}}
\newcommand{\MSnmoment}{\mathbf{n}_{\vM_{\!d}}}

\newcommand{\MSdm}{\dot{m}_{\cG}}

\newcommand{\MSho}{\boldsymbol{h}_{1}}
\newcommand{\MSht}{\boldsymbol{h}_{2}}
\newcommand{\MShth}{h_{3}}
\newcommand{\MShf}{\boldsymbol{h}_{4}}
\newcommand{\MShfi}{\boldsymbol{h}_{5}}
\newcommand{\MShs}{h_{6}}

\newcommand{\MSthrust}{\mathbf{t}_{I}}
\newcommand{\MSnthrust}{\left\lVert\mathbf{t}_{I}\right\rVert}
\newcommand{\MSdthrust}{\dot{\mathbf{t}}_{I}}

\newcommand{\MSqi}{\mathbf{q}_{I}}

\newcommand{\MSidentity}[1]{\boldsymbol{I}_{#1}}
\newcommand{\MSzeros}[1]{\boldsymbol{0}_{#1}}

%% Math Operators
% \DeclareMathOperator{\diag}{diag}

%% Matrix options
\setcounter{MaxMatrixCols}{20}

% % % numbers option provides compact numerical references in the text. 
% % %\usepackage{multicol}
% % \usepackage[normalem]{ulem}
% % \usepackage[bookmarks=true]{hyperref}
% % %\usepackage[numbers,sort]{natbib}
% % %\usepackage{cite}
% % %\usepackage{times}
% % %\usepackage{wrapfig}
% % %\usepackage{tweaklist}
% % %\usepackage{xspace}
% % \usepackage{graphicx}
% % %\usepackage[version=latest]{pgf}
% % \usepackage{tabularx}
% % \usepackage{amsmath}
% % \usepackage{amssymb}
% % \usepackage{url}
% % %\usepackage{bm}
% % \usepackage{color}
% % \usepackage{xcolor}
% % %\usepackage{colortbl}
% % %\usepackage{subfig}
% % %\usepackage[ruled,vlined]{./algorithm2e}
% % \usepackage{subfigure}
% % \usepackage{multirow}
% % %\usepackage{calrsfs}
% % %\usepackage{graphicx,import}
% % %\DeclareGraphicsExtensions{.pdf,.jpeg,.png}
% % \graphicspath{{figures/}}
% % %\usepackage{balance}
% % %\usepackage{amssymb}
% % \usepackage{comment}
% % \usepackage{siunitx}
% % \usepackage{nicefrac}
% % %\usepackage{flushend}
% % \usepackage{tikz}
% % \usetikzlibrary{shapes,arrows}

% % % Table caption wrangling
% % \usepackage{etoolbox}
% % \makeatletter
% % \patchcmd{\@makecaption}
% %   {\scshape}
% %   {}
% %   {}
% %   {}
% % \makeatletter
% % \patchcmd{\@makecaption}
% %   {\\}
% %   {.\ }
% %   {}
% %   {}
% % \makeatother

% % \usepackage{calrsfs}
% % \DeclareMathAlphabet{\pazocal}{OMS}{zplm}{m}{n}

% % bold variable shortcuts
% \newcommand{\vt}{\mathbf{t}}
% \newcommand{\by}{\mathbf{y}}
% \newcommand{\mt}{\mathbf{T}}
% \newcommand{\R}{\mathbb{R}}
% % \renewcommand{\P}{\pazocal{P}} % note: this replaces the "paragraph symbol"

% % special diagonal dots
% \newcommand{\dotsangle}{13}
% \newcommand{\dotsxshift}{.2ex}
% \newcommand{\dotsyshift}{0.2ex}
% \newcommand{\rdots}{\hspace{\dotsxshift}\raisebox{\dotsyshift}{\rotatebox{\dotsangle}{$\ddots$}}}

% % small bmatrix
% \newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}

% \newcommand{\tstart}{0}
% \newcommand{\tend}{T}
% \newcommand{\EELOG}{\texorpdfstring{{E\textsuperscript{2}LOG}}{E2LOG}}
% \newcommand{\EELOGobj}{\sigma_{\min}(\EELOG{})}
% \newcommand{\EWo}{\widetilde{W}_o}
% \newcommand{\sigMinTheta}{\sigma_{\min}(\EWo(\theta))}

% % correct bad hyphenation here
% \hyphenation{op-ti-cal net-works se-mi-con-duc-tor par-ti-cu-lar}
% %\graphicspath{{paper_figures/}}
% %\include{preamble}


% %easy commenting
% \newcommand{\rem}[1]{\textcolor{red}{\textbf{#1}}}
% \newcommand{\Karol}[1]{#1}
% \newcommand{\SW}[1]{\textcolor{green}{#1}}
% \newcommand{\CB}[1]{\textcolor{cyan}{\textbf{#1}}}
% \newcommand{\Karolnew}[1]{#1}
% \newcommand{\Stephannew}[1]{\textcolor{blue}{#1}}
% %\newcommand{\camready}[1]{\textcolor{cyan}{\textbf{camera-ready: #1}}}
% \newcommand{\camready}[1]{}

% % pretty formatting to "highlight changes"
% \definecolor{diffnewbg}{rgb}{0.9, 1.0, 0.9}
% \definecolor{diffnewfg}{rgb}{0.0, 0.6, 0.0}
% \definecolor{diffoldbg}{rgb}{1.0, 0.9, 0.9}
% \definecolor{diffoldfg}{rgb}{0.9, 0.2, 0.2}
% \newcommand{\replace}[2]{\colorbox{diffnewbg}{\textcolor{diffnewfg}{#1}}\colorbox{diffoldbg}{\textcolor{diffoldfg}{\sout{#2}}}}

% %for one of the tables
% \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% \DeclareMathOperator*{\minimize}{minimize}


% \setcounter{secnumdepth}{3}





% \DeclareMathOperator*{\Ex}{E}
% \DeclareMathOperator{\Var}{Var}
% \DeclareMathOperator{\Cov}{Cov}
% \DeclareMathOperator{\Tr}{tr}
% \DeclareMathOperator{\Vect}{vec}
% \DeclareMathOperator{\diag}{diag}
% %\DeclareMathOperator{\st}{s.t.}
% \DeclareMathOperator{\dt}{dt}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\Dim}{\texttt{dim}}
% \DeclareMathOperator*{\sd}{\texttt{sd}}

% \newcommand{\bx}{\mathbf{x}}
% \newcommand{\be}{\mathbf{e}}
% \newcommand{\bg}{\mathbf{g}}
% \newcommand{\hbx}{\hat{\mathbf{x}}}
% \newcommand{\bbx}{\bar{\mathbf{x}}}
% \newcommand{\btheta}{\boldsymbol{\theta}}
% \newcommand{\bpsi}{\boldsymbol{\psi}}
% \newcommand{\bu}{\mathbf{u}}
% %\newcommand{\bm}{\mathbf{m}}
% \newcommand{\bz}{\mathbf{z}}
% \newcommand{\bn}{\mathbf{n}}
% \newcommand{\bp}{\mathbf{p}}
% \newcommand{\hbp}{\hat{\mathbf{p}}}
% \newcommand{\bq}{\mathbf{q}}
% %\newcommand{\bf}{\mathbf{f}}
% \newcommand{\bh}{\mathbf{h}}
% \newcommand{\br}{\mathbf{r}}
% \newcommand{\bb}{\mathbf{b}}
% \newcommand{\bv}{\mathbf{v}}
% \newcommand{\bC}{\mathbf{C}}
% \newcommand{\hbb}{\hat{\mathbf{b}}}
% \newcommand{\hbn}{\hat{\mathbf{n}}}
% \newcommand{\bbb}{\bar{\mathbf{b}}}
% \newcommand{\bbu}{\bar{\mathbf{u}}}
% \newcommand{\hbpsi}{\hat{\boldsymbol \psi}}
% \newcommand{\bdelta}{\boldsymbol \delta}
% \newcommand{\hdelta}{\hat{\delta}}
% \newcommand{\hbdelta}{\hat{\boldsymbol \delta}}
% \newcommand{\bbdelta}{\bar{\boldsymbol \delta}}
% \newcommand{\bPsi}{\boldsymbol \Psi}
% \newcommand{\bw}{\mathbf{w}}
% \newcommand{\mA}{\mathcal{A}}
% \newcommand{\mN}{\mathcal{N}}
% \newcommand{\mO}{\mathcal{O}}
% \newcommand{\mcalP}{\mathcal{P}}
% \newcommand{\mB}{\mathcal{B}}
% \newcommand{\mX}{\mathcal{X}}
% \newcommand{\mZ}{\mathcal{Z}}
% \newcommand{\mQ}{\mathcal{Q}}
% \newcommand{\mR}{\mathcal{R}}
% \newcommand{\mU}{\mathcal{U}}
% \newcommand{\hmB}{\hat{\mathcal{B}}}
% \newcommand{\hmU}{\hat{\mathcal{U}}}
% \newcommand{\bmB}{\bar{\mathcal{B}}}
% \newcommand{\bmU}{\bar{\mathcal{U}}}
% \newcommand{\mT}{\pazocal{T}}
% \newcommand{\mM}{\mathcal{M}}
% \newcommand{\bPhi}{\boldsymbol{\Phi}}
% \newcommand{\sS}[1]{\sqrt{\Sigma_{#1}}}
% \newcommand{\shS}[1]{\sqrt{\hat{\Sigma}_{#1}}}
% \newcommand{\pd}{\Delta}
% \newcommand{\ubar}[1]{\underaccent{\bar}{#1}}


% %ours
% \newcommand{\todo}[1]{\textbf{\textcolor{red}{TODO: #1}}}
% \newcommand{\KH}[1]{\textbf{\textcolor{blue}{#1}}}
%  \setlength{\abovecaptionskip}{1ex}
%  \setlength{\belowcaptionskip}{1ex}
%  \setlength{\floatsep}{1ex}
%  \setlength{\textfloatsep}{1ex}

% \newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
% \newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
% \newcommand{\equref}[1]{Eq.~\ref{eq:#1}}
% \newcommand{\algref}[1]{Alg.~\ref{alg:#1}}
% \newcommand{\tabref}[1]{Tab.~\ref{tab:#1}}
% \newcommand{\prob}[1]{\text{p}(#1)} % probability
% \newcommand{\set}[1]{\mathbf{#1}} % Capital set bold letter
% \newcommand{\expectedValue}[2]{\hollow{E}_{#2}#1} % expected value
% \newcommand{\hollow}[1]{\mathbb{#1}} % hollow letter
% \DeclareMathAlphabet{\pazocal}{OMS}{zplm}{m}{n}
% \newcommand{\entropy}[1]{\text{H}\left[\;#1 \; \right]} % entropy
% \newcommand{\M}{\pazocal{M}}
% \newcommand{\D}{\pazocal{D}}
% \newcommand{\W}{\pazocal{W}}
% \newcommand{\N}{\pazocal{N}}
% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
% %\newcommand{\SW}[1]{\textbf{\textcolor{blue}{SW: #1}}}
% %\newcommand{\KH}[1]{\textbf{\textcolor{green}{KH: #1}}}
% \definecolor{jpgreen}{rgb}{0.0 0.7 0.3}
% \newcommand{\JP}[1]{\textbf{\textcolor{jpgreen}{JP: #1}}}
% \newcommand{\vc}{\mathbf{c}}
% \newcommand{\vy}{\mathbf{y}}
% \newcommand{\vp}{\mathbf{p}}
% \newcommand{\mP}{\mathbf{P}}



